The Populations of Carina. II. Chemical Enrichment

Chemical abundances are presented for 19 elements in a sample of 63 red giants in the Carina dwarf spheroidal galaxy (dSph), based on homogeneous 1D/LTE model atmosphere analyses of our own observations (32 stars) and data available in the literature (a further 31 independent stars). The (Fe) metallicity and [$\alpha$/Fe] distribution functions have mean values and dispersions of -1.59 and 0.33 dex ([Fe/H] range: -2.68 to -0.64), and 0.07 and 0.13 dex ([$\alpha$/Fe] range: -0.27 to 0.25), respectively. We confirm the finding of Venn et al. (2012) that a small percentage (some 10% in the present investigation) of the sample show clear evidence for significant enrichment by Type Ia supernovae ejecta. Calcium, with the most accurately determined abundance of the alpha-elements, shows an asymmetric distribution towards smaller values of [Ca/Fe] at all [Fe/H], most significantly over -2.0 < [Fe/H] < -1.0, suggestive of incomplete mixing of the ejecta of Type Ia SNe with the ambient medium of each of Carina's generations. Approximate color-magnitude-diagram age estimates are presented for the sample and, together with our chemical abundances, compared with the results of our previous synthetic CMD analysis, which reported the details of Carina's four well-defined populations. We searched for the Na-O anti-correlation universally reported in the Galaxy's globular clusters, and confirm that this phenomenon does not exist in Carina. We also found that one of the 32 stars in our sample has an extremely enhanced lithium abundance -- A(Li)$_{\text{NLTE}}$ = +3.36, consistent with membership of the ~1% group of Li-rich stars in dSph described by Kirby et al.

==> table1.tex <==
 
% Table 1
\begin{deluxetable}{cccccccccc}                                                                                                                   
\tablecolumns{10}                                                                                                                            
\tablewidth{0pt}

\tabletypesize{\scriptsize}
\tablecaption{\label{tab:obsdat} Coordinates, Photometry, and Radial Velocities for 32 Carina Red Giants}                  
\tablehead{                                                                                                                              
  \colhead{Object} & {RA (2000)  Dec (2000) } & {$V$}       & {$B-V$}        &    {$I$} &    {$J$}  &     {$H$} &     {$K$} &  {Vrad} &  {$\sigma$(Vrad)} \\  
            {(1)}   & {(2)}              & {(3)}       & {(4)}          &    {(5)} &    {(6)}  &    {(7)}  &     {(8)} &   {(9)} &  {(10)}  
  }                                                                                                                                       
\startdata                                                                                                                               
CC06122 &   06 41 39.64 $-$50 49 58.8 &   17.60 &    1.43 &   16.18 &   15.23 &   14.48 &   14.34 & 230.31 & 0.08  \\
CC06486 &   06 41 46.00 $-$50 51 00.6 &   18.17 &    1.24 &   16.89 &   16.01 &   15.41 &   15.27 & 226.23 & 0.19  \\
CC06975 &   06 42 10.86 $-$50 52 20.6 &   18.38 &    1.11 &   17.13 &   16.23 &   15.65 &   15.55 & 229.57 & 0.18  \\
CC07452 &   06 40 58.46 $-$50 53 35.5 &   17.80 &    1.29 &   16.41 &   15.52 &   14.88 &   14.74 & 225.23 & 0.09  \\
CC07889 &   06 41 40.83 $-$50 54 45.8 &   18.55 &    1.06 &   17.34 &   16.53 &   15.97 &   15.83 & 236.29 & 0.27  \\
CC08447 &   06 41 10.54 $-$50 55 53.0 &   17.99 &    1.25 &   16.65 &   15.72 &   15.09 &   14.94 & 232.52 & 0.10  \\
CC08469 &   06 42 17.43 $-$50 55 55.3 &   17.81 &    1.29 &   16.43 &   15.47 &   14.80 &   14.64 & 223.63 & 0.11  \\
CC08615 &   06 41 49.58 $-$50 56 11.5 &   18.50 &    1.05 &   17.32 &   16.45 &   15.93 &   15.78 & 223.91 & 0.21  \\
CC08695 &   06 41 36.49 $-$50 56 23.3 &   17.88 &    1.29 &   16.53 &   15.53 &   14.90 &   14.74 & 228.46 & 0.08  \\
CC08788 &   06 41 50.10 $-$50 56 35.2 &   18.59 &    1.04 &   17.41 &   16.56 &   16.03 &   15.92 & 228.31 & 0.11  \\
CC09000 &   06 41 54.60 $-$50 57 00.9 &   17.67 &    1.49 &   16.10 &   15.06 &   14.44 &   14.27 & 230.46 & 0.14  \\
CC09179 &   06 41 17.93 $-$50 57 20.5 &   18.30 &    1.13 &   17.04 &   16.14 &   15.58 &   15.46 & 233.00 & 0.19  \\
CC09225 &   06 41 19.70 $-$50 57 25.6 &   18.01 &    1.21 &   16.71 &   15.74 &   15.14 &   15.02 & 220.18 & 0.07  \\
CC09226 &   06 41 12.30 $-$50 57 26.1 &   18.33 &    1.04 &   17.13 &   16.25 &   15.69 &   15.57 & 219.84 & 0.20  \\
CC09430 &   06 42 05.38 $-$50 57 48.6 &   18.26 &    1.15 &   16.98 &   16.07 &   15.48 &   15.35 & 223.54 & 0.19  \\
CC09507 &   06 41 54.08 $-$50 57 56.8 &   18.31 &    1.06 &   17.13 &   16.29 &   15.73 &   15.58 & 227.39 & 0.20  \\
CC09633 &   06 41 53.85 $-$50 58 11.2 &   17.88 &    1.21 &   16.53 &   15.62 &   15.04 &   14.90 & 219.04 & 0.25  \\
CC09869 &   06 40 56.96 $-$50 58 38.4 &   18.11 &    1.20 &   16.81 &   15.89 &   15.28 &   15.13 & 219.07 & 0.07  \\
CC09929 &   06 41 54.84 $-$50 58 47.0 &   18.47 &    1.11 &   17.21 &   16.31 &   15.72 &   15.57 & 217.07 & 0.27  \\
CC10038 &   06 42 02.81 $-$50 58 59.5 &   18.25 &    1.16 &   16.98 &   16.06 &   15.45 &   15.32 & 222.85 & 0.11  \\
CC10194 &   06 40 30.85 $-$50 59 15.4 &   17.76 &    1.29 &   16.38 &   15.38 &   14.77 &   14.62 & 215.26 & 0.20  \\
CC10318 &   06 41 57.63 $-$50 59 32.8 &   17.97 &    1.25 &   16.61 &   15.65 &   14.99 &   14.84 & 222.46 & 0.15  \\
CC10414 &   06 41 47.63 $-$50 59 44.2 &   18.13 &    1.19 &   16.84 &   15.92 &   15.29 &   15.13 & 222.14 & 0.18  \\
CC10686 &   06 41 27.18 $-$51 00 18.4 &   17.75 &    1.30 &   16.36 &   15.37 &   14.69 &   14.55 & 232.56 & 0.08  \\
CC10690 &   06 41 16.31 $-$51 00 18.7 &   18.14 &    1.16 &   16.84 &   15.92 &   15.33 &   15.19 & 222.15 & 0.22  \\
CC10802 &   06 41 27.55 $-$51 00 34.9 &   18.64 &    1.06 &   17.45 &   16.61 &   15.99 &   15.83 & 236.63 & 0.24  \\
CC10944 &   06 41 16.76 $-$51 00 54.1 &   17.78 &    1.28 &   16.46 &   15.52 &   14.88 &   14.75 & 220.43 & 0.15  \\
CC11217 &   06 41 05.01 $-$51 01 36.0 &   17.62 &    1.37 &   16.20 &   15.20 &   14.50 &   14.37 & 220.78 & 0.12  \\
CC11388 &   06 40 58.04 $-$51 02 00.3 &   17.92 &    1.20 &   16.62 &   15.68 &   15.07 &   14.94 & 224.83 & 0.22  \\
CC11560 &   06 40 59.29 $-$51 02 26.7 &   18.14 &    1.15 &   16.87 &   15.98 &   15.38 &   15.23 & 217.57 & 0.12  \\
CC12038 &   06 41 00.31 $-$51 03 43.1 &   18.42 &    1.10 &   17.19 &   16.29 &   15.70 &   15.58 & 223.79 & 0.29  \\
CC12039 &   06 41 21.98 $-$51 03 43.3 &   17.78 &    1.27 &   16.42 &   15.50 &   14.83 &   14.71 & 219.02 & 0.07  \\
\enddata                                                                                                      
\end{deluxetable}      


==> table10.tex <==
% Table 10

\begin{deluxetable}{lrrrrrrrrrrrrrrrrrrrrr}                                                                                    
\tabletypesize{\tiny}                                                                                                   
\tablecolumns{22}                                                                                                       
\tablewidth{0pt}                                                                                                        
\rotate                                                                                                                 
\tablecaption{\label{tab:relabs_kvs} Summary\tablenotemark{a} of [Fe/H], [X/Fe], and Total Errors $\sigma_{\rm {Tot}}$ for 14 Literature (\citet{venn12} \& \citet{shetrone03}) Carina Red Giants}                          
\tablehead{                                                                                                                              
  \colhead{Object} & {[Fe/H]} & {O}  & {Na} & {Mg} & {Al} & {Si} & {Ca} & {Sc} & {Ti~I} & {Ti~II} & {V} & {Cr} & {Mn} & {Fe~II} & {Co} & {Ni} & {Cu} & {Ba} & {La} & {Nd} & {Eu}\\  
  }
\startdata    
     Car$-$484   &  $-$1.49 &   0.50 &  $-$0.34 &   0.16 &    ... &    ... &   0.05 &   0.08 &   0.14 &   0.24 &  $-$0.07 &  $-$0.04 &  $-$0.37 &   0.12 &    ... &  $-$0.07 &    ... &   0.30 &   0.51 &   0.67 &   0.51 \\
               &   0.14 &   0.22 &   0.20 &   0.10 &    ... &    ... &   0.04 &   0.12 &   0.09 &   0.12 &   0.10 &   0.09 &   0.06 &   0.15 &    ... &   0.07 &    ... &   0.21 &   0.11 &   0.20 &   0.22 \\
               &     75 &      1 &      1 &      2 &    ... &    ... &     20 &      8 &      7 &      4 &      8 &      3 &      6 &      7 &    ... &      9 &    ... &      1 &      3 &      1 &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
     Car$-$524   &  $-$1.73 &   0.47 &    ... &   0.25 &    ... &   0.41 &  $-$0.01 &  $-$0.02 &   0.07 &   0.03 &  $-$0.03 &  $-$0.05 &  $-$0.37 &   0.17 &    ... &  $-$0.02 &    ... &   0.19 &   0.61 &   0.44 &    ... \\
               &   0.14 &   0.21 &    ... &   0.13 &    ... &   0.21 &   0.05 &   0.13 &   0.17 &   0.13 &   0.19 &   0.14 &   0.11 &   0.16 &    ... &   0.06 &    ... &   0.20 &   0.11 &   0.19 &    ... \\
               &     64 &      1 &    ... &      2 &    ... &      1 &     19 &      7 &      2 &      4 &      1 &      3 &      3 &      8 &    ... &      6 &    ... &      1 &      2 &      1 &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
     Car$-$612   &  $-$1.38 &    ... &    ... &  $-$0.49 &    ... &    ... &  $-$0.25 &  $-$0.48 &  $-$0.37 &  $-$0.17 &  $-$0.58 &  $-$0.19 &  $-$0.46 &   0.30 &    ... &  $-$0.30 &    ... &  $-$0.45 &    ... &  $-$0.34 &    ... \\
               &   0.14 &    ... &    ... &   0.14 &    ... &    ... &   0.04 &   0.15 &   0.24 &   0.11 &   0.22 &   0.16 &   0.15 &   0.16 &    ... &   0.06 &    ... &   0.19 &    ... &   0.22 &    ... \\
               &     72 &    ... &    ... &      2 &    ... &    ... &     19 &      4 &      2 &      4 &      1 &      3 &      5 &     12 &    ... &      7 &    ... &      2 &    ... &      1 &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
     Car$-$705   &  $-$1.52 &   0.29 &  $-$0.17 &   0.19 &    ... &    ... &   0.06 &   0.21 &   0.11 &   0.19 &   0.02 &  $-$0.24 &  $-$0.30 &   0.23 &    ... &   0.02 &    ... &  $-$0.38 &    ... &   0.26 &    ... \\
               &   0.14 &   0.25 &   0.22 &   0.23 &    ... &    ... &   0.04 &   0.13 &   0.10 &   0.11 &   0.11 &   0.24 &   0.09 &   0.17 &    ... &   0.08 &    ... &   0.20 &    ... &   0.23 &    ... \\
               &     74 &      1 &      1 &      2 &    ... &    ... &     19 &      8 &      7 &      4 &      9 &      3 &      6 &      9 &    ... &      9 &    ... &      3 &    ... &      1 &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
     Car$-$769   &  $-$1.74 &   0.67 &   0.01 &   0.42 &    ... &   0.53 &   0.13 &   0.27 &   0.36 &   0.30 &   0.21 &   0.01 &  $-$0.13 &   0.33 &    ... &   0.05 &    ... &   0.04 &   0.80 &   0.25 &    ... \\
               &   0.14 &   0.24 &   0.22 &   0.09 &    ... &   0.23 &   0.07 &   0.14 &   0.10 &   0.16 &   0.17 &   0.21 &   0.14 &   0.16 &    ... &   0.06 &    ... &   0.12 &   0.23 &   0.22 &    ... \\
               &     67 &      1 &      1 &      2 &    ... &      1 &     21 &      7 &      4 &      4 &      4 &      3 &      4 &      8 &    ... &      6 &    ... &      3 &      1 &      1 &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    Car$-$1013   &  $-$1.49 &    ... &  $-$0.19 &   0.16 &    ... &   0.24 &  $-$0.11 &   0.04 &   0.22 &   0.48 &   0.06 &   0.12 &  $-$0.42 &   0.18 &   0.14 &  $-$0.11 &    ... &   0.05 &    ... &   0.40 &   0.60 \\
               &   0.15 &    ... &   0.35 &   0.06 &    ... &   0.36 &   0.06 &   0.14 &   0.12 &   0.21 &   0.13 &   0.05 &   0.08 &   0.17 &   0.35 &   0.08 &    ... &   0.13 &    ... &   0.35 &   0.36 \\
               &     73 &    ... &      1 &      2 &    ... &      1 &     20 &      9 &      7 &      4 &     10 &      2 &      4 &     10 &      1 &      9 &    ... &      2 &    ... &      1 &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    Car$-$1087   &  $-$2.47 &    ... &    ... &   0.15 &    ... &    ... &  $-$0.45 &   0.06 &    ... &   0.53 &    ... &  $-$0.51 &    ... &    ... &    ... &    ... &    ... &  $-$1.07 &    ... &    ... &    ... \\
               &   0.16 &    ... &    ... &   0.26 &    ... &    ... &   0.15 &   0.16 &    ... &   0.28 &    ... &   0.26 &    ... &    ... &    ... &    ... &    ... &   0.28 &    ... &    ... &    ... \\
               &     16 &    ... &    ... &      1 &    ... &    ... &      3 &      2 &    ... &      1 &    ... &      1 &    ... &    ... &    ... &    ... &    ... &      1 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    Car$-$5070   &  $-$1.97 &    ... &    ... &  $-$0.51 &    ... &    ... &  $-$0.13 &   0.29 &    ... &  $-$0.12 &    ... &  $-$0.80 &    ... &    ... &    ... &   0.12 &    ... &  $-$0.80 &    ... &    ... &    ... \\
               &   0.15 &    ... &    ... &   0.25 &    ... &    ... &   0.11 &   0.21 &    ... &   0.26 &    ... &   0.05 &    ... &    ... &    ... &   0.18 &    ... &   0.26 &    ... &    ... &    ... \\
               &     28 &    ... &    ... &      1 &    ... &    ... &      5 &      3 &    ... &      1 &    ... &      2 &    ... &    ... &    ... &      4 &    ... &      1 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    Car$-$7002   &  $-$2.68 &    ... &    ... &  $-$0.01 &    ... &    ... &  $-$0.02 &    ... &    ... &   0.45 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &  $-$0.84 &    ... &    ... &    ... \\
               &   0.15 &    ... &    ... &   0.23 &    ... &    ... &   0.11 &    ... &    ... &   0.23 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   0.17 &    ... &    ... &    ... \\
               &     17 &    ... &    ... &      1 &    ... &    ... &      6 &    ... &    ... &      2 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &      2 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
          M2   &  $-$1.46 &   0.53 &  $-$0.46 &   0.15 &    ... &   0.10 &   0.08 &  $-$0.14 &   0.17 &   0.30 &    ... &   0.19 &  $-$0.36 &   0.03 &  $-$0.05 &  $-$0.29 &    ... &   0.22 &   0.30 &   0.29 &   0.26 \\
               &   0.14 &   0.20 &   0.17 &   0.05 &    ... &   0.19 &   0.05 &   0.19 &   0.19 &   0.10 &    ... &   0.16 &   0.07 &   0.16 &   0.17 &   0.16 &    ... &   0.13 &   0.13 &   0.17 &   0.20 \\
               &     41 &      1 &      1 &      2 &    ... &      1 &      9 &      1 &      2 &      2 &    ... &      1 &      6 &      9 &      1 &      1 &    ... &      3 &      2 &      1 &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
          M3   &  $-$1.79 &   0.43 &    ... &  $-$0.32 &    ... &    ... &  $-$0.21 &  $-$0.38 &    ... &   0.23 &    ... &  $-$0.01 &  $-$0.48 &   0.38 &    ... &   0.07 &    ... &   0.35 &   0.38 &   0.59 &   0.85 \\
               &   0.14 &   0.19 &    ... &   0.05 &    ... &    ... &   0.04 &   0.18 &    ... &   0.11 &    ... &   0.15 &   0.07 &   0.15 &    ... &   0.15 &    ... &   0.12 &   0.12 &   0.17 &   0.19 \\
               &     40 &      1 &    ... &      2 &    ... &    ... &      7 &      1 &    ... &      2 &    ... &      1 &      6 &     10 &    ... &      1 &    ... &      3 &      2 &      1 &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
          M4   &  $-$1.49 &   0.43 &  $-$0.31 &   0.20 &   0.14 &   0.11 &   0.04 &  $-$0.22 &  $-$0.01 &   0.25 &    ... &   0.07 &  $-$0.36 &   0.07 &    ... &  $-$0.04 &  $-$0.64 &   0.16 &   0.35 &   0.42 &   0.39 \\
               &   0.14 &   0.19 &   0.16 &   0.17 &   0.17 &   0.18 &   0.04 &   0.18 &   0.13 &   0.10 &    ... &   0.15 &   0.07 &   0.16 &    ... &   0.15 &   0.17 &   0.11 &   0.11 &   0.17 &   0.19 \\
               &     40 &      1 &      1 &      2 &      1 &      1 &      9 &      1 &      2 &      2 &    ... &      1 &      6 &     11 &    ... &      1 &      1 &      3 &      2 &      1 &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
         M10   &  $-$1.99 &   0.39 &    ... &   0.01 &    ... &    ... &  $-$0.10 &   0.27 &    ... &   0.03 &    ... &  $-$0.11 &  $-$0.44 &   0.29 &    ... &    ... &    ... &   0.43 &   0.70 &   0.81 &   1.17 \\
               &   0.14 &   0.20 &    ... &   0.09 &    ... &    ... &   0.05 &   0.19 &    ... &   0.10 &    ... &   0.16 &   0.07 &   0.16 &    ... &    ... &    ... &   0.11 &   0.12 &   0.17 &   0.20 \\
               &     32 &      1 &    ... &      2 &    ... &    ... &      8 &      1 &    ... &      2 &    ... &      1 &      3 &      9 &    ... &    ... &    ... &      3 &      2 &      1 &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
         M12   &  $-$1.35 &   0.43 &  $-$0.50 &   0.21 &  $-$0.02 &   0.27 &   0.01 &   0.11 &  $-$0.07 &   0.24 &    ... &   0.07 &  $-$0.37 &   0.22 &    ... &   0.01 &  $-$0.63 &   0.23 &   0.32 &   0.23 &   0.27 \\
               &   0.14 &   0.19 &   0.16 &   0.15 &   0.17 &   0.18 &   0.05 &   0.18 &   0.10 &   0.11 &    ... &   0.15 &   0.07 &   0.16 &    ... &   0.15 &   0.17 &   0.12 &   0.16 &   0.17 &   0.19 \\
               &     42 &      1 &      1 &      2 &      1 &      1 &      9 &      1 &      2 &      2 &    ... &      1 &      6 &     10 &    ... &      1 &      1 &      3 &      2 &      1 &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
\enddata
\tablenotetext{a}{For each object the three rows contain [Fe/H] and [X/Fe]; $\sigma_{\rm {Tot}}$; and the number of lines, respectively.}
\end{deluxetable}


==> table11.tex <==
% Table 11

\begin{deluxetable}{lrrrrrrrrrr}                                                                                    
\tabletypesize{\tiny}                                                                                                   
\tablecolumns{11}                                                                                                       
\tablewidth{0pt}                                                                                                        
\tablecaption{\label{tab:relabs_lem} Summary\tablenotemark{a} of [Fe/H], [X/Fe], and Total Errors $\sigma_{\rm {Tot}}$ for 35 \citet{lemasle12} Carina Red Giants}                          
\tablehead{                                                                                                                              
  \colhead{Object} & {[Fe/H]} & {Mg} & {Ca} & {Ti~I} & {Ti~II} & {Cr} & {Mn} & {Fe~II} & {Ni} & {Ba} \\  
  }
\startdata    
     MKV0397   &  $-$2.02 &    ... &   0.44 &    ... &   0.21 &  $-$0.62 &    ... &   0.24 &    ... &  $-$0.88 \\
               &   0.15 &    ... &   0.26 &    ... &   0.12 &   0.26 &    ... &   0.17 &    ... &   0.28 \\
               &     17 &    ... &      1 &    ... &      2 &      1 &    ... &      5 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0458   &  $-$1.47 &   0.07 &   0.33 &   0.31 &   0.33 &  $-$0.17 &  $-$0.48 &   0.40 &   0.47 &   0.27 \\
               &   0.15 &   0.24 &   0.31 &   0.10 &   0.10 &   0.24 &   0.24 &   0.16 &   0.24 &   0.12 \\
               &     26 &      1 &      2 &      3 &      2 &      1 &      1 &      5 &      1 &      2 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0514   &  $-$2.10 &   0.28 &   0.08 &    ... &   0.15 &  $-$0.11 &  $-$0.40 &   0.41 &    ... &  $-$0.98 \\
               &   0.15 &   0.23 &   0.09 &    ... &   0.14 &   0.23 &   0.23 &   0.22 &    ... &   0.11 \\
               &     26 &      1 &      5 &    ... &      2 &      1 &      1 &      3 &    ... &      2 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0556   &  $-$1.17 &   0.49 &   0.03 &    ... &   0.73 &   0.27 &    ... &   0.92 &    ... &   0.42 \\
               &   0.15 &   0.21 &   0.09 &    ... &   0.22 &   0.14 &    ... &   0.29 &    ... &   0.22 \\
               &     13 &      1 &      4 &    ... &      1 &      2 &    ... &      3 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0577   &  $-$1.61 &  $-$0.13 &   0.50 &   0.69 &   0.35 &  $-$0.07 &    ... &   0.77 &    ... &   0.13 \\
               &   0.15 &   0.29 &   0.29 &   0.30 &   0.31 &   0.29 &    ... &   0.33 &    ... &   0.31 \\
               &     23 &      1 &      1 &      1 &      1 &      1 &    ... &      1 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0596   &  $-$1.58 &  $-$0.08 &  $-$0.22 &   0.47 &   0.14 &   0.12 &  $-$0.22 &   0.06 &    ... &  $-$0.31 \\
               &   0.15 &   0.25 &   0.06 &   0.26 &   0.10 &   0.25 &   0.07 &   0.16 &    ... &   0.16 \\
               &     30 &      1 &      5 &      1 &      2 &      1 &      3 &      7 &    ... &      2 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0614   &  $-$1.55 &   0.03 &    ... &   0.35 &   0.18 &  $-$0.47 &    ... &   0.28 &    ... &   0.09 \\
               &   0.15 &   0.18 &    ... &   0.19 &   0.20 &   0.18 &    ... &   0.23 &    ... &   0.21 \\
               &     21 &      1 &    ... &      1 &      1 &      1 &    ... &      3 &    ... &      2 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0628   &  $-$1.71 &   0.41 &   0.09 &  $-$0.10 &   0.36 &   0.03 &    ... &   0.35 &    ... &  $-$0.07 \\
               &   0.14 &   0.21 &   0.08 &   0.22 &   0.12 &   0.15 &    ... &   0.16 &    ... &   0.22 \\
               &     32 &      1 &      8 &      1 &      2 &      2 &    ... &      4 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0640   &  $-$1.85 &   0.34 &   0.19 &   0.31 &   0.54 &   0.16 &  $-$0.16 &   0.32 &    ... &   0.34 \\
               &   0.15 &   0.24 &   0.05 &   0.20 &   0.10 &   0.11 &   0.13 &   0.17 &    ... &   0.25 \\
               &     30 &      1 &      8 &      2 &      2 &      2 &      3 &      7 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0652   &  $-$2.31 &   0.14 &  $-$0.28 &   1.34 &  $-$0.12 &  $-$0.54 &    ... &   0.21 &    ... &    ... \\
               &   0.15 &   0.24 &   0.23 &   0.24 &   0.25 &   0.24 &    ... &   0.27 &    ... &    ... \\
               &     16 &      1 &      1 &      1 &      1 &      1 &    ... &      1 &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0677   &  $-$1.66 &   0.33 &   0.12 &   0.08 &   0.50 &   0.19 &  $-$0.41 &   0.18 &    ... &  $-$0.05 \\
               &   0.14 &   0.19 &   0.06 &   0.12 &   0.15 &   0.19 &   0.09 &   0.16 &    ... &   0.10 \\
               &     31 &      1 &      8 &      3 &      2 &      1 &      3 &      8 &    ... &      2 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0698   &  $-$1.30 &   0.12 &   0.03 &   0.09 &  $-$0.02 &   0.11 &  $-$0.28 &   0.17 &    ... &    ... \\
               &   0.15 &   0.21 &   0.06 &   0.09 &   0.11 &   0.21 &   0.07 &   0.17 &    ... &    ... \\
               &     29 &      1 &      8 &      4 &      2 &      1 &      3 &      5 &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0708   &  $-$1.51 &   0.32 &    ... &    ... &   0.65 &  $-$0.08 &    ... &   0.27 &    ... &    ... \\
               &   0.16 &   0.25 &    ... &    ... &   0.27 &   0.25 &    ... &   0.21 &    ... &    ... \\
               &     11 &      1 &    ... &    ... &      1 &      1 &    ... &      2 &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0729   &  $-$1.17 &   0.52 &   0.31 &   0.04 &   0.73 &   0.52 &  $-$0.31 &   0.24 &   0.51 &   0.12 \\
               &   0.15 &   0.22 &   0.12 &   0.16 &   0.23 &   0.22 &   0.12 &   0.23 &   0.22 &   0.23 \\
               &     24 &      1 &      6 &      3 &      1 &      1 &      2 &      4 &      1 &      2 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0733   &  $-$1.55 &  $-$0.08 &  $-$0.06 &    ... &   0.28 &  $-$0.38 &   0.13 &   0.66 &    ... &   0.05 \\
               &   0.15 &   0.25 &   0.19 &    ... &   0.26 &   0.25 &   0.25 &   0.21 &    ... &   0.26 \\
               &     19 &      1 &      3 &    ... &      1 &      1 &      1 &      4 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0740   &  $-$0.97 &  $-$0.81 &  $-$0.58 &   0.43 &   0.19 &  $-$0.56 &  $-$0.34 &   0.42 &    ... &    ... \\
               &   0.15 &   0.23 &   0.22 &   0.23 &   0.13 &   0.23 &   0.23 &   0.16 &    ... &    ... \\
               &     15 &      1 &      1 &      1 &      2 &      1 &      1 &      2 &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0743   &  $-$0.64 &  $-$0.84 &  $-$0.50 &   0.34 &   0.26 &  $-$0.31 &  $-$0.51 &   0.44 &    ... &    ... \\
               &   0.15 &   0.25 &   0.25 &   0.26 &   0.17 &   0.25 &   0.26 &   0.34 &    ... &    ... \\
               &     17 &      1 &      1 &      1 &      2 &      1 &      1 &      4 &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0770   &  $-$1.43 &   0.32 &   0.04 &    ... &   0.33 &   0.17 &    ... &   0.21 &   0.35 &    ... \\
               &   0.15 &   0.24 &   0.08 &    ... &   0.13 &   0.24 &    ... &   0.16 &   0.24 &    ... \\
               &     26 &      1 &      4 &    ... &      2 &      1 &    ... &      7 &      1 &    ... \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0780   &  $-$1.42 &  $-$0.20 &  $-$0.13 &    ... &   0.21 &  $-$0.62 &  $-$0.30 &   0.21 &    ... &   0.15 \\
               &   0.15 &   0.31 &   0.09 &    ... &   0.29 &   0.31 &   0.32 &   0.16 &    ... &   0.33 \\
               &     31 &      1 &      2 &    ... &      2 &      1 &      1 &      7 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0812   &  $-$0.83 &    ... &  $-$0.04 &    ... &   0.90 &  $-$0.11 &    ... &   0.18 &    ... &  $-$0.40 \\
               &   0.15 &    ... &   0.25 &    ... &   0.48 &   0.25 &    ... &   0.49 &    ... &   0.27 \\
               &     21 &    ... &      1 &    ... &      2 &      1 &    ... &      2 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0825   &  $-$1.37 &   0.13 &  $-$0.02 &   0.17 &   0.24 &  $-$0.04 &  $-$0.20 &   0.10 &   0.02 &  $-$0.13 \\
               &   0.15 &   0.22 &   0.09 &   0.09 &   0.13 &   0.22 &   0.11 &   0.17 &   0.22 &   0.23 \\
               &     33 &      1 &      4 &      4 &      2 &      1 &      2 &      8 &      1 &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0840   &  $-$1.19 &   0.32 &   0.04 &  $-$0.47 &   0.45 &  $-$0.06 &  $-$0.67 &   0.18 &    ... &  $-$0.05 \\
               &   0.15 &   0.19 &   0.08 &   0.20 &   0.16 &   0.19 &   0.07 &   0.17 &    ... &   0.10 \\
               &     25 &      1 &      6 &      1 &      2 &      1 &      2 &      6 &    ... &      2 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0842   &  $-$1.39 &   0.30 &   0.50 &    ... &   0.26 &  $-$0.29 &    ... &   0.50 &    ... &  $-$0.66 \\
               &   0.15 &   0.21 &   0.20 &    ... &   0.16 &   0.21 &    ... &   0.19 &    ... &   0.22 \\
               &     21 &      1 &      1 &    ... &      2 &      1 &    ... &      4 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0880   &  $-$1.52 &   0.29 &   0.11 &   0.08 &   0.27 &  $-$0.08 &  $-$0.39 &   0.26 &   0.24 &  $-$0.11 \\
               &   0.14 &   0.17 &   0.06 &   0.09 &   0.11 &   0.17 &   0.08 &   0.16 &   0.17 &   0.19 \\
               &     33 &      1 &      8 &      5 &      2 &      1 &      4 &      5 &      1 &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0900   &  $-$1.57 &   0.34 &   0.09 &   0.00 &   0.43 &   0.02 &  $-$0.39 &   0.34 &   0.00 &   0.28 \\
               &   0.14 &   0.14 &   0.07 &   0.14 &   0.13 &   0.14 &   0.07 &   0.24 &   0.14 &   0.16 \\
               &     31 &      1 &      8 &      3 &      2 &      1 &      3 &      3 &      1 &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0902   &  $-$1.90 &  $-$0.38 &  $-$0.09 &    ... &   0.13 &    ... &  $-$0.25 &   0.22 &    ... &  $-$0.58 \\
               &   0.14 &   0.17 &   0.08 &    ... &   0.10 &    ... &   0.17 &   0.19 &    ... &   0.19 \\
               &     21 &      1 &      2 &    ... &      2 &    ... &      1 &      4 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0914   &  $-$2.09 &   0.42 &   0.22 &    ... &   0.08 &  $-$0.46 &    ... &  $-$0.01 &    ... &  $-$0.44 \\
               &   0.15 &   0.24 &   0.35 &    ... &   0.25 &   0.24 &    ... &   0.19 &    ... &   0.25 \\
               &     15 &      1 &      2 &    ... &      1 &      1 &    ... &      2 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0916   &  $-$1.37 &   0.08 &   0.50 &    ... &   0.85 &  $-$0.05 &    ... &   0.68 &    ... &   0.37 \\
               &   0.15 &   0.26 &   0.26 &    ... &   0.43 &   0.26 &    ... &   0.16 &    ... &   0.28 \\
               &     17 &      1 &      1 &    ... &      2 &      1 &    ... &      3 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0925   &  $-$1.35 &   0.62 &   0.57 &    ... &   0.90 &  $-$0.29 &    ... &   0.12 &    ... &   0.06 \\
               &   0.15 &   0.19 &   0.05 &    ... &   0.21 &   0.19 &    ... &   0.17 &    ... &   0.12 \\
               &     20 &      1 &      2 &    ... &      1 &      1 &    ... &      3 &    ... &      2 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0948   &  $-$1.95 &    ... &  $-$0.16 &    ... &   0.28 &  $-$0.32 &    ... &   0.21 &    ... &   0.48 \\
               &   0.15 &    ... &   0.20 &    ... &   0.22 &   0.21 &    ... &   0.24 &    ... &   0.10 \\
               &     22 &    ... &      1 &    ... &      1 &      1 &    ... &      2 &    ... &      2 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV0976   &  $-$1.29 &   0.06 &  $-$0.05 &   0.74 &    ... &   0.33 &    ... &   0.06 &    ... &  $-$0.14 \\
               &   0.15 &   0.24 &   0.23 &   0.24 &    ... &   0.24 &    ... &   0.27 &    ... &   0.25 \\
               &     14 &      1 &      1 &      1 &    ... &      1 &    ... &      1 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV1007   &  $-$1.43 &   0.37 &   0.19 &   0.27 &   0.31 &   0.18 &  $-$0.34 &   0.10 &    ... &   0.22 \\
               &   0.15 &   0.30 &   0.07 &   0.13 &   0.32 &   0.30 &   0.11 &   0.15 &    ... &   0.32 \\
               &     22 &      1 &      2 &      5 &      1 &      1 &      4 &      3 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV1009   &  $-$1.55 &   0.28 &   0.27 &    ... &   0.26 &   0.55 &  $-$0.39 &   0.41 &    ... &   0.56 \\
               &   0.15 &   0.26 &   0.04 &    ... &   0.28 &   0.26 &   0.27 &   0.16 &    ... &   0.28 \\
               &     32 &      1 &      6 &    ... &      1 &      1 &      1 &      3 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV1012   &  $-$1.63 &   0.44 &   0.15 &   0.27 &  $-$0.05 &   0.00 &    ... &   0.41 &   0.15 &  $-$0.01 \\
               &   0.15 &   0.21 &   0.09 &   0.22 &   0.12 &   0.21 &    ... &   0.17 &   0.21 &   0.11 \\
               &     27 &      1 &      5 &      1 &      2 &      1 &    ... &      5 &      1 &      2 \\
               &        &        &        &        &        &        &        &        &        &        \\
     MKV1061   &  $-$1.37 &   0.52 &   0.13 &   0.26 &   0.34 &  $-$0.07 &    ... &   0.28 &    ... &    ... \\
               &   0.15 &   0.27 &   0.27 &   0.08 &   0.17 &   0.27 &    ... &   0.18 &    ... &    ... \\
               &     28 &      1 &      1 &      2 &      2 &      1 &    ... &      6 &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        \\
\enddata
\tablenotetext{a}{For each object the three rows contain [Fe/H] and [X/Fe]; $\sigma_{\rm {Tot}}$; and the number of lines, respectively.}
\end{deluxetable}      


==> table12.tex <==
%Table 12

\begin{deluxetable}{rlrrrrrrrrrrrr}                                                                                                                   
\tablecolumns{14}                                                                                                                            
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{\label{tab:alphas_v2} {[$\alpha$/Fe]} Values and Errors\tablenotemark{a} for 30 Carina Red Giants}                  
\tablehead{                                                                                                                              
  \colhead{Name 1}   & {Name2}  & {[Fe/H]} & {$\sigma$Fe}   & {[Mg/Fe]} & {$\sigma$Mg}  & {[Si/Fe]} & {$\sigma$Si}  & {[Ca/Fe]} & {$\sigma$Ca}  & {[Ti/Fe]} & {$\sigma$Ti}  & {[$\alpha$/Fe]} & {$\sigma$[$\alpha$/Fe]} \\  
            {(1)}    & {(2)}    & {(3)}    & {(4)}          & {(5)}     & {(6)}         & {(7)}     & {(8)}         & {(9)}     & {(10)}        & {(11)}    & {(12)}        & {(13)}       & {(14)}   
  }                                                                                                                                       
\startdata 
CC06122   &  Car-484  &   $-$1.46  &    0.10  &    0.20  &    0.09  &    0.21  &    0.22  &    0.07  &    0.03  &    0.29  &    0.09  &      0.099  &   0.026  \\
CC06975   &           &   $-$1.84  &    0.14  &    0.27  &    0.05  &     ...  &     ...  &    0.14  &    0.06  &    0.17  &    0.18  &      0.215  &   0.038  \\
CC07452   &  Car-612  &   $-$1.33  &    0.10  &   $-$0.45  &    0.11  &     ...  &     ...  &   $-$0.27  &    0.03  &   $-$0.16  &    0.09  &     $-$0.272  &   0.030  \\
CC08447   &           &   $-$1.48  &    0.13  &    0.28  &    0.23  &    0.10  &    0.22  &    0.08  &    0.04  &    0.55  &    0.13  &      0.125  &   0.038  \\
CC08469   &  Car-705  &   $-$1.43  &    0.10  &    0.00  &    0.07  &    0.42  &    0.16  &    0.04  &    0.03  &    0.16  &    0.10  &      0.037  &   0.025  \\
CC08615   &           &   $-$1.73  &    0.11  &    0.52  &    0.24  &    0.56  &    0.24  &    0.18  &    0.05  &    0.05  &    0.25  &      0.189  &   0.048  \\
 CC8695   &  M12      &   $-$1.32  &    0.10  &    0.16  &    0.10  &    0.14  &    0.22  &    0.03  &    0.04  &    0.26  &    0.10  &      0.069  &   0.034  \\
CC08788   &           &   $-$1.48  &    0.13  &    0.26  &    0.14  &    0.06  &    0.24  &    0.14  &    0.07  &    0.05  &    0.10  &      0.132  &   0.053  \\
 CC9000   &  M3       &   $-$1.81  &    0.10  &   $-$0.31  &    0.05  &     ...  &     ...  &   $-$0.22  &    0.03  &    0.28  &    0.10  &     $-$0.210  &   0.024  \\
CC09179   &           &   $-$1.78  &    0.15  &    0.03  &    0.38  &    0.84  &    0.24  &   $-$0.14  &    0.08  &   $-$0.08  &    0.12  &     $-$0.117  &   0.066  \\
CC09225   &  Car-769  &   $-$1.65  &    0.10  &    0.38  &    0.06  &    0.28  &    0.16  &    0.10  &    0.05  &    0.39  &    0.12  &      0.243  &   0.035  \\
CC09226   &           &   $-$1.56  &    0.13  &    0.18  &    0.15  &    0.34  &    0.29  &    0.11  &    0.06  &    0.24  &    0.18  &      0.130  &   0.053  \\
CC09430   &           &   $-$2.13  &    0.15  &    0.75  &    0.22  &     ...  &     ...  &    0.14  &    0.09  &    0.37  &    0.21  &      0.247  &   0.077  \\
CC09633   &  Car-5070 &   $-$2.24  &    0.11  &   $-$0.17  &    0.17  &     ...  &     ...  &    0.01  &    0.07  &    0.03  &    0.14  &     $-$0.003  &   0.058  \\
CC09869   &           &   $-$1.26  &    0.15  &    0.19  &    0.04  &    0.13  &    0.14  &    0.06  &    0.06  &    0.29  &    0.23  &      0.153  &   0.033  \\
CC09929   &           &   $-$1.50  &    0.15  &    0.16  &    0.08  &    0.21  &    0.26  &    0.24  &    0.08  &    0.21  &    0.17  &      0.201  &   0.054  \\
CC10038   &           &   $-$1.30  &    0.15  &    0.24  &    0.25  &    0.33  &    0.18  &   $-$0.02  &    0.08  &    0.35  &    0.17  &      0.062  &   0.070  \\
CC10194   &           &   $-$1.42  &    0.15  &    0.15  &    0.14  &    0.18  &    0.27  &    0.01  &    0.08  &    0.23  &    0.16  &      0.074  &   0.064  \\
CC10318   &  M2       &   $-$1.53  &    0.10  &    0.15  &    0.05  &    0.31  &    0.16  &    0.06  &    0.04  &    0.33  &    0.09  &      0.114  &   0.029  \\
CC10414   &           &   $-$1.35  &    0.14  &    0.10  &    0.25  &    0.29  &    0.14  &    0.12  &    0.07  &    0.04  &    0.12  &      0.100  &   0.059  \\
CC10686   &           &   $-$1.68  &    0.13  &    0.30  &    0.19  &    0.24  &    0.21  &    0.07  &    0.03  &    0.32  &    0.16  &      0.084  &   0.029  \\
CC10944   &           &   $-$1.89  &    0.12  &    0.26  &    0.13  &    0.44  &    0.24  &    0.06  &    0.06  &    0.21  &    0.22  &      0.102  &   0.053  \\
CC11217   &           &   $-$1.28  &    0.14  &    0.09  &    0.12  &    0.11  &    0.15  &    0.04  &    0.04  &    0.36  &    0.11  &      0.079  &   0.036  \\
CC11560   &           &   $-$1.60  &    0.14  &    0.03  &    0.11  &     ...  &     ...  &    0.15  &    0.04  &    0.05  &    0.10  &      0.125  &   0.035  \\
CC12039   &  Car-1013 &   $-$1.56  &    0.09  &    0.18  &    0.06  &    0.22  &    0.17  &   $-$0.02  &    0.04  &    0.36  &    0.13  &      0.063  &   0.031  \\
          &  Car-524  &   $-$1.73  &    0.14  &    0.25  &    0.13  &    0.41  &    0.21  &   $-$0.01  &    0.05  &    0.03  &    0.13  &      0.024  &   0.044  \\
          &  Car-1087 &   $-$2.47  &    0.16  &    0.15  &    0.26  &     ...  &     ...  &   $-$0.45  &    0.15  &    0.53  &    0.28  &     $-$0.153  &   0.118  \\
          &  Car-7002 &   $-$2.68  &    0.15  &   $-$0.01  &    0.23  &     ...  &     ...  &   $-$0.02  &    0.11  &    0.45  &    0.23  &      0.055  &   0.091  \\
          &  M4       &   $-$1.49  &    0.14  &    0.20  &    0.17  &    0.11  &    0.18  &    0.04  &    0.04  &    0.25  &    0.10  &      0.075  &   0.036  \\
          &  M10      &   $-$1.99  &    0.14  &    0.01  &    0.09  &     ...  &     ...  &   $-$0.10  &    0.05  &    0.03  &    0.10  &     $-$0.057  &   0.040  \\

\enddata                                                                        
\tablenotetext{a} {The errors appear in the columns following the abundances; and the column header (e.g.) $\sigma$Mg stands for $\sigma$[Mg/Fe].} 
\end{deluxetable}      


==> table13.tex <==
% Table 13
\begin{deluxetable}{lccrr}                                                                                    
\tabletypesize{\scriptsize}                                                                                                   
\tablecolumns{5}                                                                                                       
\tablewidth{0pt}                                                                                                        
\tablecaption{\label{tab:iwamoto}Fraction of Type Ia Material, $\langle\Delta$[X$_{\rm i}$/Fe]$\rangle$, and [Ba/Fe] in the Carina Red Giants} 
\tablehead{                                                            
  \colhead   {Star} & {Iwamato Type\tablenotemark{a}}  & {Type Ia Fraction}  & {$\langle\Delta$[X$_{\rm i}$/Fe]$\rangle$}  & $\Delta$[Ba/Fe] \\  
  \colhead   {(1)}  & {(2)}                            & {(3)}                & {(4)}           & {(5)}      
  }
\startdata    
MKV0842     & TypeII   &   0.00   &  $-$0.07 &  $-$0.54 \\
CC10194     & WDD3     &   0.06   &  $-$0.19 &   0.25 \\
MKV0677     & TypeII   &   0.02   &  $-$0.10 &   0.05 \\
MKV0628     & TypeII   &   0.02   &  $-$0.12 &   0.03 \\
MKV0640     & WDD1     &   0.06   &  $-$0.02 &   0.44 \\
MKV0914     & TypeII   &   0.02   &  $-$0.12 &  $-$0.29 \\
MKV0925     & TypeII   &   0.00   &   0.28 &   0.19 \\
Car-7002\tablenotemark{b}    & ...      &    ...   &    ... &    ... \\
MKV0812\tablenotemark{b}     & ...      &    ...   &    ... &    ... \\
CC09869     & W70      &   0.06   &  $-$0.15 &   0.17 \\
MKV0780     & W70      &   0.22   &  $-$0.36 &   0.27 \\
MKV0976     & WDD1     &   0.14   &  $-$0.04 &   0.00 \\
CC11388\tablenotemark{b}     & ...      &    ...   &    ... &    ... \\
CC07452     & W70      &   0.40   &  $-$0.56 &  $-$0.54 \\
CC11560     & TypeII   &   0.02   &  $-$0.08 &   0.53 \\
CC12038     & TypeII   &   0.02   &  $-$0.05 &   0.23 \\
CC11217     & W70      &   0.06   &  $-$0.17 &   0.21 \\
MKV0596     & WDD3     &   0.17   &  $-$0.38 &  $-$0.21 \\
CC08447     & TypeII   &   0.04   &  $-$0.15 &   0.21 \\
CC09226     & WDD1     &   0.06   &  $-$0.14 &   0.55 \\
Car-524     & TypeII   &   0.02   &  $-$0.23 &   0.29 \\
Car-1087    & WDD3     &   0.12   &  $-$0.50 &  $-$0.68 \\
MKV0880     & TypeII   &   0.02   &  $-$0.14 &  $-$0.01 \\
CC10690     & WDD3     &   0.30   &  $-$0.39 &  $-$0.21 \\
CC10944     & TypeII   &   0.00   &  $-$0.10 &   0.30 \\
CC09179     & TypeII   &   0.02   &  $-$0.23 &   0.51 \\
CC09225     & TypeII   &   0.02   &  $-$0.02 &   0.26 \\
CC12039     & TypeII   &   0.02   &  $-$0.17 &   0.21 \\
MKV0698     & CDD2     &   0.08   &  $-$0.24 &    ... \\
CC10686     & TypeII   &   0.02   &  $-$0.16 &   0.37 \\
CC10802     & WDD2     &   0.10   &  $-$0.07 &   0.34 \\
MKV0740     & WDD3     &   0.58   &  $-$0.31 &    ... \\
MKV1061     & TypeII   &   0.00   &   0.00 &    ... \\
CC08695     & W70      &   0.06   &  $-$0.14 &   0.36 \\
MKV0948\tablenotemark{b}     & ...      &    ...   &    ... &    ... \\
CC06122     & TypeII   &   0.04   &  $-$0.16 &   0.50 \\
CC07889     & WDD1     &   0.10   &  $-$0.17 &  $-$0.51 \\
MKV1007     & TypeII   &   0.02   &  $-$0.06 &   0.33 \\
MKV0577     & WDD1     &   0.14   &   0.08 &   0.23 \\
MKV0743     & WDD3     &   0.54   &  $-$0.24 &    ... \\
CC06486     & TypeII   &   0.00   &  $-$0.28 &  $-$0.74 \\
M10         & WDD3     &   0.10   &  $-$0.25 &   0.53 \\
CC10414     & W70      &   0.08   &  $-$0.19 &  $-$0.13 \\
M4          & CDD2     &   0.06   &  $-$0.19 &   0.26 \\
CC08615     & TypeII   &   0.02   &  $-$0.07 &   0.36 \\
CC08788     & W7       &   0.06   &  $-$0.12 &   0.14 \\
CC09633     & W7       &   0.22   &  $-$0.35 &  $-$0.66 \\
CC09507     & CDD1     &   0.28   &  $-$0.31 &   0.61 \\
CC09000     & WDD3     &   0.14   &  $-$0.41 &   0.41 \\
CC09929     & TypeII   &   0.04   &  $-$0.03 &   0.50 \\
CC10318     & W70      &   0.06   &  $-$0.15 &   0.33 \\
MKV0458     & W70      &   0.04   &   0.09 &   0.37 \\
MKV0397\tablenotemark{b}     & ...      &    ...   &    ... &    ... \\
CC10038     & TypeII   &   0.02   &  $-$0.13 &   0.14 \\
CC09430     & WDD1     &   0.10   &  $-$0.03 &   0.05 \\
MKV0916     & TypeII   &   0.04   &   0.19 &   0.49 \\
CC06975     & CDD1     &   0.04   &  $-$0.03 &   0.49 \\
CC08469     & W70      &   0.06   &  $-$0.22 &   0.14 \\
MKV0729     & TypeII   &   0.02   &   0.08 &   0.29 \\
MKV0556     & TypeII   &   0.02   &  $-$0.02 &   0.59 \\
MKV0733     & W7       &   0.16   &  $-$0.19 &   0.15 \\
MKV0614\tablenotemark{b}     & ...      &    ...   &    ... &    ... \\
MKV0708\tablenotemark{b}     & ...      &    ...   &    ... &    ... \\
\enddata
\tablenotetext{a}{Admixed \citet{iwamoto99} Type Ia supernova. ``Type II'' implies zero Type Ia}
\tablenotetext{b}{Insufficient information: too few elements observable}
\end{deluxetable}      


==> table14.tex <==
% Table 14

\begin{deluxetable}{cllcc}                                                                                    
\tabletypesize{\scriptsize}                                                                                                   
\tablecolumns{5}                                                                                                       
\tablewidth{0pt}                                                                                                        
\tablecaption{\label{tab:appendix} Cross-identification and Coordinates of Program Stars}                          
\tablehead{                                                                                                                              
  \colhead{This work\tablenotemark{a}} & {Venn et al.\tablenotemark{a}}  & {Shetrone et al.\tablenotemark{a}}  & {Lemasle et al.\tablenotemark{a}} & {RA (2000) Dec} \\   
  \colhead   {(1)}    & {(2)}          & {(3)}              & {(4)}            & {(5)}       
  }
\startdata    
          &           &           & MKV0842   & 06 40 22.51  $-$50 59 01.9 \\
CC10194   &           &           &           & 06 40 30.82  $-$50 59 15.0 \\
          &           &           & MKV0677   & 06 40 31.12  $-$50 55 24.5 \\
          &           &           & MKV0628   & 06 40 35.37  $-$50 54 07.6 \\
          &           &           & MKV0640   & 06 40 40.82  $-$50 54 29.2 \\
          &           &           & MKV0914   & 06 40 42.49  $-$51 00 42.7 \\
          &           &           & MKV0925   & 06 40 43.17  $-$51 01 06.6 \\
          & Car-7002  &           &           & 06 40 49.15  $-$51 00 32.9 \\
          &           &           & MKV0812   & 06 40 51.62  $-$50 58 21.7 \\
CC09869   &           &           & MKV0825   & 06 40 56.95  $-$50 58 38.2 \\
          &           &           & MKV0780   & 06 40 57.09  $-$50 57 44.3 \\
          &           &           & MKV0976   & 06 40 57.68  $-$51 02 40.7 \\
CC11388   &           &           &           & 06 40 58.04  $-$51 02 00.0 \\
CC07452   & Car-612   &           &           & 06 40 58.47  $-$50 53 35.2 \\
CC11560   &           &           & MKV1009   & 06 40 59.29  $-$51 02 26.4 \\
CC12038   &           &           & MKV1012   & 06 41 00.31  $-$51 03 42.9 \\
CC11217   &           &           &           & 06 41 05.01  $-$51 01 35.8 \\
          &           &           & MKV0596   & 06 41 05.35  $-$51 05 25.5 \\
CC08447   &           &           &           & 06 41 10.54  $-$50 55 52.8 \\
CC09226   &           &           & MKV0770   & 06 41 12.29  $-$50 57 25.8 \\
          & Car-524   &           &           & 06 41 14.68  $-$50 51 09.7 \\
          & Car-1087  &           &           & 06 41 15.45  $-$51 01 16.0 \\
          &           &           & MKV0880   & 06 41 15.66  $-$50 59 47.9 \\
CC10690   &           &           & MKV0902   & 06 41 16.30  $-$51 00 18.5 \\
CC10944   &           &           &           & 06 41 16.75  $-$51 00 53.8 \\
CC09179   &           &           &           & 06 41 17.92  $-$50 57 20.3 \\
CC09225   & Car-769   &           &           & 06 41 19.69  $-$50 57 25.4 \\
CC12039   & Car-1013  &           &           & 06 41 21.97  $-$51 03 43.1 \\
          &           &           & MKV0698   & 06 41 26.09  $-$50 55 43.7 \\
CC10686   &           &           & MKV0900   & 06 41 27.18  $-$51 00 18.2 \\
CC10802   &           &           &           & 06 41 27.53  $-$51 00 34.7 \\
          &           &           & MKV0740   & 06 41 29.08  $-$50 56 46.5 \\
          &           &           & MKV1061   & 06 41 29.15  $-$51 05 22.3 \\
CC08695   &           & M12       &           & 06 41 36.47  $-$50 56 23.2 \\
          &           &           & MKV0948   & 06 41 37.65  $-$51 01 43.7 \\
CC06122   & Car-484   &           &           & 06 41 39.62  $-$50 49 58.8 \\
CC07889   &           &           & MKV0652   & 06 41 40.83  $-$50 54 45.7 \\
          &           &           & MKV1007   & 06 41 44.63  $-$51 03 31.1 \\
          &           &           & MKV0577   & 06 41 45.03  $-$50 52 49.0 \\
          &           &           & MKV0743   & 06 41 45.91  $-$50 56 54.3 \\
CC06486   &           &           & MKV0514   & 06 41 45.99  $-$50 51 00.6 \\
          &           & M10       &           & 06 41 46.34  $-$51 01 22.5 \\
CC10414   &           &           &           & 06 41 47.62  $-$50 59 44.0 \\
          &           & M4        &           & 06 41 48.20  $-$50 55 01.4 \\
CC08615   &           &           &           & 06 41 49.58  $-$50 56 11.3 \\
CC08788   &           &           &           & 06 41 50.09  $-$50 56 35.0 \\
CC09633   & Car-5070  &           &           & 06 41 53.83  $-$50 58 10.9 \\
CC09507   &           &           &           & 06 41 54.07  $-$50 57 56.6 \\
CC09000   &           & M3        &           & 06 41 54.58  $-$50 57 00.6 \\
CC09929   &           &           &           & 06 41 54.83  $-$50 58 46.8 \\
CC10318   &           & M2        &           & 06 41 57.62  $-$50 59 32.5 \\
          &           &           & MKV0458   & 06 41 58.19  $-$50 48 58.0 \\
          &           &           & MKV0397   & 06 41 58.27  $-$50 46 41.4 \\
CC10038   &           &           & MKV0840   & 06 42 02.79  $-$50 58 59.2 \\
CC09430   &           &           &           & 06 42 05.37  $-$50 57 48.2 \\
          &           &           & MKV0916   & 06 42 08.97  $-$51 00 48.0 \\
CC06975   &           &           &           & 06 42 10.84  $-$50 52 20.4 \\
CC08469   & Car-705   &           &           & 06 42 17.39  $-$50 55 55.0 \\
          &           &           & MKV0729   & 06 42 17.45  $-$50 56 26.3 \\
          &           &           & MKV0556   & 06 42 22.26  $-$50 52 09.5 \\
          &           &           & MKV0733   & 06 42 30.38  $-$50 56 33.3 \\
          &           &           & MKV0614   & 06 42 37.95  $-$50 53 37.6 \\
          &           &           & MKV0708   & 06 42 38.52  $-$50 56 00.8 \\
\enddata
\tablenotetext{a}{The headers in Columns 1 -- 4 refer to the present work, \citet{venn12}, \citet{shetrone03}, and \citet{lemasle12}, respectively.}
\end{deluxetable}      


==> table15.tex <==
% Table 15
\begin{deluxetable}{lrrrrrrrrrrrrrrrrrrr}                                                                                    
\tabletypesize{\tiny}                                                                                                   
\tablecolumns{20}                                                                                                       
\tablewidth{0pt}                                                                                                        
\rotate                                                                                                                 
\tablecaption{\label{tab:relabs_aver} Average [Fe/H], [X/Fe], and Errors\tablenotemark{a} for the 63 Independent Carina Red Giants}                          
\tablehead{                                                                                                                              
  \colhead{Object\tablenotemark{b}} & {[Fe/H]} & {O}  & {Na} & {Mg} & {Si} & {Ca} & {Sc} & {Ti} & {V} & {Cr} & {Mn} & {Fe~II} & {Co} & {Ni} & {Cu} & {Ba} & {La} & {Nd} & {Eu}\\  
  }
\startdata    
MKV0842  & $-$1.39 &   ... &   ... &  0.30 &   ... &  0.50 &   ... &  0.26 &   ... & $-$0.29 &   ... &  0.50 &   ... &   ... &   ... & $-$0.66 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.21 &   ... &  0.20 &   ... &  0.16 &   ... &  0.21 &   ... &  0.19 &   ... &   ... &   ... &  0.22 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC10194  & $-$1.42 &  0.17 & $-$0.31 &  0.15 &  0.18 &  0.01 & $-$0.27 &  0.22 & $-$0.25 &  0.00 & $-$0.90 & $-$0.01 &   ... & $-$0.25 &   ... &  0.13 &  0.24 & $-$0.31 &   ... \\       
         &  0.15 &  0.27 &  0.24 &  0.14 &  0.27 &  0.08 &  0.15 &  0.12 &  0.19 &  0.23 &  0.17 &  0.21 &   ... &  0.12 &   ... &  0.22 &  0.26 &  0.25 &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0677  & $-$1.66 &   ... &   ... &  0.33 &   ... &  0.12 &   ... &  0.24 &   ... &  0.19 & $-$0.41 &  0.18 &   ... &   ... &   ... & $-$0.05 &   ... &   ... &   ... \\       
         &  0.14 &   ... &   ... &  0.19 &   ... &  0.06 &   ... &  0.09 &   ... &  0.19 &  0.09 &  0.16 &   ... &   ... &   ... &  0.10 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0628  & $-$1.71 &   ... &   ... &  0.41 &   ... &  0.09 &   ... &  0.25 &   ... &  0.03 &   ... &  0.35 &   ... &   ... &   ... & $-$0.07 &   ... &   ... &   ... \\       
         &  0.14 &   ... &   ... &  0.21 &   ... &  0.08 &   ... &  0.11 &   ... &  0.15 &   ... &  0.16 &   ... &   ... &   ... &  0.22 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0640  & $-$1.85 &   ... &   ... &  0.34 &   ... &  0.19 &  0.52 &  0.49 &   ... &  0.16 & $-$0.16 &  0.32 &   ... &   ... &   ... &  0.34 &  1.09 &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.24 &   ... &  0.05 &  0.25 &  0.09 &   ... &  0.11 &  0.13 &  0.17 &   ... &   ... &   ... &  0.25 &  0.25 &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0914  & $-$2.09 &   ... &   ... &  0.42 &   ... &  0.22 &   ... &  0.08 &   ... & $-$0.46 &   ... & $-$0.01 &   ... &   ... &   ... & $-$0.44 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.24 &   ... &  0.35 &   ... &  0.25 &   ... &  0.24 &   ... &  0.19 &   ... &   ... &   ... &  0.25 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0925  & $-$1.35 &   ... &   ... &  0.62 &   ... &  0.57 &   ... &  0.90 &   ... & $-$0.29 &   ... &  0.12 &   ... &   ... &   ... &  0.06 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.19 &   ... &  0.05 &   ... &  0.21 &   ... &  0.19 &   ... &  0.17 &   ... &   ... &   ... &  0.12 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
Car$-$7002 & $-$2.68 &   ... &   ... & $-$0.01 &   ... & $-$0.02 &   ... &  0.45 &   ... &   ... &   ... &   ... &   ... &   ... &   ... & $-$0.84 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.23 &   ... &  0.11 &   ... &  0.23 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  0.17 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0812  & $-$0.83 &   ... &   ... &   ... &   ... & $-$0.04 &   ... &  0.90 &   ... & $-$0.11 &   ... &  0.18 &   ... &   ... &   ... & $-$0.40 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &   ... &   ... &  0.25 &   ... &  0.48 &   ... &  0.25 &   ... &  0.49 &   ... &   ... &   ... &  0.27 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC09869  & $-$1.32 &   ... & $-$0.19 &  0.19 &  0.13 &  0.04 &  0.14 &  0.15 & $-$0.28 &  0.02 & $-$0.30 &  0.10 &   ... & $-$0.10 &   ... &  0.04 &  0.48 &   ... &   ... \\       
MKV0825  &  0.11 &   ... &  0.22 &  0.04 &  0.14 &  0.05 &  0.14 &  0.06 &  0.16 &  0.11 &  0.06 &  0.12 &   ... &  0.08 &   ... &  0.14 &  0.11 &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0780  & $-$1.42 &   ... &   ... & $-$0.20 &   ... & $-$0.13 &   ... &  0.21 &   ... & $-$0.62 & $-$0.30 &  0.21 &   ... &   ... &   ... &  0.15 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.31 &   ... &  0.09 &   ... &  0.29 &   ... &  0.31 &  0.32 &  0.16 &   ... &   ... &   ... &  0.33 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0976  & $-$1.29 &   ... &   ... &  0.06 &   ... & $-$0.05 &   ... &  0.74 &   ... &  0.33 &   ... &  0.06 &   ... &   ... &   ... & $-$0.14 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.24 &   ... &  0.23 &   ... &  0.24 &   ... &  0.24 &   ... &  0.27 &   ... &   ... &   ... &  0.25 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC11388  & $-$1.52 &   ... &   ... &  0.52 &   ... &  0.08 &   ... &   ... &   ... &   ... &   ... &   ... &   ... & $-$0.04 &   ... &  0.02 &   ... &   ... &   ... \\       
         &  0.14 &   ... &   ... &  0.25 &   ... &  0.15 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  0.25 &   ... &  0.14 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC07452  & $-$1.33 &   ... & $-$0.69 & $-$0.45 &   ... & $-$0.27 & $-$0.62 & $-$0.22 & $-$0.63 & $-$0.14 & $-$0.36 &  0.27 &   ... & $-$0.35 &   ... & $-$0.67 &   ... & $-$0.34 &   ... \\       
Car$-$612  &  0.10 &   ... &  0.19 &  0.11 &   ... &  0.03 &  0.12 &  0.07 &  0.16 &  0.08 &  0.07 &  0.12 &   ... &  0.05 &   ... &  0.10 &   ... &  0.22 &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC11560  & $-$1.58 &  0.58 &  0.25 &  0.07 &   ... &  0.21 &  0.16 &  0.18 &  0.33 & $-$0.03 & $-$0.28 &  0.39 &   ... & $-$0.06 &   ... &  0.43 &  0.89 &   ... &   ... \\       
MKV1009  &  0.10 &  0.24 &  0.21 &  0.10 &   ... &  0.03 &  0.18 &  0.08 &  0.39 &  0.12 &  0.18 &  0.12 &   ... &  0.17 &   ... &  0.18 &  0.23 &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC12038  & $-$1.56 &   ... & $-$0.25 &  0.43 &  0.55 &  0.15 & $-$0.10 &  0.14 &   ... & $-$0.10 & $-$0.25 &  0.31 &   ... & $-$0.11 &   ... &  0.13 &  0.59 &   ... &   ... \\       
MKV1012  &  0.11 &   ... &  0.24 &  0.16 &  0.44 &  0.06 &  0.13 &  0.09 &   ... &  0.16 &  0.24 &  0.12 &   ... &  0.08 &   ... &  0.09 &  0.25 &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC11217  & $-$1.28 &  0.28 & $-$0.23 &  0.09 &  0.11 &  0.04 & $-$0.04 &  0.23 & $-$0.13 & $-$0.12 & $-$0.31 &  0.14 & $-$0.41 & $-$0.11 &   ... &  0.07 &  0.12 &   ... &  0.44 \\       
         &  0.14 &  0.21 &  0.17 &  0.12 &  0.15 &  0.04 &  0.14 &  0.07 &  0.13 &  0.12 &  0.06 &  0.16 &  0.18 &  0.07 &   ... &  0.11 &  0.13 &   ... &  0.20 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0596  & $-$1.58 &   ... &   ... & $-$0.08 &   ... & $-$0.22 &   ... &  0.18 &   ... &  0.12 & $-$0.22 &  0.06 &   ... &   ... &   ... & $-$0.31 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.25 &   ... &  0.06 &   ... &  0.09 &   ... &  0.25 &  0.07 &  0.16 &   ... &   ... &   ... &  0.16 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC08447  & $-$1.48 &   ... & $-$0.21 &  0.28 &  0.10 &  0.08 &  0.01 &  0.29 &  0.02 & $-$0.07 & $-$0.29 &  0.32 &   ... & $-$0.27 & $-$0.48 &  0.11 &   ... &   ... &   ... \\       
         &  0.13 &   ... &  0.20 &  0.23 &  0.22 &  0.04 &  0.16 &  0.08 &  0.16 &  0.10 &  0.14 &  0.19 &   ... &  0.09 &  0.20 &  0.14 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC09226  & $-$1.50 &  0.45 & $-$0.22 &  0.22 &  0.34 &  0.08 &  0.10 &  0.30 &  0.58 & $-$0.01 & $-$0.17 &  0.18 &   ... & $-$0.06 &   ... &  0.45 &  1.15 &   ... &   ... \\       
MKV0770  &  0.10 &  0.27 &  0.26 &  0.13 &  0.29 &  0.05 &  0.16 &  0.11 &  0.19 &  0.11 &  0.25 &  0.12 &   ... &  0.07 &   ... &  0.21 &  0.26 &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
Car$-$524  & $-$1.73 &  0.47 &   ... &  0.25 &  0.41 & $-$0.01 & $-$0.02 &  0.04 & $-$0.03 & $-$0.05 & $-$0.37 &  0.17 &   ... & $-$0.02 &   ... &  0.19 &  0.61 &  0.44 &   ... \\       
         &  0.14 &  0.21 &   ... &  0.13 &  0.21 &  0.05 &  0.13 &  0.10 &  0.19 &  0.14 &  0.11 &  0.16 &   ... &  0.06 &   ... &  0.20 &  0.11 &  0.19 &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
Car$-$1087 & $-$2.47 &   ... &   ... &  0.15 &   ... & $-$0.45 &  0.06 &  0.53 &   ... & $-$0.51 &   ... &   ... &   ... &   ... &   ... & $-$1.07 &   ... &   ... &   ... \\       
         &  0.16 &   ... &   ... &  0.26 &   ... &  0.15 &  0.16 &  0.28 &   ... &  0.26 &   ... &   ... &   ... &   ... &   ... &  0.28 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0880  & $-$1.52 &   ... &   ... &  0.29 &  0.51 &  0.11 &   ... &  0.16 &   ... & $-$0.08 & $-$0.39 &  0.26 &   ... &  0.24 &   ... & $-$0.11 &   ... &   ... &  0.52 \\       
         &  0.14 &   ... &   ... &  0.17 &  0.20 &  0.06 &   ... &  0.07 &   ... &  0.17 &  0.08 &  0.16 &   ... &  0.17 &   ... &  0.19 &   ... &   ... &  0.21 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC10690  & $-$1.93 &   ... &   ... & $-$0.40 &   ... & $-$0.17 & $-$0.27 &  0.15 &   ... & $-$0.39 & $-$0.25 &  0.29 &   ... & $-$0.37 &   ... & $-$0.31 &   ... &   ... &   ... \\       
MKV0902  &  0.10 &   ... &   ... &  0.13 &   ... &  0.05 &  0.21 &  0.09 &   ... &  0.12 &  0.17 &  0.12 &   ... &  0.13 &   ... &  0.10 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC10944  & $-$1.89 &   ... &   ... &  0.26 &  0.44 &  0.06 & $-$0.01 &  0.32 &  0.27 & $-$0.06 & $-$0.47 &  0.30 &   ... & $-$0.01 &   ... &  0.20 &   ... &   ... &   ... \\       
         &  0.12 &   ... &   ... &  0.13 &  0.24 &  0.06 &  0.16 &  0.16 &  0.34 &  0.09 &  0.09 &  0.16 &   ... &  0.06 &   ... &  0.12 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC09179  & $-$1.78 &   ... &   ... &  0.03 &  0.84 & $-$0.14 & $-$0.22 & $-$0.08 &  0.29 & $-$0.13 &   ... &  0.31 &   ... & $-$0.28 &   ... &  0.41 &   ... &   ... &  0.95 \\       
         &  0.15 &   ... &   ... &  0.38 &  0.24 &  0.08 &  0.17 &  0.12 &  0.22 &  0.12 &   ... &  0.16 &   ... &  0.10 &   ... &  0.16 &   ... &   ... &  0.25 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC09225  & $-$1.65 &  0.56 & $-$0.19 &  0.38 &  0.28 &  0.10 &  0.15 &  0.34 &  0.10 & $-$0.21 & $-$0.26 &  0.25 &  0.08 &  0.03 &   ... &  0.16 &  0.76 &  0.23 &   ... \\       
Car$-$769  &  0.10 &  0.16 &  0.14 &  0.06 &  0.16 &  0.05 &  0.10 &  0.07 &  0.13 &  0.09 &  0.08 &  0.12 &  0.19 &  0.05 &   ... &  0.09 &  0.15 &  0.15 &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC12039  & $-$1.56 &  0.50 & $-$0.17 &  0.18 &  0.22 & $-$0.02 &  0.08 &  0.23 & $-$0.01 &  0.08 & $-$0.36 &  0.15 &  0.14 & $-$0.08 &   ... &  0.11 &   ... &  0.40 &  0.54 \\       
Car$-$1013 &  0.09 &  0.21 &  0.16 &  0.06 &  0.17 &  0.04 &  0.10 &  0.07 &  0.11 &  0.04 &  0.06 &  0.12 &  0.35 &  0.05 &   ... &  0.08 &   ... &  0.35 &  0.17 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0698  & $-$1.30 &   ... &   ... &  0.12 &   ... &  0.03 &   ... &  0.05 &   ... &  0.11 & $-$0.28 &  0.17 &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.21 &   ... &  0.06 &   ... &  0.07 &   ... &  0.21 &  0.07 &  0.17 &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC10686  & $-$1.63 &  0.56 & $-$0.21 &  0.33 &  0.24 &  0.07 &  0.13 &  0.18 & $-$0.29 & $-$0.14 & $-$0.44 &  0.22 &  0.07 & $-$0.05 & $-$0.64 &  0.27 &  0.38 &   ... &  0.44 \\       
MKV0900  &  0.10 &  0.21 &  0.19 &  0.11 &  0.21 &  0.03 &  0.14 &  0.06 &  0.15 &  0.07 &  0.06 &  0.13 &  0.19 &  0.06 &  0.19 &  0.10 &  0.15 &   ... &  0.21 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC10802  & $-$1.27 &   ... & $-$0.50 & $-$0.05 &  0.45 &  0.13 & $-$0.09 &  0.41 & $-$0.16 &  0.09 & $-$0.30 &  0.42 &  0.42 & $-$0.11 &   ... &  0.19 &   ... &   ... &   ... \\       
         &  0.14 &   ... &  0.24 &  0.43 &  0.25 &  0.13 &  0.13 &  0.21 &  0.11 &  0.20 &  0.22 &  0.20 &  0.23 &  0.17 &   ... &  0.25 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0740  & $-$0.97 &   ... &   ... & $-$0.81 &   ... & $-$0.58 &   ... &  0.25 &   ... & $-$0.56 & $-$0.34 &  0.42 &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.23 &   ... &  0.22 &   ... &  0.11 &   ... &  0.23 &  0.23 &  0.16 &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV1061  & $-$1.37 &   ... &   ... &  0.52 &   ... &  0.13 &   ... &  0.27 &   ... & $-$0.07 &   ... &  0.28 &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.27 &   ... &  0.27 &   ... &  0.07 &   ... &  0.27 &   ... &  0.18 &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC08695  & $-$1.32 &  0.34 & $-$0.36 &  0.16 &  0.22 &  0.03 & $-$0.01 &  0.09 & $-$0.19 & $-$0.18 & $-$0.45 &  0.22 & $-$0.27 & $-$0.17 & $-$0.69 &  0.22 &  0.30 &  0.18 &  0.39 \\       
M12      &  0.10 &  0.15 &  0.12 &  0.10 &  0.14 &  0.04 &  0.11 &  0.06 &  0.16 &  0.10 &  0.06 &  0.12 &  0.21 &  0.08 &  0.13 &  0.07 &  0.13 &  0.13 &  0.14 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0948  & $-$1.95 &   ... &   ... &   ... &   ... & $-$0.16 &   ... &  0.28 &   ... & $-$0.32 &   ... &  0.21 &   ... &   ... &   ... &  0.48 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &   ... &   ... &  0.20 &   ... &  0.22 &   ... &  0.21 &   ... &  0.24 &   ... &   ... &   ... &  0.10 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC06122  & $-$1.46 &  0.41 & $-$0.27 &  0.20 &  0.21 &  0.07 &  0.11 &  0.20 & $-$0.07 & $-$0.03 & $-$0.35 &  0.11 & $-$0.03 & $-$0.07 & $-$0.63 &  0.40 &  0.50 &  0.67 &  0.51 \\       
Car$-$484  &  0.10 &  0.15 &  0.14 &  0.09 &  0.22 &  0.03 &  0.10 &  0.05 &  0.08 &  0.07 &  0.05 &  0.11 &  0.19 &  0.06 &  0.19 &  0.12 &  0.08 &  0.20 &  0.22 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC07889  & $-$2.30 &   ... &   ... &  0.49 &   ... &  0.10 &  0.12 &  0.53 &   ... & $-$0.46 &   ... &  0.37 &   ... &  0.43 &   ... & $-$0.79 &   ... &   ... &   ... \\       
MKV0652  &  0.10 &   ... &   ... &  0.17 &   ... &  0.08 &  0.24 &  0.14 &   ... &  0.13 &   ... &  0.21 &   ... &  0.23 &   ... &  0.12 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV1007  & $-$1.43 &   ... &   ... &  0.37 &   ... &  0.19 &   ... &  0.28 &   ... &  0.18 & $-$0.34 &  0.10 &   ... &   ... &   ... &  0.22 &  0.74 &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.30 &   ... &  0.07 &   ... &  0.12 &   ... &  0.30 &  0.11 &  0.15 &   ... &   ... &   ... &  0.32 &  0.32 &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0577  & $-$1.61 &   ... &   ... & $-$0.13 &   ... &  0.50 &   ... &  0.53 &   ... & $-$0.07 &   ... &  0.77 &   ... &   ... &   ... &  0.13 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.29 &   ... &  0.29 &   ... &  0.22 &   ... &  0.29 &   ... &  0.33 &   ... &   ... &   ... &  0.31 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0743  & $-$0.64 &   ... &   ... & $-$0.84 &   ... & $-$0.50 &   ... &  0.28 &   ... & $-$0.31 & $-$0.51 &  0.44 &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.25 &   ... &  0.25 &   ... &  0.14 &   ... &  0.25 &  0.26 &  0.34 &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC06486  & $-$2.07 &   ... &  0.19 &  0.19 &   ... &  0.09 &  0.14 &  0.15 &   ... & $-$0.15 & $-$0.40 &  0.41 &   ... &  0.08 &   ... & $-$0.88 &   ... &   ... &   ... \\       
MKV0514  &  0.11 &   ... &  0.28 &  0.11 &   ... &  0.06 &  0.29 &  0.14 &   ... &  0.11 &  0.23 &  0.18 &   ... &  0.11 &   ... &  0.10 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
M10      & $-$1.99 &  0.39 &   ... &  0.01 &   ... & $-$0.10 &  0.27 &  0.03 &   ... & $-$0.11 & $-$0.44 &  0.29 &   ... &   ... &   ... &  0.43 &  0.70 &  0.81 &  1.17 \\       
         &  0.14 &  0.20 &   ... &  0.09 &   ... &  0.05 &  0.19 &  0.10 &   ... &  0.16 &  0.07 &  0.16 &   ... &   ... &   ... &  0.11 &  0.12 &  0.17 &  0.20 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC10414  & $-$1.35 &  0.57 & $-$0.76 &  0.10 &  0.29 &  0.12 &  0.00 &  0.07 & $-$0.04 & $-$0.22 & $-$0.32 &  0.11 &   ... & $-$0.13 & $-$0.32 & $-$0.26 &  0.34 &  0.36 &  0.62 \\       
         &  0.14 &  0.26 &  0.24 &  0.25 &  0.14 &  0.07 &  0.18 &  0.07 &  0.34 &  0.18 &  0.15 &  0.17 &   ... &  0.09 &  0.23 &  0.21 &  0.25 &  0.24 &  0.25 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
M4       & $-$1.49 &  0.43 & $-$0.31 &  0.20 &  0.11 &  0.04 & $-$0.22 &  0.15 &   ... &  0.07 & $-$0.36 &  0.07 &   ... & $-$0.04 & $-$0.64 &  0.16 &  0.35 &  0.42 &  0.39 \\       
         &  0.14 &  0.19 &  0.16 &  0.17 &  0.18 &  0.04 &  0.18 &  0.08 &   ... &  0.15 &  0.07 &  0.16 &   ... &  0.15 &  0.17 &  0.11 &  0.11 &  0.17 &  0.19 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC08615  & $-$1.73 &  0.55 & $-$0.06 &  0.52 &  0.56 &  0.18 &  0.05 &  0.25 &   ... & $-$0.19 &   ... &  0.38 &   ... &  0.14 &   ... &  0.26 &  0.64 &   ... &   ... \\       
         &  0.11 &  0.24 &  0.23 &  0.24 &  0.24 &  0.05 &  0.24 &  0.18 &   ... &  0.04 &   ... &  0.16 &   ... &  0.15 &   ... &  0.33 &  0.24 &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC08788  & $-$1.48 &   ... & $-$0.13 &  0.26 &  0.06 &  0.14 &  0.36 &  0.08 &  0.39 & $-$0.19 &  0.01 &  0.33 &   ... &  0.01 &   ... &  0.04 &   ... &   ... &  0.80 \\       
         &  0.13 &   ... &  0.24 &  0.14 &  0.24 &  0.07 &  0.21 &  0.10 &  0.29 &  0.07 &  0.11 &  0.17 &   ... &  0.13 &   ... &  0.13 &   ... &   ... &  0.25 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC09633  & $-$2.24 &   ... &   ... & $-$0.17 &   ... &  0.01 &  0.39 &  0.03 &   ... & $-$0.47 &  0.21 &  0.48 &   ... &  0.04 &   ... & $-$0.91 &   ... &   ... &   ... \\       
Car$-$5070 &  0.11 &   ... &   ... &  0.17 &   ... &  0.07 &  0.13 &  0.14 &   ... &  0.03 &  0.24 &  0.14 &   ... &  0.14 &   ... &  0.18 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC09507  & $-$1.72 &   ... &   ... & $-$0.12 &   ... & $-$0.11 & $-$0.08 & $-$0.14 &  0.51 &  0.17 &  0.24 &  0.20 &   ... & $-$0.27 &   ... &  0.51 &  0.72 &  0.31 &   ... \\       
         &  0.12 &   ... &   ... &  0.07 &   ... &  0.06 &  0.19 &  0.24 &  0.23 &  0.13 &  0.23 &  0.16 &   ... &  0.10 &   ... &  0.13 &  0.24 &  0.24 &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC09000  & $-$1.81 &  0.43 &   ... & $-$0.31 &   ... & $-$0.22 & $-$0.31 &  0.08 & $-$0.18 & $-$0.14 & $-$0.46 &  0.40 &   ... & $-$0.21 &   ... &  0.31 &  0.41 &  0.56 &  0.85 \\       
M3       &  0.10 &  0.19 &   ... &  0.05 &   ... &  0.03 &  0.12 &  0.06 &  0.33 &  0.08 &  0.05 &  0.11 &   ... &  0.06 &   ... &  0.08 &  0.10 &  0.12 &  0.14 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC09929  & $-$1.50 &  0.76 & $-$0.39 &  0.16 &  0.21 &  0.24 &  0.20 &  0.21 &  0.16 &  0.00 & $-$0.32 &  0.29 &   ... &  0.03 &   ... &  0.40 &  0.73 &   ... &  0.85 \\       
         &  0.15 &  0.26 &  0.24 &  0.08 &  0.26 &  0.08 &  0.22 &  0.17 &  0.11 &  0.10 &  0.16 &  0.19 &   ... &  0.10 &   ... &  0.14 &  0.12 &   ... &  0.26 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC10318  & $-$1.53 &  0.58 & $-$0.46 &  0.15 &  0.22 &  0.06 &  0.26 &  0.26 & $-$0.31 & $-$0.06 & $-$0.36 &  0.13 &  0.03 & $-$0.07 &   ... &  0.23 &  0.35 &  0.31 &  0.26 \\       
M2       &  0.10 &  0.15 &  0.17 &  0.05 &  0.12 &  0.04 &  0.11 &  0.07 &  0.21 &  0.09 &  0.06 &  0.12 &  0.13 &  0.07 &   ... &  0.12 &  0.11 &  0.13 &  0.20 \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0458  & $-$1.47 &   ... &   ... &  0.07 &   ... &  0.33 &   ... &  0.32 &   ... & $-$0.17 & $-$0.48 &  0.40 &   ... &  0.47 &   ... &  0.27 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.24 &   ... &  0.31 &   ... &  0.07 &   ... &  0.24 &  0.24 &  0.16 &   ... &  0.24 &   ... &  0.12 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0397  & $-$2.02 &   ... &   ... &   ... &   ... &  0.44 &   ... &  0.21 &   ... & $-$0.62 &   ... &  0.24 &   ... &   ... &   ... & $-$0.88 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &   ... &   ... &  0.26 &   ... &  0.12 &   ... &  0.26 &   ... &  0.17 &   ... &   ... &   ... &  0.28 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC10038  & $-$1.25 &  0.54 & $-$0.29 &  0.29 &  0.33 &  0.01 &  0.02 &  0.14 & $-$0.15 & $-$0.03 & $-$0.61 &  0.12 & $-$0.04 & $-$0.20 &   ... & $-$0.01 &  0.57 &   ... &   ... \\       
MKV0840  &  0.11 &  0.23 &  0.21 &  0.15 &  0.18 &  0.06 &  0.09 &  0.09 &  0.12 &  0.08 &  0.06 &  0.12 &  0.21 &  0.08 &   ... &  0.09 &  0.21 &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC09430  & $-$2.13 &   ... &   ... &  0.75 &   ... &  0.14 &  0.38 &  0.37 &   ... & $-$0.28 &  0.44 &  0.37 &   ... & $-$0.03 &   ... & $-$0.13 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.22 &   ... &  0.09 &  0.12 &  0.21 &   ... &  0.07 &  0.09 &  0.24 &   ... &  0.07 &   ... &  0.12 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0916  & $-$1.37 &   ... &   ... &  0.08 &   ... &  0.50 &   ... &  0.85 &   ... & $-$0.05 &   ... &  0.68 &   ... &   ... &   ... &  0.37 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.26 &   ... &  0.26 &   ... &  0.43 &   ... &  0.26 &   ... &  0.16 &   ... &   ... &   ... &  0.28 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC06975  & $-$1.84 &   ... &   ... &  0.27 &   ... &  0.14 &  0.39 &  0.17 &   ... & $-$0.03 & $-$0.13 &  0.55 &   ... &  0.10 &   ... &  0.39 &   ... &  0.41 &   ... \\       
         &  0.14 &   ... &   ... &  0.05 &   ... &  0.06 &  0.40 &  0.18 &   ... &  0.09 &  0.23 &  0.34 &   ... &  0.15 &   ... &  0.12 &   ... &  0.24 &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
CC08469  & $-$1.43 &  0.29 & $-$0.29 &  0.00 &  0.42 &  0.04 &  0.09 &  0.13 & $-$0.04 & $-$0.25 & $-$0.35 &  0.23 &   ... & $-$0.07 & $-$0.56 &  0.03 &  0.24 &  0.26 &   ... \\       
Car$-$705  &  0.10 &  0.18 &  0.16 &  0.07 &  0.16 &  0.03 &  0.09 &  0.06 &  0.09 &  0.14 &  0.07 &  0.13 &   ... &  0.04 &  0.24 &  0.10 &  0.14 &  0.23 &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0729  & $-$1.17 &   ... &   ... &  0.52 &   ... &  0.31 &   ... &  0.27 &   ... &  0.52 & $-$0.31 &  0.24 &   ... &  0.51 &   ... &  0.12 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.22 &   ... &  0.12 &   ... &  0.13 &   ... &  0.22 &  0.12 &  0.23 &   ... &  0.22 &   ... &  0.23 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0556  & $-$1.17 &   ... &   ... &  0.49 &   ... &  0.03 &   ... &  0.73 &   ... &  0.27 &   ... &  0.92 &   ... &   ... &   ... &  0.42 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.21 &   ... &  0.09 &   ... &  0.22 &   ... &  0.14 &   ... &  0.29 &   ... &   ... &   ... &  0.22 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0733  & $-$1.55 &   ... &   ... & $-$0.08 &   ... & $-$0.06 &   ... &  0.28 &   ... & $-$0.38 &  0.13 &  0.66 &   ... &   ... &   ... &  0.05 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.25 &   ... &  0.19 &   ... &  0.26 &   ... &  0.25 &  0.25 &  0.21 &   ... &   ... &   ... &  0.26 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0614  & $-$1.55 &   ... &   ... &  0.03 &   ... &   ... &   ... &  0.27 &   ... & $-$0.47 &   ... &  0.28 &   ... &   ... &   ... &  0.09 &   ... &   ... &   ... \\       
         &  0.15 &   ... &   ... &  0.18 &   ... &   ... &   ... &  0.14 &   ... &  0.18 &   ... &  0.23 &   ... &   ... &   ... &  0.21 &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
MKV0708  & $-$1.51 &   ... &   ... &  0.32 &   ... &   ... &   ... &  0.65 &   ... & $-$0.08 &   ... &  0.27 &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\       
         &  0.16 &   ... &   ... &  0.25 &   ... &   ... &   ... &  0.27 &   ... &  0.25 &   ... &  0.21 &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\       
 & & & & & & & & & & & & & & & & & & & \\                                                                                                                                 
\enddata                                                                        
\tablenotetext{a}{For each object the two rows contain [Fe/H] and [X/Fe]; and $\sigma_{\rm {Tot}}$, respectively.}
\tablenotetext{b}{In each block, one or two names are given when one or two observations are available.}
\end{deluxetable}      


==> table2.tex <==
% Table 2
\begin{center}                                                                                                          
\begin{deluxetable}{lccrrrrrrrrrrrr}                                                                                    
\tabletypesize{\tiny}                                                                                                   
\tablecolumns{15}                                                                                                       
\tablewidth{0pt}                                                                                                        
\rotate                                                                                                                 
\tablecaption{\label{tab:ew1} Atomic Data and Equivalent Widths (m{\AA}) for 11 Carina Red Giants}                          
\tablehead{                                                                                                             
\colhead{Species} & {Wavelength} &  {$\chi$} & {log$gf$} & {CC06122} & {CC06486} & {CC06975} & {CC07452} & {CC07889} & {CC08447} & {CC08469} & {CC08615} & {CC08695} & {CC08788} & {CC09000} \\
{(1)} & {(2)} & {(3)} & {(4)} & {(5)} & {(6)} & {(7)} & {(8)} & {(9)} & {(10)} & {(11)} & {(12)} & {(13)} & {(14)} & {(15)}
}                                                                                                                       
\startdata                                                                                                              
$S/N$\tablenotemark{a}  &  &  &  &      17 &       10 &        8 &       18 &        9 &       16 &       11 &       11 &       14 &       10 &       23 \\
W(min)\,(m{\AA})  &  &  &  &      26 &       28 &       31 &       14 &       34 &       24 &       24 &       20 &       23 &       23 &       20 \\
Fe I  &  5302.30 &   3.28 & $-$0.880 &  153.5 &    ... &  126.3 &  144.5 &   66.5 &  122.7 &  147.7 &  115.0 &  143.3 &  121.7 &  140.7 \\
Fe I  &  5307.37 &   1.61 & $-$2.912 &  183.0 &   90.5 &  113.7 &  162.0 &   57.0 &  136.3 &  166.7 &  117.3 &  138.3 &  109.0 &  145.0 \\
Fe I  &  5324.19 &   3.21 & $-$0.100 &  186.5 &    ... &    ... &    ... &  118.5 &  186.5 &  182.0 &    ... &  181.0 &    ... &  193.0 \\
Fe I  &  5332.90 &   1.56 & $-$2.780 &    ... &    ... &  103.0 &  192.5 &   68.5 &    ... &    ... &    ... &  168.5 &    ... &    ... \\
Fe I  &  5339.93 &   3.27 & $-$0.720 &  139.5 &  102.0 &    ... &  160.5 &   29.5 &  144.3 &  147.3 &  110.0 &  157.3 &  143.5 &  147.3 \\
Fe I  &  5364.86 &   4.45 &  0.228 &  124.0 &   43.0 &   70.0 &  114.5 &    ... &   97.0 &  109.7 &   72.5 &  116.0 &   96.5 &   94.3 \\
Fe I  &  5367.48 &   4.42 &  0.443 &  128.3 &   66.0 &   67.7 &  126.0 &    ... &  108.7 &  111.0 &  112.3 &  105.0 &    ... &  105.3 \\
Fe I  &  5369.96 &   4.37 &  0.536 &  129.5 &   56.3 &   69.5 &  118.7 &   33.0 &  121.0 &  113.5 &   60.5 &  134.5 &   97.0 &  102.0 \\
Fe I  &  5371.50 &   0.96 & $-$1.644 &    ... &  180.5 &    ... &    ... &  154.5 &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5383.37 &   4.31 &  0.645 &  145.7 &    ... &  130.7 &  161.3 &    ... &  149.0 &  126.0 &    ... &  164.0 &  105.0 &  122.5 \\
Fe I  &  5389.48 &   4.42 & $-$0.400 &    ... &    ... &    ... &   90.5 &    ... &   54.5 &  103.5 &    ... &    ... &    ... &    ... \\
Fe I  &  5393.17 &   3.24 & $-$0.920 &  183.5 &   91.0 &   98.0 &  159.5 &    ... &  148.0 &    ... &  109.0 &  153.5 &    ... &    ... \\
Fe I  &  5397.13 &   0.91 & $-$1.982 &    ... &  189.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5400.51 &   4.37 & $-$0.150 &  109.5 &    ... &   52.0 &  119.7 &    ... &   92.0 &   75.0 &   53.0 &  105.7 &  107.0 &   89.5 \\
Fe I  &  5405.77 &   0.99 & $-$1.852 &    ... &  177.5 &    ... &    ... &  163.0 &    ... &    ... &  181.5 &    ... &    ... &    ... \\
Fe I  &  5410.92 &   4.47 &  0.398 &  135.7 &   50.0 &    ... &  107.0 &    ... &  108.5 &  118.0 &   84.7 &   93.3 &   72.0 &   95.0 \\
Fe I  &  5415.20 &   4.39 &  0.643 &  137.3 &    ... &  111.0 &  136.0 &    ... &  109.7 &  144.3 &   94.3 &  141.0 &    ... &  109.5 \\
Fe I  &  5417.04 &   4.42 & $-$1.420 &   35.3 &    ... &    ... &   23.5 &    ... &   34.3 &   26.7 &    ... &    ... &    ... &   19.0 \\
Fe I  &  5424.07 &   4.32 &  0.520 &  160.5 &   54.0 &  102.0 &  159.0 &   57.5 &  143.5 &  182.0 &  113.3 &  119.3 &  144.0 &  145.5 \\
Fe I  &  5429.70 &   0.96 & $-$1.881 &    ... &  189.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5434.52 &   1.01 & $-$2.126 &    ... &  163.5 &  194.0 &    ... &  188.5 &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5445.05 &   4.39 & $-$0.020 &  117.5 &   43.3 &   99.5 &  113.0 &    ... &   93.0 &  100.7 &   74.7 &  114.7 &   90.5 &  101.0 \\
Fe I  &  5446.92 &   0.99 & $-$1.914 &    ... &    ... &    ... &    ... &  142.0 &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5464.28 &   4.14 & $-$1.402 &    ... &   32.0 &    ... &    ... &    ... &    ... &   42.0 &    ... &    ... &    ... &    ... \\
Fe I  &  5497.52 &   1.01 & $-$2.825 &    ... &  175.5 &  135.0 &    ... &  123.5 &  184.0 &    ... &  165.5 &    ... &  194.0 &    ... \\
Fe I  &  5501.46 &   0.96 & $-$3.046 &    ... &  120.5 &  156.0 &  197.0 &  133.0 &  192.5 &    ... &  130.0 &    ... &  154.0 &    ... \\
Fe I  &  5506.79 &   0.99 & $-$2.789 &    ... &  144.0 &  192.0 &    ... &  129.0 &    ... &    ... &  162.0 &    ... &  160.0 &  201.5 \\
Fe I  &  5569.62 &   3.42 & $-$0.540 &  153.3 &   76.5 &  108.5 &  158.7 &   70.0 &  149.7 &  143.3 &  108.0 &  164.3 &   95.0 &  138.5 \\
Fe I  &  5576.09 &   3.43 & $-$1.000 &  153.7 &   57.0 &   87.0 &  134.7 &    ... &  119.7 &  161.7 &   77.7 &  125.7 &   97.5 &  122.3 \\
Fe I  &  5586.76 &   3.37 & $-$0.144 &  186.0 &    ... &  103.0 &  186.0 &  100.0 &  155.7 &  161.0 &  140.7 &  180.3 &  159.0 &  175.0 \\
Fe I  &  5624.54 &   3.42 & $-$0.755 &    ... &   62.5 &  102.0 &  155.5 &    ... &  143.5 &  150.5 &    ... &    ... &    ... &    ... \\
Fe I  &  5686.53 &   4.55 & $-$0.450 &    ... &    ... &    ... &   84.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5701.54 &   2.56 & $-$2.143 &  134.7 &    ... &   89.0 &  134.7 &   32.0 &  117.7 &  141.0 &   93.0 &  120.3 &   87.0 &  110.0 \\
Fe I  &  5956.69 &   0.86 & $-$4.498 &  181.7 &    ... &   67.0 &  167.0 &    ... &   97.0 &  189.0 &   77.3 &  144.3 &  141.0 &  156.0 \\
Fe I  &  6003.03 &   3.88 & $-$1.110 &   88.7 &    ... &    ... &   82.3 &    ... &   84.7 &   72.3 &   74.0 &   92.0 &   67.0 &   78.3 \\
Fe I  &  6024.05 &   4.55 & $-$0.110 &   99.3 &   50.7 &    ... &  101.3 &    ... &  102.7 &  117.5 &   55.0 &   76.5 &    ... &   71.0 \\
Fe I  &  6027.05 &   4.07 & $-$1.089 &   79.0 &    ... &   39.5 &   94.5 &    ... &   71.7 &   86.0 &   48.0 &    ... &   42.3 &   49.3 \\
Fe I  &  6056.01 &   4.73 & $-$0.450 &   46.0 &    ... &    ... &   62.3 &    ... &    ... &   62.0 &    ... &    ... &   29.5 &   29.3 \\
Fe I  &  6065.48 &   2.61 & $-$1.410 &  185.0 &  112.7 &  112.3 &  167.3 &   84.0 &  158.3 &  190.7 &  120.5 &  172.0 &    ... &  149.5 \\
Fe I  &  6078.50 &   4.79 & $-$0.370 &   36.3 &    ... &    ... &    ... &    ... &   33.0 &   41.5 &    ... &   65.5 &    ... &   42.5 \\
Fe I  &  6082.72 &   2.22 & $-$3.548 &   85.0 &    ... &    ... &   78.3 &    ... &   60.3 &   75.0 &    ... &   89.7 &   26.0 &   59.0 \\
Fe I  &  6102.18 &   4.84 & $-$0.516 &   67.5 &    ... &    ... &   33.0 &    ... &   53.3 &   65.0 &   23.5 &   57.5 &   39.0 &   39.5 \\
Fe I  &  6120.26 &   0.91 & $-$5.940 &   43.3 &    ... &    ... &   24.3 &    ... &    ... &    ... &    ... &   46.5 &    ... &    ... \\
Fe I  &  6137.69 &   2.59 & $-$1.346 &  169.0 &  127.3 &  134.0 &  182.7 &  102.7 &  185.0 &  206.5 &  185.3 &  219.5 &  140.0 &  178.0 \\
Fe I  &  6151.62 &   2.18 & $-$3.371 &  105.3 &    ... &   53.3 &   91.7 &    ... &   74.3 &  107.0 &   50.0 &  117.3 &   75.0 &   79.7 \\
Fe I  &  6157.75 &   4.07 & $-$1.260 &   70.7 &    ... &    ... &   72.3 &   27.0 &   50.5 &   73.0 &   31.3 &   71.7 &    ... &   47.0 \\
Fe I  &  6165.36 &   4.14 & $-$1.473 &    ... &    ... &    ... &   37.3 &    ... &    ... &   56.0 &    ... &   42.7 &    ... &   27.0 \\
Fe I  &  6173.34 &   2.22 & $-$2.850 &  131.7 &   68.7 &    ... &  123.0 &   39.0 &  109.0 &  117.7 &   62.0 &  121.3 &   81.3 &  107.0 \\
Fe I  &  6180.20 &   2.73 & $-$2.649 &   92.7 &    ... &   47.3 &   83.0 &    ... &    ... &  120.3 &    ... &  101.5 &    ... &   72.7 \\
Fe I  &  6187.99 &   3.94 & $-$1.580 &   51.0 &    ... &   20.0 &   69.7 &   55.3 &    ... &   66.5 &    ... &   68.0 &   28.0 &   36.5 \\
Fe I  &  6200.31 &   2.61 & $-$2.373 &  139.3 &   72.5 &    ... &  117.0 &    ... &   96.3 &    ... &    ... &  112.7 &    ... &  149.0 \\
Fe I  &  6213.43 &   2.22 & $-$2.481 &  144.0 &   60.0 &   72.5 &  152.3 &   59.0 &  122.3 &  138.5 &   75.0 &  157.7 &  110.0 &  131.7 \\
Fe I  &  6219.28 &   2.20 & $-$2.448 &  149.0 &  103.7 &   97.7 &  157.0 &    ... &  130.0 &  149.5 &  122.0 &  156.7 &  131.5 &  153.7 \\
Fe I  &  6229.23 &   2.84 & $-$2.900 &   62.7 &    ... &    ... &   58.3 &    ... &    ... &   61.0 &   29.3 &   49.0 &    ... &   42.0 \\
Fe I  &  6230.74 &   2.56 & $-$1.276 &    ... &  150.5 &  135.0 &  189.0 &   75.5 &  189.5 &    ... &  167.5 &    ... &  144.0 &    ... \\
Fe I  &  6232.65 &   3.65 & $-$1.223 &   99.3 &    ... &    ... &   90.0 &    ... &   71.5 &  103.5 &   33.0 &   87.0 &   53.3 &   67.7 \\
Fe I  &  6240.65 &   2.22 & $-$3.173 &   94.7 &    ... &   58.3 &   93.0 &    ... &   78.7 &  102.0 &   44.0 &   98.7 &   69.3 &   82.0 \\
Fe I  &  6246.32 &   3.60 & $-$0.733 &    ... &   33.0 &   76.5 &  137.7 &   53.0 &  123.7 &  132.0 &   59.7 &  138.7 &  104.0 &  113.3 \\
Fe I  &  6252.56 &   2.40 & $-$1.767 &  184.0 &  127.0 &  148.7 &  172.7 &   92.5 &  155.3 &  184.0 &  116.0 &  184.3 &  156.0 &  178.5 \\
Fe I  &  6254.26 &   2.28 & $-$2.443 &  148.0 &   81.3 &   99.7 &  138.0 &    ... &  144.0 &  164.5 &  112.0 &  159.7 &  117.0 &  159.5 \\
Fe I  &  6265.13 &   2.18 & $-$2.540 &  159.3 &  103.0 &   55.3 &  154.7 &    ... &  129.3 &  166.7 &   80.0 &  145.7 &  108.7 &  141.7 \\
Fe I  &  6280.62 &   0.86 & $-$4.387 &  172.0 &   79.0 &  121.0 &  157.5 &   65.0 &  147.0 &  174.0 &   53.0 &  168.5 &  119.5 &    ... \\
Fe I  &  6297.79 &   2.22 & $-$2.640 &  156.7 &    ... &   79.3 &  141.5 &    ... &  130.0 &  138.0 &    ... &  135.5 &    ... &    ... \\
Fe I  &  6301.50 &   3.65 & $-$0.720 &  128.0 &   61.0 &    ... &  138.3 &    ... &  117.0 &  153.0 &   95.5 &  120.5 &    ... &    ... \\
Fe I  &  6302.49 &   3.69 & $-$1.150 &   92.5 &   33.0 &    ... &   95.0 &    ... &   59.5 &   95.0 &    ... &    ... &   62.5 &   64.5 \\
Fe I  &  6311.51 &   2.83 & $-$3.220 &   47.0 &    ... &    ... &   62.0 &    ... &    ... &   60.0 &    ... &   54.0 &    ... &   26.3 \\
Fe I  &  6322.68 &   2.59 & $-$2.469 &  118.5 &   91.0 &   56.0 &  124.0 &    ... &  101.0 &  127.0 &   98.0 &  133.0 &  111.5 &  120.5 \\
Fe I  &  6335.33 &   2.20 & $-$2.177 &  173.7 &    ... &  117.3 &  164.3 &   50.3 &  159.7 &  161.0 &  124.7 &  152.3 &  123.0 &  153.5 \\
Fe I  &  6336.82 &   3.69 & $-$1.050 &  100.0 &    ... &    ... &  114.7 &    ... &   94.3 &  185.7 &   51.0 &  131.0 &   87.7 &   87.0 \\
Fe I  &  6344.15 &   2.43 & $-$2.877 &  113.3 &   55.5 &    ... &   89.7 &    ... &    ... &  120.3 &   50.0 &    ... &   62.3 &   88.3 \\
Fe I  &  6355.03 &   2.84 & $-$2.291 &   97.0 &    ... &   46.0 &  113.0 &    ... &   94.0 &  103.0 &   39.3 &  114.3 &   76.3 &   74.0 \\
Fe I  &  6380.74 &   4.19 & $-$1.375 &   35.5 &    ... &    ... &   43.5 &    ... &   37.3 &   35.0 &    ... &   38.0 &   26.5 &   29.0 \\
Fe I  &  6392.54 &   2.28 & $-$3.950 &   42.5 &   30.0 &   33.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  6393.61 &   2.43 & $-$1.576 &  176.0 &   98.3 &  122.7 &  193.5 &   87.0 &  182.3 &  182.0 &  153.5 &  189.3 &    ... &  181.0 \\
Fe I  &  6408.03 &   3.69 & $-$1.000 &  115.7 &    ... &   61.3 &  116.7 &    ... &  101.7 &  102.7 &    ... &  112.0 &   53.0 &   89.5 \\
Fe I  &  6411.65 &   3.65 & $-$0.717 &  135.0 &   79.3 &  113.3 &  140.3 &    ... &  117.3 &  150.0 &  119.3 &  135.7 &  119.7 &  128.0 \\
Fe I  &  6419.96 &   4.73 & $-$0.240 &   76.0 &   29.5 &   31.7 &   68.3 &    ... &   67.0 &   75.3 &   49.0 &   78.0 &    ... &   41.5 \\
Fe I  &  6421.35 &   2.28 & $-$2.014 &  169.7 &  115.3 &  130.0 &  186.3 &   85.3 &  156.0 &  170.3 &  125.0 &  185.3 &    ... &  167.0 \\
Fe I  &  6430.85 &   2.18 & $-$1.946 &  195.0 &  113.5 &  128.7 &  182.3 &   86.0 &  162.7 &  181.0 &  126.0 &  181.0 &  161.5 &  187.0 \\
Fe I  &  6481.87 &   2.27 & $-$3.010 &  119.7 &   63.7 &   71.3 &  117.3 &    ... &   96.7 &  112.0 &    ... &  136.5 &   66.0 &   98.0 \\
Fe I  &  6494.98 &   2.40 & $-$1.239 &  215.0 &  133.3 &  147.7 &  191.3 &  104.0 &  179.7 &  219.5 &  157.0 &  199.5 &  161.7 &  197.0 \\
Fe I  &  6498.94 &   0.96 & $-$4.689 &  150.3 &   50.7 &   67.5 &  141.0 &    ... &  105.3 &  158.0 &   70.0 &  129.0 &   77.7 &  120.0 \\
Fe I  &  6518.37 &   2.83 & $-$2.297 &   96.3 &    ... &   34.5 &   87.0 &    ... &   84.5 &  112.0 &    ... &   91.0 &    ... &   65.5 \\
Fe I  &  6533.93 &   4.55 & $-$1.460 &    ... &    ... &    ... &   43.0 &    ... &   39.5 &    ... &    ... &   29.0 &    ... &    ... \\
Fe I  &  6569.22 &   4.73 & $-$0.420 &   66.5 &    ... &    ... &   58.0 &    ... &   51.3 &   88.3 &   44.7 &   66.0 &    ... &   42.0 \\
Fe I  &  6574.23 &   0.99 & $-$5.022 &  120.3 &    ... &   53.0 &  112.0 &    ... &   74.7 &  123.0 &   36.0 &   97.0 &   58.0 &   93.0 \\
Fe I  &  6581.22 &   1.48 & $-$4.680 &   78.0 &    ... &    ... &   73.0 &    ... &   50.0 &   80.0 &    ... &   67.3 &    ... &    ... \\
Fe I  &  6592.91 &   2.73 & $-$1.470 &  168.3 &  105.0 &  121.0 &  174.0 &   88.0 &  149.7 &  161.5 &  139.0 &  164.0 &  150.0 &  155.7 \\
Fe I  &  6593.87 &   2.43 & $-$2.366 &  155.7 &   73.3 &   70.7 &  135.7 &   32.5 &  119.3 &  139.0 &   86.0 &  160.3 &  120.0 &  134.5 \\
Fe I  &  6597.56 &   4.79 & $-$1.070 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   41.5 &    ... \\
Fe I  &  6608.03 &   2.28 & $-$3.940 &   41.7 &    ... &    ... &   36.3 &    ... &    ... &   20.0 &   53.5 &   47.0 &   65.0 &    ... \\
Fe I  &  6609.11 &   2.56 & $-$2.661 &  114.0 &   60.0 &   63.0 &  109.7 &    ... &    ... &   99.7 &   56.3 &  106.7 &   57.5 &   88.0 \\
Fe I  &  6627.54 &   4.54 & $-$1.680 &   23.5 &    ... &   29.7 &   20.0 &    ... &    ... &    ... &   22.0 &    ... &   25.0 &    ... \\
Fe I  &  6633.75 &   4.56 & $-$0.799 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  6663.44 &   2.42 & $-$2.479 &  151.7 &   46.7 &   86.7 &  150.0 &   65.0 &  132.0 &  164.3 &   71.5 &  155.7 &    ... &  132.0 \\
Fe I  &  6677.99 &   2.69 & $-$1.420 &  194.3 &   92.7 &  141.0 &  161.3 &   61.5 &  152.3 &  204.5 &  128.0 &  183.7 &  159.0 &  178.0 \\
Fe I  &  6750.15 &   2.42 & $-$2.621 &  131.3 &    ... &   73.3 &  125.7 &   46.0 &  102.7 &  137.0 &   42.3 &  132.7 &   64.0 &  100.0 \\
Fe II &  5414.08 &   3.22 & $-$3.610 &    ... &    ... &    ... &   51.0 &    ... &    ... &   21.5 &    ... &   34.5 &   35.5 &   18.0 \\
Fe II &  5425.25 &   3.20 & $-$3.360 &    ... &    ... &   70.5 &   54.3 &    ... &   59.0 &   69.0 &   36.5 &   51.7 &   59.5 &   52.0 \\
Fe II &  5534.85 &   3.24 & $-$2.920 &    ... &    ... &    ... &   95.5 &    ... &   73.5 &    ... &   84.5 &   85.0 &  102.5 &    ... \\
Fe II &  5991.38 &   3.15 & $-$3.740 &   27.3 &    ... &    ... &   49.7 &    ... &   33.0 &   27.7 &    ... &   23.0 &   36.5 &   28.5 \\
Fe II &  6149.25 &   3.89 & $-$2.720 &   41.3 &    ... &    ... &   46.0 &   44.0 &   61.5 &   47.0 &    ... &   39.3 &    ... &   38.3 \\
Fe II &  6238.38 &   3.89 & $-$2.670 &   41.0 &    ... &    ... &   53.0 &    ... &   22.0 &   49.0 &    ... &   30.7 &    ... &   39.0 \\
Fe II &  6247.56 &   3.89 & $-$2.360 &   58.0 &   22.0 &    ... &   67.0 &    ... &   69.7 &   74.5 &    ... &   68.3 &   74.0 &    ... \\
Fe II &  6369.46 &   2.89 & $-$4.020 &    ... &    ... &    ... &   38.0 &    ... &    ... &    ... &    ... &   33.7 &    ... &   20.5 \\
Fe II &  6416.93 &   3.89 & $-$2.790 &   33.3 &    ... &   28.0 &   48.7 &    ... &   33.5 &   49.0 &   28.5 &    ... &   41.3 &   27.5 \\
Fe II &  6432.68 &   2.89 & $-$3.710 &   45.3 &    ... &   36.0 &   72.3 &    ... &   47.3 &   57.7 &   69.5 &   55.0 &   93.5 &   63.5 \\
Fe II &  6456.39 &   3.90 & $-$2.080 &   60.5 &    ... &    ... &   72.0 &   43.5 &   86.0 &   81.0 &    ... &    ... &   69.7 &   73.0 \\
Fe II &  6516.08 &   2.89 & $-$3.450 &   55.3 &   55.0 &    ... &   69.3 &    ... &   59.0 &   56.0 &   52.7 &   72.5 &   42.3 &   59.0 \\
O  I  &  6300.31 &   0.00 & $-$9.750 &   37.3 &  $<$30.0 &  $<$35.0 &   12.5 &  $<$35.0 &   23.0 &   38.7 &   22.0 &   28.3 &    ... &   19.0 \\
Na I  &  5688.21 &   2.10 & $-$0.370 &   67.0 &   35.5 &  $<$35.0 &   35.0 &  $<$50.0 &   53.5 &   52.0 &   36.5 &   79.0 &   46.5 &  $<$25.0 \\
Mg I  &  5528.41 &   4.34 & $-$0.480 &  204.5 &  120.7 &  144.0 &  157.0 &  140.0 &  188.3 &  171.7 &  184.3 &  186.0 &  176.0 &  142.3 \\
Mg I  &  5711.09 &   4.35 & $-$1.728 &   93.0 &   29.7 &   53.3 &   41.7 &    ... &   73.0 &   80.0 &   59.3 &   87.3 &   65.5 &   30.0 \\
Al I  &  6696.03 &   3.14 & $-$1.570 &  $<$25.0 &  $<$30.0 &  $<$35.0 &  $<$15.0 &  $<$35.0 &   20.0 &  $<$25.0 &  $<$25.0 &   17.5 &  $<$25.0 &  $<$20.0 \\
Si I  &  6142.48 &   5.62 & $-$1.510 &    ... &    ... &    ... &    ... &    ... &    ... &   25.0 &    ... &   18.5 &    ... &    ... \\
Si I  &  6155.14 &   5.62 & $-$0.800 &   37.3 &    ... &   28.0 &    ... &    ... &   27.7 &   47.5 &   37.0 &   38.5 &   23.5 &    ... \\
Si I  &  6237.33 &   5.61 & $-$1.020 &    ... &    ... &    ... &    ... &    ... &    ... &   20.5 &   15.5 &    ... &    ... &    ... \\
Si I  &  6244.48 &   5.61 & $-$1.270 &    ... &    ... &    ... &    ... &    ... &    ... &   26.5 &    ... &    ... &    ... &    ... \\
Ca I  &  5349.47 &   2.71 & $-$0.310 &    ... &    ... &   67.0 &    ... &    ... &    ... &    ... &   74.0 &    ... &    ... &    ... \\
Ca I  &  5581.97 &   2.52 & $-$0.555 &  106.7 &   35.5 &   54.3 &   86.0 &    ... &  103.3 &  106.3 &   65.0 &  136.0 &   82.5 &    ... \\
Ca I  &  5588.75 &   2.52 &  0.210 &  157.7 &   84.0 &  119.3 &  143.7 &  101.0 &  151.7 &  134.3 &  128.0 &  170.0 &  116.5 &  121.7 \\
Ca I  &  5590.12 &   2.52 & $-$0.571 &  101.0 &    ... &    ... &   78.3 &   35.0 &   93.7 &   90.0 &   51.3 &   94.0 &  108.3 &   62.0 \\
Ca I  &  5594.47 &   2.52 &  0.097 &    ... &    ... &  135.5 &  118.5 &    ... &  144.0 &  162.0 &    ... &  187.0 &    ... &  136.0 \\
Ca I  &  5598.49 &   2.52 & $-$0.087 &  177.0 &   97.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Ca I  &  5857.45 &   2.93 &  0.230 &  154.0 &   71.7 &    ... &  107.7 &    ... &  131.7 &  144.0 &  119.0 &  134.0 &  144.0 &   92.5 \\
Ca I  &  5601.28 &   2.53 & $-$0.523 &  103.7 &   42.3 &    ... &   87.0 &   32.0 &   88.0 &  100.3 &   76.0 &   95.0 &   93.5 &    ... \\
Ca I  &  6102.73 &   1.88 & $-$0.790 &  161.5 &  102.0 &  112.0 &  122.5 &   59.3 &  142.0 &  161.5 &  103.3 &  160.5 &  124.5 &  109.5 \\
Ca I  &  6122.23 &   1.89 & $-$0.320 &  197.7 &  116.0 &  141.7 &  180.0 &   90.0 &  164.7 &  185.0 &  136.0 &  178.3 &  161.0 &  148.7 \\
Ca I  &  6161.30 &   2.52 & $-$1.270 &   72.0 &   26.5 &   34.0 &   36.0 &    ... &    ... &   61.7 &   35.5 &    ... &   43.0 &   28.3 \\
Ca I  &  6162.17 &   1.90 & $-$0.090 &  212.5 &  144.3 &  148.3 &  181.3 &   95.3 &  174.0 &  211.0 &  176.7 &  182.0 &  194.3 &  170.7 \\
Ca I  &  6166.44 &   2.52 & $-$1.140 &   68.3 &    ... &    ... &   51.3 &    ... &   42.7 &   74.7 &   36.7 &   66.3 &   49.3 &   25.7 \\
Ca I  &  6169.04 &   2.52 & $-$0.800 &   97.3 &    ... &   59.7 &   63.0 &    ... &   79.5 &   92.5 &    ... &   99.0 &   85.0 &   53.5 \\
Ca I  &  6169.56 &   2.52 & $-$0.480 &  125.0 &   34.0 &   75.0 &   78.0 &   38.3 &   97.7 &  118.5 &   79.0 &  111.3 &   70.7 &   68.5 \\
Ca I  &  6439.08 &   2.52 &  0.390 &  166.7 &   89.3 &  110.0 &  150.7 &   79.5 &  157.7 &  178.0 &  135.7 &  167.3 &  159.0 &  145.7 \\
Ca I  &  6449.81 &   2.52 & $-$0.502 &    ... &    ... &    ... &    ... &   56.0 &    ... &    ... &    ... &    ... &    ... &    ... \\
Ca I  &  6455.60 &   2.52 & $-$1.290 &   58.5 &    ... &    ... &   30.5 &   24.0 &   58.7 &   63.7 &   33.5 &   75.3 &    ... &    ... \\
Ca I  &  6471.67 &   2.52 & $-$0.760 &  113.7 &    ... &   61.5 &   77.0 &    ... &   88.7 &  100.0 &   73.0 &  109.7 &    ... &   56.7 \\
Ca I  &  6493.79 &   2.52 & $-$0.320 &  132.3 &   79.3 &   65.3 &   91.0 &    ... &  104.3 &  115.3 &   69.7 &  117.0 &   82.3 &   85.0 \\
Ca I  &  6499.65 &   2.52 & $-$0.820 &   92.7 &   49.0 &    ... &   95.3 &    ... &   77.7 &  112.5 &   65.3 &  102.7 &   62.7 &   46.3 \\
Ca I  &  6717.68 &   2.71 & $-$0.610 &  115.7 &   44.5 &   62.3 &   87.3 &    ... &   92.3 &  107.5 &   75.0 &  125.7 &    ... &   57.5 \\
Sc II &  5318.37 &   1.36 & $-$2.010 &   30.3 &    ... &    ... &    ... &    ... &   23.3 &    ... &    ... &    ... &   55.3 &    ... \\
Sc II &  5526.79 &   1.77 &  0.030 &  124.3 &   85.7 &  137.7 &    ... &   70.0 &  115.0 &  126.7 &   82.5 &  128.7 &  128.3 &   79.7 \\
Sc II &  5641.00 &   1.50 & $-$1.130 &   69.5 &    ... &    ... &   16.5 &    ... &   56.3 &   69.0 &    ... &   62.0 &    ... &    ... \\
Sc II &  5657.91 &   1.51 & $-$0.600 &    ... &    ... &   70.5 &    ... &    ... &    ... &  100.5 &    ... &    ... &    ... &    ... \\
Sc II &  5667.16 &   1.50 & $-$1.310 &    ... &    ... &    ... &    ... &    ... &    ... &   62.0 &    ... &   45.5 &    ... &    ... \\
Sc II &  5669.06 &   1.50 & $-$1.200 &  111.5 &    ... &    ... &    ... &    ... &   79.0 &    ... &   49.5 &    ... &   70.5 &   41.7 \\
Sc II &  6245.62 &   1.51 & $-$0.970 &    ... &    ... &    ... &    ... &    ... &   55.0 &   75.0 &    ... &   66.5 &   59.0 &    ... \\
Sc II &  6309.90 &   1.50 & $-$1.520 &    ... &    ... &    ... &    ... &    ... &   26.5 &    ... &    ... &    ... &    ... &    ... \\
Sc II &  6604.58 &   1.36 & $-$1.310 &   64.0 &    ... &    ... &    ... &    ... &   56.0 &   70.3 &    ... &   49.3 &    ... &   26.0 \\
Ti I  &  5490.16 &   1.46 & $-$0.933 &   64.0 &    ... &    ... &    ... &    ... &   21.5 &   45.3 &    ... &   60.0 &    ... &    ... \\
Ti I  &  5978.54 &   1.87 & $-$0.440 &   24.3 &    ... &    ... &   23.7 &    ... &    ... &   50.0 &    ... &   45.7 &    ... &    ... \\
Ti I  &  6126.22 &   1.07 & $-$1.425 &   70.3 &    ... &    ... &    ... &    ... &   45.3 &   80.5 &    ... &   65.7 &    ... &   29.0 \\
Ti I  &  6258.10 &   1.44 & $-$0.355 &  107.0 &    ... &    ... &   40.0 &    ... &   77.5 &  108.5 &   47.0 &    ... &   50.5 &    ... \\
Ti I  &  6303.77 &   1.44 & $-$1.570 &    ... &    ... &    ... &   17.0 &    ... &    ... &    ... &   12.5 &   33.5 &    ... &    ... \\
Ti I  &  6312.24 &   1.46 & $-$1.550 &   31.3 &    ... &    ... &   11.0 &    ... &    ... &   26.0 &    ... &   24.5 &    ... &    ... \\
Ti I  &  6336.10 &   1.44 & $-$1.740 &    ... &    ... &    ... &   10.5 &    ... &    ... &    ... &    ... &   24.0 &    ... &    ... \\
Ti I  &  6554.24 &   1.44 & $-$1.218 &   39.7 &    ... &    ... &    ... &    ... &   26.0 &   44.0 &    ... &   37.5 &    ... &    ... \\
Ti I  &  6556.08 &   1.46 & $-$1.074 &   66.0 &    ... &    ... &   21.0 &    ... &   37.0 &   49.0 &   31.5 &   46.3 &   44.5 &   24.0 \\
Ti I  &  6599.13 &   0.90 & $-$2.090 &   30.0 &    ... &    ... &    ... &    ... &    ... &   33.5 &    ... &    ... &    ... &    ... \\
Ti I  &  6743.13 &   0.90 & $-$1.630 &   68.3 &    ... &    ... &   29.3 &    ... &    ... &   80.3 &    ... &    ... &    ... &   31.7 \\
Ti II &  5336.77 &   1.58 & $-$1.700 &    ... &    ... &    ... &  123.0 &   78.0 &  136.7 &    ... &  103.3 &  142.3 &    ... &  137.5 \\
Ti II &  5381.01 &   1.57 & $-$1.780 &  126.5 &    ... &   81.3 &   87.0 &    ... &  132.7 &   97.0 &   54.0 &  104.0 &  101.7 &    ... \\
Ti II &  5418.77 &   1.58 & $-$2.110 &  115.3 &    ... &   78.0 &   90.3 &    ... &  104.7 &  105.0 &   84.0 &  109.0 &   77.0 &   87.7 \\
Ti II &  6559.59 &   2.05 & $-$2.019 &    ... &    ... &    ... &   41.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Ti II &  6606.95 &   2.06 & $-$2.790 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
V  I  &  6090.21 &   1.08 & $-$0.060 &   63.7 &    ... &    ... &   15.0 &    ... &   47.0 &   65.7 &    ... &   85.3 &   26.5 &    ... \\
V  I  &  6119.53 &   1.06 & $-$0.320 &   43.7 &    ... &    ... &    ... &    ... &   37.0 &    ... &    ... &   49.0 &    ... &    ... \\
V  I  &  6135.37 &   1.05 & $-$0.750 &   49.0 &    ... &    ... &    ... &    ... &   36.5 &    ... &    ... &   38.0 &    ... &    ... \\
V  I  &  6150.15 &   0.30 & $-$1.790 &   50.0 &    ... &   28.3 &   30.0 &    ... &   52.3 &   46.7 &    ... &   61.0 &   40.3 &   27.0 \\
V  I  &  6199.19 &   0.29 & $-$1.290 &   73.0 &    ... &    ... &    ... &    ... &   32.5 &   54.5 &    ... &   42.3 &    ... &    ... \\
V  I  &  6216.36 &   0.28 & $-$0.810 &   45.5 &    ... &    ... &   27.0 &    ... &    ... &    ... &    ... &   57.7 &    ... &    ... \\
V  I  &  6224.51 &   0.29 & $-$2.010 &   44.0 &    ... &    ... &    ... &    ... &   23.5 &    ... &    ... &   26.5 &    ... &    ... \\
V  I  &  6233.20 &   0.28 & $-$2.070 &   34.3 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
V  I  &  6243.11 &   0.30 & $-$0.980 &    ... &    ... &    ... &   24.5 &    ... &   54.0 &    ... &    ... &    ... &    ... &    ... \\
V  I  &  6251.82 &   0.29 & $-$1.300 &   70.7 &    ... &    ... &   14.0 &    ... &   33.3 &   56.5 &    ... &   65.3 &   29.0 &   20.5 \\
V  I  &  6292.82 &   0.29 & $-$1.520 &   50.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
V  I  &  6531.41 &   1.22 & $-$0.840 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Cr I  &  5345.80 &   1.00 & $-$0.980 &  181.3 &   80.0 &  117.5 &  175.5 &   61.0 &  151.3 &  156.0 &  116.0 &  160.7 &  135.5 &  158.0 \\
Cr I  &  5348.33 &   1.00 & $-$1.290 &  168.3 &   86.0 &  108.0 &  145.5 &    ... &  129.7 &  152.3 &   91.3 &  140.3 &  101.7 &  146.7 \\
Cr I  &  5409.80 &   1.03 & $-$0.720 &  215.0 &  110.7 &    ... &  186.0 &   54.0 &  174.0 &  170.0 &  127.3 &  160.0 &  141.0 &  185.3 \\
Cr I  &  6330.09 &   0.94 & $-$2.920 &   68.7 &    ... &    ... &   52.3 &    ... &   48.0 &   82.0 &    ... &   64.0 &    ... &   27.7 \\
Mn I  &  5407.42 &   2.14 & $-$1.743 &   66.0 &    ... &    ... &    ... &    ... &   72.0 &    ... &    ... &   52.0 &   39.5 &    ... \\
Mn I  &  5420.36 &   2.14 & $-$1.460 &   90.3 &    ... &    ... &   90.3 &    ... &   62.3 &  118.0 &    ... &   75.7 &    ... &   48.3 \\
Mn I  &  5432.55 &   0.00 & $-$3.795 &  147.3 &    ... &   57.0 &  128.0 &    ... &   96.0 &  127.0 &    ... &  115.3 &   73.5 &  107.0 \\
Mn I  &  5516.77 &   2.18 & $-$1.847 &   54.0 &    ... &    ... &   56.5 &    ... &    ... &    ... &    ... &   29.0 &    ... &    ... \\
Mn I  &  6013.51 &   3.07 & $-$0.252 &   70.7 &    ... &    ... &   62.0 &    ... &   23.5 &   52.5 &    ... &   47.7 &    ... &    ... \\
Mn I  &  6021.82 &   3.08 &  0.035 &    ... &    ... &    ... &   87.3 &    ... &   66.7 &   93.3 &    ... &   87.3 &    ... &   61.7 \\
Co I  &  5647.23 &   2.28 & $-$1.560 &   35.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   25.0 &    ... &    ... \\
Ni I  &  5578.73 &   1.68 & $-$2.670 &  103.7 &   36.5 &   49.0 &    ... &   37.0 &   76.3 &  112.5 &    ... &   79.3 &   39.0 &   65.7 \\
Ni I  &  5587.87 &   1.93 & $-$2.370 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   64.0 &   71.5 \\
Ni I  &  6108.12 &   1.68 & $-$2.450 &   97.7 &   44.0 &    ... &   69.3 &    ... &   71.0 &  114.3 &   45.0 &   88.3 &   63.3 &   71.3 \\
Ni I  &  6128.97 &   1.68 & $-$3.390 &   54.0 &    ... &    ... &   31.0 &    ... &   32.0 &   58.3 &   35.5 &   35.0 &    ... &   34.3 \\
Ni I  &  6176.82 &   4.09 & $-$0.430 &   32.3 &    ... &    ... &    ... &    ... &    ... &    ... &   35.7 &    ... &   22.0 &    ... \\
Ni I  &  6327.60 &   1.68 & $-$3.090 &   83.3 &    ... &   64.0 &   53.0 &    ... &   37.0 &   83.5 &   55.7 &   86.0 &   32.5 &   50.7 \\
Ni I  &  6384.67 &   4.15 & $-$1.000 &   31.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   31.0 &    ... \\
Ni I  &  6482.80 &   1.94 & $-$2.850 &   75.7 &   38.0 &   43.7 &   39.0 &    ... &    ... &   77.5 &    ... &   67.7 &   34.5 &   38.5 \\
Ni I  &  6586.32 &   1.95 & $-$2.790 &   64.0 &    ... &    ... &   50.7 &    ... &    ... &   68.3 &    ... &   69.7 &    ... &   35.0 \\
Ni I  &  6643.64 &   1.68 & $-$2.300 &  149.3 &   74.0 &   66.0 &  115.3 &    ... &  119.0 &  135.0 &   70.3 &  145.7 &  105.7 &  116.0 \\
Ni I  &  6767.78 &   1.83 & $-$2.170 &  129.0 &   74.3 &   78.0 &  110.3 &    ... &  100.7 &  123.5 &   89.0 &  117.3 &  100.7 &  106.3 \\
Cu I  &  5700.24 &   1.64 & $-$2.330 &   28.7 &    ... &    ... &    ... &    ... &   24.0 &   34.0 &    ... &   23.5 &    ... &    ... \\
Zn I  &  6362.35 &   5.80 &  0.140 &    ... &    ... &    ... &    ... &    ... &    ... &   27.0 &    ... &    ... &    ... &    ... \\
Y  II &  5402.78 &   1.84 & $-$0.510 &   29.7 &    ... &    ... &    ... &    ... &    ... &    ... &   37.0 &    ... &    ... &    ... \\
Ba II &  5853.69 &   0.60 & $-$1.010 &  159.3 &   83.0 &  119.0 &   79.7 &    ... &  127.5 &  141.0 &  160.3 &  142.0 &  116.5 &  141.0 \\
Ba II &  6141.73 &   0.70 & $-$0.077 &  226.5 &   90.0 &  183.0 &  150.3 &   82.7 &  191.3 &  208.5 &  152.7 &  200.5 &    ... &  202.5 \\
Ba II &  6496.91 &   0.60 & $-$0.380 &  238.0 &  101.0 &  177.7 &  137.7 &   58.3 &  167.3 &  206.0 &  154.3 &  191.3 &  177.0 &  202.5 \\
La II &  5303.52 &   0.32 & $-$1.350 &    ... &    ... &    ... &    ... &    ... &    ... &   21.7 &   20.5 &   28.0 &    ... &    ... \\
La II &  6320.43 &   0.17 & $-$1.562 &   55.3 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   31.0 \\
La II &  6390.46 &   0.32 & $-$1.400 &   35.5 &    ... &    ... &    ... &    ... &    ... &   37.0 &    ... &    ... &    ... &    ... \\
La II &  6774.27 &   0.13 & $-$1.708 &   45.3 &    ... &    ... &    ... &    ... &    ... &   25.0 &    ... &   21.5 &    ... &   15.5 \\
Nd II &  5319.82 &   0.55 & $-$0.140 &    ... &    ... &   48.0 &    ... &    ... &    ... &    ... &    ... &   63.5 &    ... &   80.0 \\
Eu II &  6645.13 &   1.37 &  0.120 &   22.0 &    ... &    ... &   13.0 &    ... &    ... &    ... &    ... &   36.3 &   34.5 &   37.0 \\
\enddata                                                                                                                
\tablenotetext{a}{$S/N$ per $\sim$0.28\,{\AA}~pixel at 5300 -- 5700\,{\AA}.}                                                      
\end{deluxetable}                                                                                                       
\end{center}                                                                    


==> table3.tex <==
% Table 3
\begin{center}                                                                                                          
\begin{deluxetable}{lccrrrrrrrrrrrr}                                                                                    
\tabletypesize{\tiny}                                                                                                   
\tablecolumns{15}                                                                                                       
\tablewidth{0pt}                                                                                                        
\rotate                                                                                                                 
\tablecaption{\label{tab:ew2} Atomic Data and Equivalent Widths (m{\AA}) for 11 Carina Red Giants}                          
\tablehead{                                                                                                             
\colhead{Species} & {Wavelength} &  {$\chi$} & {log$gf$} & {CC09179} & {CC09225} & {CC09226} & {CC09430} & {CC09507} & {CC09633} & {CC09869} & {CC09929} & {CC10038} & {CC10194} & {CC10318} \\
{(1)} & {(2)} & {(3)} & {(4)} & {(5)} & {(6)} & {(7)} & {(8)} & {(9)} & {(10)} & {(11)} & {(12)} & {(13)} & {(14)} & {(15)}
}                                                                                                                       
\startdata                                                                                                              
$S/N$\tablenotemark{a}  &  &  &  &      13 &       18 &       14 &       12 &       13 &       11 &       12 &        8 &       12 &        9 &       10 \\
W(min)\,(m{\AA})  &  &  &  &      20 &       20 &       20 &       25 &       22 &       29 &       25 &       30 &       22 &       26 &       25 \\
Fe I  &  5302.30 &   3.28 & $-$0.880 &   83.7 &  129.0 &   98.0 &   73.0 &   97.0 &   54.0 &  127.7 &  118.0 &  133.0 &  124.0 &  129.0 \\
Fe I  &  5307.37 &   1.61 & $-$2.912 &   90.3 &  132.3 &  116.5 &   89.5 &  101.0 &   62.0 &  162.0 &   72.0 &  131.7 &  179.5 &    ... \\
Fe I  &  5324.19 &   3.21 & $-$0.100 &    ... &    ... &  147.5 &    ... &    ... &   94.5 &  186.0 &    ... &    ... &    ... &    ... \\
Fe I  &  5332.90 &   1.56 & $-$2.780 &    ... &    ... &    ... &    ... &  119.0 &    ... &  158.0 &    ... &    ... &    ... &  145.5 \\
Fe I  &  5339.93 &   3.27 & $-$0.720 &  130.0 &  148.7 &  130.7 &  102.0 &  116.0 &   46.0 &  136.0 &    ... &  121.7 &  140.5 &  153.7 \\
Fe I  &  5364.86 &   4.45 &  0.228 &   43.0 &   85.3 &   90.7 &    ... &   54.7 &    ... &  113.5 &  109.0 &   94.5 &   97.0 &   86.7 \\
Fe I  &  5367.48 &   4.42 &  0.443 &   97.3 &  106.0 &   94.5 &   64.3 &   85.3 &   58.5 &  111.7 &  123.0 &  104.0 &  125.0 &  122.5 \\
Fe I  &  5369.96 &   4.37 &  0.536 &   90.3 &   97.5 &   98.0 &   69.0 &   78.7 &   42.0 &  125.0 &    ... &  109.0 &   99.5 &  125.0 \\
Fe I  &  5371.50 &   0.96 & $-$1.644 &  197.0 &    ... &    ... &  184.5 &  194.5 &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5383.37 &   4.31 &  0.645 &   89.0 &  119.7 &  102.0 &   92.5 &  106.0 &    ... &  152.5 &    ... &  127.7 &  103.5 &   97.0 \\
Fe I  &  5389.48 &   4.42 & $-$0.400 &    ... &    ... &    ... &    ... &    ... &    ... &  104.0 &    ... &    ... &    ... &    ... \\
Fe I  &  5393.17 &   3.24 & $-$0.920 &  120.0 &  126.0 &  124.0 &   88.5 &  129.0 &   92.0 &  146.0 &    ... &    ... &  154.5 &  188.0 \\
Fe I  &  5397.13 &   0.91 & $-$1.982 &  182.5 &    ... &    ... &  194.5 &  185.5 &  182.5 &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5400.51 &   4.37 & $-$0.150 &   52.5 &   85.0 &   70.0 &    ... &    ... &    ... &  113.0 &    ... &    ... &   97.0 &    ... \\
Fe I  &  5405.77 &   0.99 & $-$1.852 &    ... &    ... &    ... &  193.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5410.92 &   4.47 &  0.398 &   82.5 &   78.5 &   85.7 &   67.3 &   74.5 &    ... &  112.0 &   88.5 &  100.5 &  116.5 &  107.3 \\
Fe I  &  5415.20 &   4.39 &  0.643 &   98.5 &  129.3 &   96.0 &   59.3 &  113.0 &   50.5 &  137.0 &   94.3 &  135.3 &  110.0 &  124.0 \\
Fe I  &  5417.04 &   4.42 & $-$1.420 &    ... &    ... &   23.5 &    ... &   23.5 &    ... &    ... &    ... &   19.0 &    ... &    ... \\
Fe I  &  5424.07 &   4.32 &  0.520 &  107.0 &  138.5 &  124.3 &   70.7 &  127.0 &   58.0 &  175.5 &  132.5 &  131.7 &  131.7 &  106.0 \\
Fe I  &  5429.70 &   0.96 & $-$1.881 &    ... &    ... &    ... &    ... &    ... &  193.0 &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5434.52 &   1.01 & $-$2.126 &  167.0 &  195.5 &  174.0 &  168.5 &    ... &  171.0 &    ... &  154.0 &    ... &    ... &    ... \\
Fe I  &  5445.05 &   4.39 & $-$0.020 &   70.3 &   92.0 &   79.0 &    ... &   61.0 &    ... &  107.0 &    ... &  121.5 &  114.0 &   93.0 \\
Fe I  &  5446.92 &   0.99 & $-$1.914 &    ... &    ... &    ... &  188.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5464.28 &   4.14 & $-$1.402 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5497.52 &   1.01 & $-$2.825 &    ... &  197.5 &  178.5 &  167.0 &    ... &    ... &    ... &  188.0 &    ... &    ... &    ... \\
Fe I  &  5501.46 &   0.96 & $-$3.046 &  137.5 &    ... &  156.5 &    ... &  150.0 &    ... &    ... &  169.5 &    ... &    ... &  184.0 \\
Fe I  &  5506.79 &   0.99 & $-$2.789 &  156.0 &  184.0 &  176.0 &  147.5 &  155.5 &  151.0 &    ... &  157.0 &    ... &  197.5 &  187.0 \\
Fe I  &  5569.62 &   3.42 & $-$0.540 &   93.5 &  137.0 &   94.0 &   88.0 &   96.0 &    ... &  153.0 &    ... &  158.3 &  162.7 &  131.3 \\
Fe I  &  5576.09 &   3.43 & $-$1.000 &   99.5 &  120.0 &   91.5 &   76.3 &  104.5 &    ... &  138.0 &  140.0 &  122.5 &  123.5 &  137.5 \\
Fe I  &  5586.76 &   3.37 & $-$0.144 &  109.0 &  151.5 &  133.3 &  119.3 &  122.0 &  104.0 &  172.0 &  145.3 &  154.3 &  156.0 &  154.0 \\
Fe I  &  5624.54 &   3.42 & $-$0.755 &    ... &    ... &    ... &   76.0 &  101.5 &   52.0 &    ... &    ... &    ... &  158.0 &    ... \\
Fe I  &  5686.53 &   4.55 & $-$0.450 &    ... &   63.5 &   43.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   42.0 \\
Fe I  &  5701.54 &   2.56 & $-$2.143 &   71.0 &  118.0 &   77.7 &   70.0 &   78.0 &    ... &  115.0 &   88.0 &  123.0 &  122.5 &  114.5 \\
Fe I  &  5956.69 &   0.86 & $-$4.498 &   63.0 &  141.0 &  130.0 &    ... &    ... &    ... &  147.7 &    ... &  109.5 &   94.3 &  109.0 \\
Fe I  &  6003.03 &   3.88 & $-$1.110 &    ... &   70.0 &   74.0 &    ... &   36.5 &    ... &   87.5 &    ... &   78.5 &    ... &   68.5 \\
Fe I  &  6024.05 &   4.55 & $-$0.110 &   64.0 &   67.0 &   70.0 &    ... &   55.7 &    ... &   75.7 &   75.0 &   81.0 &    ... &    ... \\
Fe I  &  6027.05 &   4.07 & $-$1.089 &   39.0 &   66.3 &   41.0 &   30.5 &    ... &    ... &   86.5 &   50.0 &   72.0 &    ... &    ... \\
Fe I  &  6056.01 &   4.73 & $-$0.450 &    ... &    ... &    ... &    ... &   18.0 &    ... &    ... &    ... &   67.7 &    ... &    ... \\
Fe I  &  6065.48 &   2.61 & $-$1.410 &  111.3 &  142.0 &  116.0 &   83.3 &  129.0 &   95.0 &  153.3 &    ... &  150.5 &  168.7 &  160.7 \\
Fe I  &  6078.50 &   4.79 & $-$0.370 &   34.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   52.0 &   68.3 &    ... \\
Fe I  &  6082.72 &   2.22 & $-$3.548 &   24.5 &   40.0 &    ... &    ... &    ... &    ... &   38.7 &    ... &    ... &   89.3 &   45.5 \\
Fe I  &  6102.18 &   4.84 & $-$0.516 &   20.0 &   38.0 &    ... &    ... &   40.5 &    ... &   57.5 &   52.5 &   43.5 &   49.5 &   37.5 \\
Fe I  &  6120.26 &   0.91 & $-$5.940 &    ... &    ... &    ... &    ... &    ... &    ... &   45.0 &    ... &    ... &    ... &    ... \\
Fe I  &  6137.69 &   2.59 & $-$1.346 &  116.5 &  139.0 &  120.3 &  128.0 &  151.3 &    ... &    ... &    ... &  172.0 &  175.0 &  152.0 \\
Fe I  &  6151.62 &   2.18 & $-$3.371 &   36.0 &   76.3 &   53.7 &    ... &   41.5 &    ... &   86.7 &   82.3 &  102.7 &   56.3 &   76.0 \\
Fe I  &  6157.75 &   4.07 & $-$1.260 &    ... &   36.0 &    ... &    ... &   35.5 &   30.0 &   74.0 &    ... &   63.3 &   52.3 &   65.3 \\
Fe I  &  6165.36 &   4.14 & $-$1.473 &    ... &    ... &    ... &    ... &    ... &    ... &   54.5 &    ... &    ... &    ... &    ... \\
Fe I  &  6173.34 &   2.22 & $-$2.850 &   55.7 &   97.3 &   60.7 &   37.0 &   75.0 &    ... &  124.7 &   82.5 &   86.0 &  112.7 &  120.3 \\
Fe I  &  6180.20 &   2.73 & $-$2.649 &   35.0 &   71.3 &   79.5 &    ... &   26.0 &    ... &    ... &    ... &   61.5 &   82.5 &    ... \\
Fe I  &  6187.99 &   3.94 & $-$1.580 &    ... &    ... &    ... &    ... &   29.0 &    ... &   67.5 &    ... &    ... &    ... &    ... \\
Fe I  &  6200.31 &   2.61 & $-$2.373 &   79.5 &    ... &   68.5 &    ... &   75.0 &    ... &    ... &   54.5 &  139.5 &  142.0 &    ... \\
Fe I  &  6213.43 &   2.22 & $-$2.481 &   84.5 &  123.0 &   86.0 &   76.5 &   91.3 &   45.3 &  146.0 &  118.0 &  120.0 &  103.7 &  141.7 \\
Fe I  &  6219.28 &   2.20 & $-$2.448 &  102.3 &  130.3 &   82.7 &   72.0 &    ... &   78.0 &  140.3 &  146.3 &  138.0 &    ... &    ... \\
Fe I  &  6229.23 &   2.84 & $-$2.900 &    ... &   32.3 &   26.7 &    ... &    ... &    ... &   48.0 &    ... &   48.5 &   76.5 &   34.0 \\
Fe I  &  6230.74 &   2.56 & $-$1.276 &  139.0 &  174.5 &  161.0 &    ... &  132.0 &  121.0 &    ... &  169.5 &    ... &    ... &    ... \\
Fe I  &  6232.65 &   3.65 & $-$1.223 &   32.3 &   63.0 &   58.3 &    ... &    ... &    ... &   84.3 &   85.7 &   73.3 &   76.7 &   74.0 \\
Fe I  &  6240.65 &   2.22 & $-$3.173 &    ... &   66.5 &   44.0 &   40.0 &   45.0 &    ... &   94.7 &    ... &   79.7 &   80.5 &   71.0 \\
Fe I  &  6246.32 &   3.60 & $-$0.733 &   53.0 &   90.0 &   80.7 &   69.5 &   66.3 &   37.0 &  123.7 &    ... &  121.5 &  122.5 &  127.7 \\
Fe I  &  6252.56 &   2.40 & $-$1.767 &  123.0 &  162.3 &  108.0 &  102.0 &  145.0 &   90.0 &  161.7 &  104.5 &  140.5 &  136.3 &  153.0 \\
Fe I  &  6254.26 &   2.28 & $-$2.443 &   82.7 &  129.5 &  118.5 &   71.7 &   84.0 &    ... &  148.0 &    ... &  132.3 &  127.0 &  153.0 \\
Fe I  &  6265.13 &   2.18 & $-$2.540 &   93.7 &  125.7 &   87.0 &   72.0 &  104.0 &   60.5 &  140.5 &  104.5 &  130.7 &  123.0 &  119.7 \\
Fe I  &  6280.62 &   0.86 & $-$4.387 &   84.0 &  107.5 &   96.5 &   70.5 &   80.0 &   49.5 &  137.5 &  109.5 &  135.0 &  142.5 &  123.0 \\
Fe I  &  6297.79 &   2.22 & $-$2.640 &    ... &  111.5 &   79.5 &    ... &    ... &    ... &  129.0 &  101.3 &  130.5 &  134.5 &  146.0 \\
Fe I  &  6301.50 &   3.65 & $-$0.720 &    ... &  109.5 &  107.0 &    ... &   83.0 &    ... &  108.0 &  101.7 &  163.0 &  108.5 &  129.0 \\
Fe I  &  6302.49 &   3.69 & $-$1.150 &   36.5 &   37.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  6311.51 &   2.83 & $-$3.220 &    ... &   31.5 &    ... &   34.0 &   22.5 &    ... &    ... &   34.7 &   38.7 &    ... &   45.5 \\
Fe I  &  6322.68 &   2.59 & $-$2.469 &   63.5 &   99.0 &    ... &    ... &   71.5 &    ... &  132.3 &  105.0 &  109.0 &  122.0 &  113.7 \\
Fe I  &  6335.33 &   2.20 & $-$2.177 &  110.5 &  144.3 &  109.7 &    ... &  100.5 &   96.0 &  157.3 &  143.0 &  149.0 &  147.0 &  140.7 \\
Fe I  &  6336.82 &   3.69 & $-$1.050 &   67.7 &  100.0 &   80.3 &   35.0 &   59.0 &    ... &  186.0 &   64.0 &   94.5 &  119.0 &   98.5 \\
Fe I  &  6344.15 &   2.43 & $-$2.877 &    ... &   85.0 &   41.0 &   27.0 &   54.0 &    ... &    ... &    ... &   95.3 &   87.0 &   75.0 \\
Fe I  &  6355.03 &   2.84 & $-$2.291 &    ... &   72.7 &   61.0 &    ... &   56.5 &    ... &   96.5 &   80.5 &   98.7 &   89.3 &   88.7 \\
Fe I  &  6380.74 &   4.19 & $-$1.375 &    ... &   37.0 &   34.7 &    ... &    ... &    ... &    ... &    ... &   45.0 &   63.0 &    ... \\
Fe I  &  6392.54 &   2.28 & $-$3.950 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  6393.61 &   2.43 & $-$1.576 &  133.0 &  169.5 &  151.0 &  119.3 &  127.5 &  128.5 &  146.5 &  176.0 &  164.0 &  169.0 &  176.7 \\
Fe I  &  6408.03 &   3.69 & $-$1.000 &   53.0 &   85.3 &   59.0 &   31.7 &   51.7 &    ... &  102.3 &   78.0 &  104.0 &  102.0 &  106.3 \\
Fe I  &  6411.65 &   3.65 & $-$0.717 &   85.0 &  114.0 &   94.0 &   53.5 &   85.7 &   51.5 &  137.5 &  130.5 &  128.0 &  137.7 &  106.0 \\
Fe I  &  6419.96 &   4.73 & $-$0.240 &   20.0 &   34.5 &    ... &    ... &    ... &   29.5 &   76.7 &    ... &   74.0 &    ... &   52.3 \\
Fe I  &  6421.35 &   2.28 & $-$2.014 &  127.5 &  150.3 &  107.0 &  103.7 &  132.7 &   86.5 &  161.3 &  138.3 &  160.0 &  168.5 &  151.3 \\
Fe I  &  6430.85 &   2.18 & $-$1.946 &  117.7 &  148.0 &  136.3 &  112.0 &  127.3 &    ... &  171.7 &  143.0 &  163.7 &  157.0 &  158.3 \\
Fe I  &  6481.87 &   2.27 & $-$3.010 &   65.0 &   85.0 &    ... &    ... &    ... &    ... &  116.5 &   73.5 &  105.5 &  103.5 &   92.5 \\
Fe I  &  6494.98 &   2.40 & $-$1.239 &  145.0 &  176.0 &  126.0 &  132.0 &  143.0 &  120.0 &  169.0 &  179.0 &  200.5 &  206.0 &  184.7 \\
Fe I  &  6498.94 &   0.96 & $-$4.689 &   64.5 &   94.5 &   64.0 &   60.0 &   67.3 &   37.7 &  135.0 &   98.5 &  113.0 &  124.7 &  104.5 \\
Fe I  &  6518.37 &   2.83 & $-$2.297 &    ... &    ... &    ... &    ... &    ... &    ... &  106.7 &    ... &   93.0 &    ... &   78.0 \\
Fe I  &  6533.93 &   4.55 & $-$1.460 &    ... &    ... &    ... &    ... &    ... &    ... &   59.5 &    ... &    ... &    ... &    ... \\
Fe I  &  6569.22 &   4.73 & $-$0.420 &    ... &   40.7 &   44.3 &   23.0 &   25.0 &    ... &   57.7 &    ... &   65.0 &    ... &   44.3 \\
Fe I  &  6574.23 &   0.99 & $-$5.022 &   47.5 &   73.3 &   44.7 &   46.7 &    ... &    ... &  107.0 &   57.0 &   92.0 &  101.5 &   82.7 \\
Fe I  &  6581.22 &   1.48 & $-$4.680 &    ... &   48.5 &   32.0 &   18.5 &    ... &    ... &   83.7 &    ... &   49.0 &    ... &   44.5 \\
Fe I  &  6592.91 &   2.73 & $-$1.470 &  117.0 &  134.5 &  103.0 &   75.0 &  140.7 &   67.0 &  160.0 &  126.7 &  142.0 &  152.0 &  123.7 \\
Fe I  &  6593.87 &   2.43 & $-$2.366 &   95.0 &  118.3 &  113.3 &   60.0 &  108.7 &   53.3 &  145.3 &  133.5 &  134.5 &  122.5 &  120.7 \\
Fe I  &  6597.56 &   4.79 & $-$1.070 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  6608.03 &   2.28 & $-$3.940 &    ... &   45.3 &   31.0 &    ... &    ... &    ... &   31.5 &    ... &    ... &    ... &   23.0 \\
Fe I  &  6609.11 &   2.56 & $-$2.661 &   56.5 &   84.0 &   46.5 &   38.5 &   54.3 &    ... &   85.3 &   89.0 &  104.5 &   84.0 &   94.0 \\
Fe I  &  6627.54 &   4.54 & $-$1.680 &    ... &    ... &   18.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  6633.75 &   4.56 & $-$0.799 &    ... &    ... &    ... &    ... &    ... &    ... &   61.5 &    ... &    ... &    ... &    ... \\
Fe I  &  6663.44 &   2.42 & $-$2.479 &   63.5 &  123.5 &    ... &   74.3 &   73.0 &   47.5 &  154.0 &  157.3 &  131.7 &  123.0 &    ... \\
Fe I  &  6677.99 &   2.69 & $-$1.420 &  133.0 &  144.7 &  145.7 &  131.5 &  107.0 &   81.7 &  159.5 &  130.0 &  192.0 &  206.5 &  192.3 \\
Fe I  &  6750.15 &   2.42 & $-$2.621 &    ... &   95.3 &   65.5 &   56.0 &   66.0 &   40.0 &  125.3 &  129.0 &   97.0 &    ... &  103.3 \\
Fe II &  5414.08 &   3.22 & $-$3.610 &   44.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   18.5 &    ... &   26.0 \\
Fe II &  5425.25 &   3.20 & $-$3.360 &   37.5 &   39.0 &   42.0 &   42.0 &    ... &    ... &    ... &    ... &   64.5 &   44.5 &   48.5 \\
Fe II &  5534.85 &   3.24 & $-$2.920 &    ... &    ... &    ... &    ... &    ... &   38.5 &    ... &   76.5 &   75.0 &    ... &    ... \\
Fe II &  5991.38 &   3.15 & $-$3.740 &    ... &   28.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe II &  6149.25 &   3.89 & $-$2.720 &   26.0 &   27.0 &   24.5 &    ... &    ... &    ... &    ... &    ... &   23.0 &   23.0 &   21.5 \\
Fe II &  6238.38 &   3.89 & $-$2.670 &    ... &   37.7 &    ... &   28.7 &    ... &    ... &   35.0 &   23.0 &    ... &   31.7 &   29.0 \\
Fe II &  6247.56 &   3.89 & $-$2.360 &    ... &   57.3 &   66.0 &    ... &   41.0 &    ... &   74.3 &    ... &   41.5 &   69.0 &   60.7 \\
Fe II &  6369.46 &   2.89 & $-$4.020 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   31.5 &    ... &    ... \\
Fe II &  6416.93 &   3.89 & $-$2.790 &   25.0 &    ... &    ... &    ... &   37.0 &    ... &   35.0 &    ... &   28.0 &    ... &    ... \\
Fe II &  6432.68 &   2.89 & $-$3.710 &   35.7 &   50.0 &   50.0 &   24.0 &   41.7 &    ... &   39.0 &   59.5 &   37.5 &   33.5 &   35.7 \\
Fe II &  6456.39 &   3.90 & $-$2.080 &   53.0 &   66.5 &   46.3 &   33.0 &    ... &   26.5 &   94.0 &    ... &   73.0 &    ... &   82.0 \\
Fe II &  6516.08 &   2.89 & $-$3.450 &   62.5 &   54.0 &   51.0 &    ... &   47.5 &   42.0 &   58.5 &   54.5 &   45.0 &   49.5 &   52.3 \\
O  I  &  6300.31 &   0.00 & $-$9.750 &  $<$25.0 &   34.0 &   23.5 &  $<$25.0 &  $<$25.0 &  $<$30.0 &   18.0 &   49.0 &   41.0 &   29.5 &   43.5 \\
Na I  &  5688.21 &   2.10 & $-$0.370 &  $<$25.0 &   37.0 &   36.5 &  $<$25.0 &  $<$25.0 &  $<$30.0 &   70.5 &   36.0 &   58.5 &   52.5 &  $<$35.0 \\
Mg I  &  5528.41 &   4.34 & $-$0.480 &  141.3 &  172.5 &  149.0 &  160.7 &  118.3 &   92.0 &  178.3 &  159.5 &  191.5 &  172.7 &  165.7 \\
Mg I  &  5711.09 &   4.35 & $-$1.728 &   21.5 &   84.0 &   52.3 &   52.3 &   30.7 &    ... &   98.0 &   70.3 &   77.3 &   76.3 &   55.5 \\
Al I  &  6696.03 &   3.14 & $-$1.570 &  $<$20.0 &  $<$20.0 &  $<$20.0 &  $<$25.0 &  $<$25.0 &  $<$30.0 &  $<$25.0 &  $<$30.0 &  $<$30.0 &  $<$25.0 &  $<$25.0 \\
Si I  &  6142.48 &   5.62 & $-$1.510 &    ... &   17.5 &    ... &    ... &    ... &    ... &    ... &    ... &   24.0 &    ... &    ... \\
Si I  &  6155.14 &   5.62 & $-$0.800 &    ... &   23.0 &   20.5 &   22.0 &    ... &    ... &   36.5 &   31.0 &   43.0 &   35.5 &   27.5 \\
Si I  &  6237.33 &   5.61 & $-$1.020 &   19.5 &    ... &    ... &   22.5 &    ... &    ... &   32.0 &    ... &   27.0 &    ... &   27.3 \\
Si I  &  6244.48 &   5.61 & $-$1.270 &   26.0 &    ... &   24.3 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Ca I  &  5349.47 &   2.71 & $-$0.310 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Ca I  &  5581.97 &   2.52 & $-$0.555 &    ... &   84.0 &   76.3 &   45.5 &   39.5 &    ... &  109.7 &   85.5 &   99.0 &   78.5 &   88.3 \\
Ca I  &  5588.75 &   2.52 &  0.210 &   83.3 &  140.3 &  122.7 &   91.7 &  107.5 &   73.0 &  159.0 &  113.3 &  153.5 &  146.7 &  133.0 \\
Ca I  &  5590.12 &   2.52 & $-$0.571 &   47.5 &   76.7 &   75.3 &   42.5 &   46.0 &   41.7 &   91.5 &   83.7 &   96.0 &   72.0 &   63.0 \\
Ca I  &  5594.47 &   2.52 &  0.097 &   85.0 &  160.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Ca I  &  5598.49 &   2.52 & $-$0.087 &    ... &  151.5 &    ... &   84.0 &    ... &   57.5 &    ... &    ... &    ... &    ... &    ... \\
Ca I  &  5857.45 &   2.93 &  0.230 &   59.5 &  107.5 &    ... &    ... &    ... &   37.0 &  146.5 &  138.3 &  110.0 &  137.7 &    ... \\
Ca I  &  5601.28 &   2.53 & $-$0.523 &   41.0 &   59.0 &   55.5 &   33.0 &    ... &   36.0 &  117.0 &   91.0 &    ... &   82.7 &    ... \\
Ca I  &  6102.73 &   1.88 & $-$0.790 &   97.0 &  122.5 &  108.3 &   68.0 &   91.0 &   44.5 &  136.0 &  124.0 &  124.0 &  141.5 &  111.3 \\
Ca I  &  6122.23 &   1.89 & $-$0.320 &  131.7 &  164.7 &  145.0 &  130.7 &  120.3 &   94.0 &  192.0 &  203.0 &  186.7 &  177.0 &  165.7 \\
Ca I  &  6161.30 &   2.52 & $-$1.270 &    ... &   38.5 &   23.0 &    ... &    ... &    ... &   53.5 &   73.3 &   48.5 &   55.3 &    ... \\
Ca I  &  6162.17 &   1.90 & $-$0.090 &  146.7 &  188.0 &  173.7 &  116.0 &  134.0 &   87.5 &  206.5 &    ... &  178.0 &  199.5 &  191.3 \\
Ca I  &  6166.44 &   2.52 & $-$1.140 &    ... &   46.0 &   35.0 &    ... &   30.0 &    ... &   71.3 &   52.0 &   69.0 &   52.5 &   58.3 \\
Ca I  &  6169.04 &   2.52 & $-$0.800 &   28.5 &   78.0 &    ... &    ... &   42.7 &    ... &   90.0 &  109.5 &   78.0 &    ... &   77.0 \\
Ca I  &  6169.56 &   2.52 & $-$0.480 &   27.3 &   95.5 &    ... &   32.5 &   39.3 &   44.0 &  103.0 &   95.5 &   91.5 &  126.7 &  107.7 \\
Ca I  &  6439.08 &   2.52 &  0.390 &  110.7 &  145.0 &  141.0 &   90.0 &  115.7 &   97.7 &  135.3 &  156.0 &  154.3 &  166.3 &  143.0 \\
Ca I  &  6449.81 &   2.52 & $-$0.502 &    ... &    ... &    ... &    ... &   72.5 &    ... &    ... &    ... &    ... &    ... &    ... \\
Ca I  &  6455.60 &   2.52 & $-$1.290 &    ... &   27.0 &   28.0 &   42.0 &    ... &    ... &   71.5 &    ... &   54.7 &    ... &   59.0 \\
Ca I  &  6471.67 &   2.52 & $-$0.760 &   47.0 &   64.7 &   71.3 &   60.0 &   56.0 &    ... &   88.3 &  113.5 &   85.5 &   97.0 &   76.0 \\
Ca I  &  6493.79 &   2.52 & $-$0.320 &   53.0 &  112.7 &   92.0 &    ... &   60.7 &    ... &  131.7 &  104.5 &   61.0 &   80.7 &  101.0 \\
Ca I  &  6499.65 &   2.52 & $-$0.820 &   49.0 &   68.0 &   50.0 &   31.5 &   30.0 &   28.0 &  115.3 &   88.3 &   88.0 &   75.5 &   72.0 \\
Ca I  &  6717.68 &   2.71 & $-$0.610 &    ... &   87.3 &   77.0 &    ... &   37.5 &    ... &  110.0 &   95.0 &  108.5 &   89.7 &   91.7 \\
Sc II &  5318.37 &   1.36 & $-$2.010 &   19.5 &    ... &    ... &    ... &    ... &    ... &   45.7 &    ... &    ... &    ... &   48.0 \\
Sc II &  5526.79 &   1.77 &  0.030 &   65.0 &  116.7 &   97.7 &   90.5 &   69.0 &   81.0 &  124.7 &   82.0 &  103.7 &   93.7 &  123.5 \\
Sc II &  5641.00 &   1.50 & $-$1.130 &    ... &   61.5 &   55.0 &   41.0 &   32.0 &   41.5 &   75.5 &   85.0 &   57.3 &   45.5 &   68.0 \\
Sc II &  5657.91 &   1.51 & $-$0.600 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   95.0 &    ... &  121.5 \\
Sc II &  5667.16 &   1.50 & $-$1.310 &    ... &   33.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Sc II &  5669.06 &   1.50 & $-$1.200 &   27.0 &   60.5 &   57.0 &   43.0 &   61.0 &    ... &   63.5 &   70.5 &   59.5 &   58.5 &   71.5 \\
Sc II &  6245.62 &   1.51 & $-$0.970 &   19.5 &   59.0 &   44.5 &    ... &   23.0 &    ... &    ... &    ... &    ... &    ... &    ... \\
Sc II &  6309.90 &   1.50 & $-$1.520 &    ... &    ... &    ... &   31.5 &    ... &    ... &    ... &    ... &   40.5 &    ... &    ... \\
Sc II &  6604.58 &   1.36 & $-$1.310 &    ... &   58.0 &    ... &    ... &   49.0 &    ... &   67.5 &   68.5 &   57.0 &   42.7 &    ... \\
Ti I  &  5490.16 &   1.46 & $-$0.933 &    ... &    ... &    ... &    ... &    ... &    ... &   48.7 &    ... &    ... &   31.5 &   24.3 \\
Ti I  &  5978.54 &   1.87 & $-$0.440 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   26.0 &   36.0 &   40.5 \\
Ti I  &  6126.22 &   1.07 & $-$1.425 &    ... &   48.0 &    ... &    ... &    ... &    ... &   53.0 &    ... &   63.3 &   55.5 &    ... \\
Ti I  &  6258.10 &   1.44 & $-$0.355 &    ... &    ... &    ... &    ... &    ... &    ... &   85.0 &    ... &   64.5 &    ... &    ... \\
Ti I  &  6303.77 &   1.44 & $-$1.570 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Ti I  &  6312.24 &   1.46 & $-$1.550 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Ti I  &  6336.10 &   1.44 & $-$1.740 &    ... &    ... &   15.0 &    ... &    ... &    ... &    ... &    ... &    ... &   42.5 &    ... \\
Ti I  &  6554.24 &   1.44 & $-$1.218 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   21.0 &   42.0 &   36.5 \\
Ti I  &  6556.08 &   1.46 & $-$1.074 &    ... &   25.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   39.0 \\
Ti I  &  6599.13 &   0.90 & $-$2.090 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Ti I  &  6743.13 &   0.90 & $-$1.630 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   37.7 \\
Ti II &  5336.77 &   1.58 & $-$1.700 &   77.0 &  138.7 &  100.0 &  100.3 &    ... &   50.0 &  157.0 &   93.5 &  132.5 &  125.0 &  114.0 \\
Ti II &  5381.01 &   1.57 & $-$1.780 &    ... &  110.0 &   83.3 &   62.5 &   73.3 &    ... &  100.0 &  113.3 &  110.0 &    ... &  137.0 \\
Ti II &  5418.77 &   1.58 & $-$2.110 &   48.7 &  108.3 &   92.0 &   73.7 &    ... &   40.0 &  101.0 &   90.0 &   87.0 &   91.5 &    ... \\
Ti II &  6559.59 &   2.05 & $-$2.019 &    ... &    ... &    ... &    ... &    ... &    ... &   69.5 &    ... &    ... &    ... &    ... \\
Ti II &  6606.95 &   2.06 & $-$2.790 &    ... &    ... &    ... &    ... &    ... &   23.5 &    ... &    ... &    ... &    ... &    ... \\
V  I  &  6090.21 &   1.08 & $-$0.060 &    ... &   46.0 &    ... &    ... &    ... &    ... &   43.0 &   50.5 &   46.0 &   48.0 &   35.7 \\
V  I  &  6119.53 &   1.06 & $-$0.320 &   23.5 &   29.0 &    ... &    ... &    ... &    ... &   33.7 &    ... &    ... &   35.0 &   38.3 \\
V  I  &  6135.37 &   1.05 & $-$0.750 &    ... &    ... &    ... &    ... &    ... &    ... &   35.5 &    ... &    ... &    ... &    ... \\
V  I  &  6150.15 &   0.30 & $-$1.790 &    ... &   23.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
V  I  &  6199.19 &   0.29 & $-$1.290 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   50.5 &    ... &   44.0 &    ... \\
V  I  &  6216.36 &   0.28 & $-$0.810 &    ... &   24.5 &    ... &    ... &    ... &    ... &   61.0 &    ... &    ... &   43.0 &   37.7 \\
V  I  &  6224.51 &   0.29 & $-$2.010 &    ... &   18.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
V  I  &  6233.20 &   0.28 & $-$2.070 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   26.5 &    ... \\
V  I  &  6243.11 &   0.30 & $-$0.980 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
V  I  &  6251.82 &   0.29 & $-$1.300 &   18.0 &   21.5 &    ... &    ... &   32.5 &    ... &   30.0 &    ... &   48.0 &    ... &    ... \\
V  I  &  6292.82 &   0.29 & $-$1.520 &    ... &    ... &   26.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
V  I  &  6531.41 &   1.22 & $-$0.840 &    ... &   21.5 &   21.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Cr I  &  5345.80 &   1.00 & $-$0.980 &  107.7 &  134.0 &  131.3 &   85.0 &  130.7 &   63.3 &  171.5 &  143.0 &  162.0 &  134.7 &  146.7 \\
Cr I  &  5348.33 &   1.00 & $-$1.290 &   77.5 &  116.7 &   92.7 &   71.0 &  117.5 &   48.3 &  155.0 &  114.0 &  127.7 &  140.0 &  121.7 \\
Cr I  &  5409.80 &   1.03 & $-$0.720 &  123.0 &  137.7 &  119.7 &   88.0 &  127.7 &   84.3 &  166.5 &  169.0 &  168.0 &  189.7 &  159.7 \\
Cr I  &  6330.09 &   0.94 & $-$2.920 &    ... &   33.3 &   24.5 &    ... &    ... &    ... &   79.0 &   39.5 &   54.0 &   94.0 &   47.0 \\
Mn I  &  5407.42 &   2.14 & $-$1.743 &    ... &    ... &    ... &   28.5 &   35.3 &    ... &   51.5 &    ... &   81.0 &    ... &    ... \\
Mn I  &  5420.36 &   2.14 & $-$1.460 &    ... &    ... &    ... &    ... &    ... &    ... &   93.0 &    ... &   75.0 &    ... &    ... \\
Mn I  &  5432.55 &   0.00 & $-$3.795 &    ... &  110.0 &    ... &    ... &    ... &   37.3 &  107.5 &   74.0 &   91.0 &   59.0 &   93.0 \\
Mn I  &  5516.77 &   2.18 & $-$1.847 &    ... &    ... &    ... &   26.0 &    ... &    ... &    ... &   41.0 &    ... &    ... &   27.5 \\
Mn I  &  6013.51 &   3.07 & $-$0.252 &    ... &   47.7 &    ... &   18.5 &    ... &    ... &    ... &   30.5 &   48.7 &   46.0 &   58.0 \\
Mn I  &  6021.82 &   3.08 &  0.035 &    ... &   59.0 &   62.0 &    ... &    ... &    ... &   97.3 &   67.5 &   60.0 &   30.5 &   68.3 \\
Co I  &  5647.23 &   2.28 & $-$1.560 &    ... &   22.5 &    ... &    ... &    ... &    ... &    ... &    ... &   26.5 &   17.5 &   30.0 \\
Ni I  &  5578.73 &   1.68 & $-$2.670 &    ... &   79.3 &    ... &   36.5 &   36.0 &    ... &   73.0 &   87.5 &   74.5 &   68.0 &   87.3 \\
Ni I  &  5587.87 &   1.93 & $-$2.370 &    ... &    ... &    ... &   30.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Ni I  &  6108.12 &   1.68 & $-$2.450 &   19.5 &   84.3 &   62.5 &   43.0 &   40.0 &    ... &   95.0 &   85.0 &   96.7 &   90.0 &  101.0 \\
Ni I  &  6128.97 &   1.68 & $-$3.390 &    ... &    ... &   23.5 &    ... &    ... &    ... &   48.0 &    ... &   31.7 &   22.0 &    ... \\
Ni I  &  6176.82 &   4.09 & $-$0.430 &    ... &   35.7 &   20.0 &    ... &    ... &    ... &   47.0 &   46.0 &    ... &    ... &   47.0 \\
Ni I  &  6327.60 &   1.68 & $-$3.090 &   24.5 &   78.3 &    ... &    ... &    ... &    ... &   81.3 &   72.0 &   55.0 &   43.5 &   65.0 \\
Ni I  &  6384.67 &   4.15 & $-$1.000 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   21.0 &    ... &    ... \\
Ni I  &  6482.80 &   1.94 & $-$2.850 &    ... &   49.0 &   28.7 &    ... &   24.0 &    ... &   60.3 &   33.7 &   62.0 &   65.0 &   42.0 \\
Ni I  &  6586.32 &   1.95 & $-$2.790 &    ... &   49.0 &   39.3 &    ... &   23.0 &    ... &   60.3 &    ... &   39.7 &   61.0 &   36.7 \\
Ni I  &  6643.64 &   1.68 & $-$2.300 &   57.7 &  115.7 &   78.0 &   66.0 &   46.0 &   37.3 &  143.3 &  121.0 &  128.3 &  144.0 &  122.0 \\
Ni I  &  6767.78 &   1.83 & $-$2.170 &   55.7 &  108.0 &   81.3 &    ... &   51.0 &    ... &  117.0 &   90.3 &   92.0 &  100.0 &  119.3 \\
Cu I  &  5700.24 &   1.64 & $-$2.330 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   21.5 &   18.0 &    ... &    ... \\
Zn I  &  6362.35 &   5.80 &  0.140 &    ... &   23.0 &    ... &    ... &    ... &    ... &    ... &   49.5 &    ... &    ... &    ... \\
Y  II &  5402.78 &   1.84 & $-$0.510 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   23.5 &    ... &   16.0 &    ... \\
Ba II &  5853.69 &   0.60 & $-$1.010 &  120.7 &  138.3 &  137.5 &    ... &  132.7 &    ... &  122.0 &  128.5 &  104.3 &  155.0 &  168.3 \\
Ba II &  6141.73 &   0.70 & $-$0.077 &  152.3 &  190.7 &  160.7 &  117.3 &    ... &    ... &  185.0 &    ... &  173.3 &  174.0 &  151.7 \\
Ba II &  6496.91 &   0.60 & $-$0.380 &  150.7 &  179.7 &  158.0 &  118.7 &  173.7 &   52.0 &  202.0 &  190.0 &  176.0 &  174.7 &  170.0 \\
La II &  5303.52 &   0.32 & $-$1.350 &    ... &   15.5 &    ... &    ... &   25.5 &    ... &   31.5 &   37.5 &   21.5 &    ... &   21.5 \\
La II &  6320.43 &   0.17 & $-$1.562 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
La II &  6390.46 &   0.32 & $-$1.400 &    ... &   44.0 &   60.0 &    ... &    ... &    ... &   38.5 &   37.0 &    ... &   29.5 &   28.5 \\
La II &  6774.27 &   0.13 & $-$1.708 &    ... &    ... &   13.5 &    ... &    ... &    ... &    ... &   37.5 &    ... &    ... &    ... \\
Nd II &  5319.82 &   0.55 & $-$0.140 &    ... &   56.0 &    ... &    ... &   44.0 &    ... &    ... &    ... &    ... &   38.5 &   62.5 \\
Eu II &  6645.13 &   1.37 &  0.120 &   33.7 &   18.7 &    ... &    ... &    ... &   17.5 &   20.5 &   39.0 &    ... &    ... &    ... \\
\enddata                                                                                                                
\tablenotetext{a}{$S/N$ per $\sim$0.28\,{\AA}~pixel at 5300 -- 5700\,{\AA}.}                                                      
\end{deluxetable}                                                                                                       
\end{center}                                                                    


==> table4.tex <==
% Table 4

\begin{center}                                                                                                          
\begin{deluxetable}{lccrrrrrrrrrrr}                                                                                     
\tabletypesize{\tiny}                                                                                                   
\tablecolumns{14}                                                                                                       
\tablewidth{0pt}                                                                                                        
\rotate                                                                                                                 
\tablecaption{\label{tab:ew3} Atomic Data and Equivalent Widths (m{\AA}) for 10 Carina Red Giants}                   
\tablehead{                                                                                                             
\colhead{Species} & {Wavelength} & {$\chi$} & {log$gf$} & {CC10414} & {CC10686} & {CC10690} & {CC10802} & {CC10944} & {CC11217} & {CC11388} & {CC11560} & {CC12038} & {CC12039} \\
{(1)} & {(2)} & {(3)} & {(4)} & {(5)} & {(6)} & {(7)} & {(8)} & {(9)} & {(10)} & {(11)} & {(12)} & {(13)} & {(14)}
}                                                                                                                       
\startdata                                                                                                              

$S/N$\tablenotemark{a}  &  &  &  &       9 &       20 &       14 &        7 &       16 &       16 &       10 &       11 &        8 &       18 \\
W(min)\,(m{\AA})  &  &  &  &      26 &       15 &       25 &       33 &       20 &       22 &       26 &       23 &       24 &       22 \\
Fe I  &  5302.30 &   3.28 & $-$0.880 &  118.5 &  126.3 &   97.0 &    ... &  101.0 &  155.0 &    ... &  106.5 &  132.5 &  141.3 \\
Fe I  &  5307.37 &   1.61 & $-$2.912 &  166.7 &  134.0 &  115.5 &  120.5 &  121.0 &  166.3 &  145.5 &  109.0 &   98.3 &  139.7 \\
Fe I  &  5324.19 &   3.21 & $-$0.100 &    ... &    ... &  130.0 &    ... &    ... &    ... &    ... &    ... &    ... &  178.0 \\
Fe I  &  5332.90 &   1.56 & $-$2.780 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &  155.0 &    ... &    ... \\
Fe I  &  5339.93 &   3.27 & $-$0.720 &  162.5 &  126.3 &  109.0 &  133.7 &  106.7 &  164.3 &    ... &  109.5 &  132.5 &  143.3 \\
Fe I  &  5364.86 &   4.45 &  0.228 &  104.0 &   78.5 &   62.3 &  111.0 &   78.0 &  120.7 &   84.0 &   82.7 &    ... &   97.5 \\
Fe I  &  5367.48 &   4.42 &  0.443 &    ... &  109.0 &   92.3 &    ... &   79.7 &  138.0 &    ... &  104.3 &   97.3 &  104.7 \\
Fe I  &  5369.96 &   4.37 &  0.536 &  134.0 &  100.0 &   75.0 &    ... &   81.7 &  138.5 &    ... &  111.0 &  107.0 &  122.0 \\
Fe I  &  5371.50 &   0.96 & $-$1.644 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5383.37 &   4.31 &  0.645 &  163.0 &  107.0 &   94.3 &    ... &  105.5 &  155.5 &  130.5 &   99.0 &  136.0 &  146.3 \\
Fe I  &  5389.48 &   4.42 & $-$0.400 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   54.5 \\
Fe I  &  5393.17 &   3.24 & $-$0.920 &    ... &    ... &    ... &    ... &    ... &  180.5 &    ... &  138.5 &    ... &  131.5 \\
Fe I  &  5397.13 &   0.91 & $-$1.982 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5400.51 &   4.37 & $-$0.150 &  131.5 &   70.0 &    ... &    ... &   57.5 &  129.7 &   99.5 &   70.0 &    ... &   91.0 \\
Fe I  &  5405.77 &   0.99 & $-$1.852 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5410.92 &   4.47 &  0.398 &  111.7 &   94.7 &   89.0 &    ... &   78.7 &  122.7 &  125.5 &   80.5 &   89.3 &   87.5 \\
Fe I  &  5415.20 &   4.39 &  0.643 &  111.7 &  110.0 &  112.7 &  150.5 &   88.3 &  162.3 &    ... &   81.0 &  114.0 &  122.0 \\
Fe I  &  5417.04 &   4.42 & $-$1.420 &    ... &    ... &    ... &   34.0 &    ... &   23.0 &    ... &    ... &    ... &    ... \\
Fe I  &  5424.07 &   4.32 &  0.520 &  150.5 &  134.0 &   96.0 &  109.0 &  113.0 &    ... &    ... &  162.3 &    ... &  124.7 \\
Fe I  &  5429.70 &   0.96 & $-$1.881 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5434.52 &   1.01 & $-$2.126 &    ... &    ... &  185.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5445.05 &   4.39 & $-$0.020 &  112.3 &   79.7 &   74.5 &  108.0 &   77.0 &  121.0 &  118.5 &   80.3 &   90.7 &   79.7 \\
Fe I  &  5446.92 &   0.99 & $-$1.914 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5464.28 &   4.14 & $-$1.402 &    ... &    ... &    ... &    ... &    ... &   53.5 &    ... &    ... &    ... &    ... \\
Fe I  &  5497.52 &   1.01 & $-$2.825 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  5501.46 &   0.96 & $-$3.046 &  183.5 &  187.5 &  164.0 &    ... &  191.5 &    ... &    ... &  180.5 &  179.0 &  192.0 \\
Fe I  &  5506.79 &   0.99 & $-$2.789 &    ... &    ... &    ... &    ... &  184.5 &    ... &    ... &  185.5 &  171.5 &    ... \\
Fe I  &  5569.62 &   3.42 & $-$0.540 &  120.7 &  132.5 &   95.7 &  120.0 &  115.5 &  177.5 &    ... &  152.5 &  136.0 &  128.7 \\
Fe I  &  5576.09 &   3.43 & $-$1.000 &  115.5 &  116.0 &  102.7 &  113.0 &   77.0 &  146.0 &    ... &  109.3 &  109.3 &  124.0 \\
Fe I  &  5586.76 &   3.37 & $-$0.144 &  164.5 &  153.3 &  128.7 &  142.7 &  142.0 &  196.0 &  160.5 &  139.7 &  141.5 &  167.0 \\
Fe I  &  5624.54 &   3.42 & $-$0.755 &  146.5 &  122.0 &    ... &    ... &  104.5 &    ... &    ... &    ... &    ... &  133.0 \\
Fe I  &  5686.53 &   4.55 & $-$0.450 &  111.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   39.0 &    ... \\
Fe I  &  5701.54 &   2.56 & $-$2.143 &  115.5 &  105.0 &   84.0 &   87.5 &   93.5 &  153.3 &    ... &  100.7 &   89.0 &  105.5 \\
Fe I  &  5956.69 &   0.86 & $-$4.498 &   93.7 &  109.5 &    ... &    ... &  101.0 &  175.3 &  149.0 &   87.0 &    ... &  137.0 \\
Fe I  &  6003.03 &   3.88 & $-$1.110 &  104.7 &   68.0 &   41.0 &    ... &   47.7 &  100.5 &    ... &   67.0 &   73.0 &   69.0 \\
Fe I  &  6024.05 &   4.55 & $-$0.110 &  113.0 &   85.0 &    ... &  135.0 &   45.0 &  105.5 &  103.0 &   62.0 &    ... &   86.3 \\
Fe I  &  6027.05 &   4.07 & $-$1.089 &   70.3 &   41.0 &   28.5 &   57.0 &   28.7 &    ... &   88.0 &    ... &    ... &   50.5 \\
Fe I  &  6056.01 &   4.73 & $-$0.450 &   75.0 &   39.0 &    ... &   31.0 &    ... &   78.0 &    ... &   76.0 &   50.5 &   35.0 \\
Fe I  &  6065.48 &   2.61 & $-$1.410 &  174.0 &  134.3 &   95.0 &  117.0 &  140.3 &  190.0 &    ... &  139.0 &  131.0 &  154.5 \\
Fe I  &  6078.50 &   4.79 & $-$0.370 &   77.0 &   36.3 &    ... &    ... &    ... &   62.3 &    ... &   33.5 &    ... &   52.7 \\
Fe I  &  6082.72 &   2.22 & $-$3.548 &   65.3 &   48.0 &    ... &   70.0 &   19.5 &   85.7 &   45.5 &   27.5 &    ... &    ... \\
Fe I  &  6102.18 &   4.84 & $-$0.516 &    ... &   37.0 &    ... &   75.0 &   21.5 &   66.0 &    ... &   42.0 &   55.0 &   27.5 \\
Fe I  &  6120.26 &   0.91 & $-$5.940 &    ... &   13.0 &    ... &   57.0 &    ... &   56.0 &   27.5 &    ... &    ... &    ... \\
Fe I  &  6137.69 &   2.59 & $-$1.346 &  223.5 &  169.0 &  139.3 &    ... &  161.0 &  204.5 &    ... &  143.7 &  139.7 &  175.0 \\
Fe I  &  6151.62 &   2.18 & $-$3.371 &   68.3 &   69.0 &   52.5 &   69.0 &   52.0 &  114.0 &  100.5 &   63.0 &    ... &   71.3 \\
Fe I  &  6157.75 &   4.07 & $-$1.260 &   58.0 &   52.5 &    ... &   52.0 &    ... &   71.3 &    ... &   43.5 &    ... &   51.7 \\
Fe I  &  6165.36 &   4.14 & $-$1.473 &  144.5 &   30.7 &    ... &    ... &    ... &   55.3 &    ... &    ... &   63.0 &    ... \\
Fe I  &  6173.34 &   2.22 & $-$2.850 &  109.3 &  101.3 &   58.3 &  107.0 &   85.0 &  131.0 &  118.0 &   69.3 &   88.0 &  119.0 \\
Fe I  &  6180.20 &   2.73 & $-$2.649 &   95.0 &   72.7 &   25.0 &    ... &   36.5 &  101.0 &   68.5 &   47.5 &    ... &   72.0 \\
Fe I  &  6187.99 &   3.94 & $-$1.580 &    ... &   31.3 &    ... &    ... &    ... &   57.3 &    ... &    ... &    ... &   36.0 \\
Fe I  &  6200.31 &   2.61 & $-$2.373 &   93.5 &  105.5 &   61.0 &   89.0 &  106.7 &  129.7 &    ... &   97.5 &   87.0 &  119.5 \\
Fe I  &  6213.43 &   2.22 & $-$2.481 &  126.0 &  119.3 &   93.0 &  112.5 &  107.0 &  149.7 &  128.0 &  117.5 &    ... &  133.5 \\
Fe I  &  6219.28 &   2.20 & $-$2.448 &  152.3 &  123.0 &   99.5 &  132.0 &   74.5 &  162.0 &  158.0 &  127.0 &  116.0 &  131.3 \\
Fe I  &  6229.23 &   2.84 & $-$2.900 &    ... &   46.3 &    ... &   50.5 &    ... &   71.7 &    ... &   43.3 &    ... &   33.7 \\
Fe I  &  6230.74 &   2.56 & $-$1.276 &    ... &  180.0 &  146.0 &  160.0 &  156.0 &    ... &    ... &  153.0 &  135.5 &    ... \\
Fe I  &  6232.65 &   3.65 & $-$1.223 &   99.0 &   64.0 &   37.0 &   64.5 &   42.7 &  111.7 &    ... &   84.0 &   72.7 &   55.3 \\
Fe I  &  6240.65 &   2.22 & $-$3.173 &   77.0 &   73.0 &   36.5 &   82.7 &   47.7 &  116.0 &    ... &    ... &  112.5 &   75.0 \\
Fe I  &  6246.32 &   3.60 & $-$0.733 &  115.5 &  104.3 &    ... &   99.3 &   92.3 &  125.0 &  102.5 &   94.0 &   55.7 &  119.5 \\
Fe I  &  6252.56 &   2.40 & $-$1.767 &  161.0 &  162.0 &  127.0 &  166.7 &  148.3 &  204.0 &  161.5 &  156.7 &  151.0 &  165.5 \\
Fe I  &  6254.26 &   2.28 & $-$2.443 &  162.3 &  124.7 &   89.5 &  124.0 &  113.3 &  171.3 &    ... &  124.7 &  107.3 &  137.5 \\
Fe I  &  6265.13 &   2.18 & $-$2.540 &  138.0 &  121.7 &   91.0 &  128.0 &  116.3 &  177.0 &    ... &  125.5 &  109.5 &  136.0 \\
Fe I  &  6280.62 &   0.86 & $-$4.387 &  152.0 &  139.0 &   98.5 &  112.5 &  117.5 &  181.0 &    ... &   98.5 &  116.5 &  123.0 \\
Fe I  &  6297.79 &   2.22 & $-$2.640 &  138.5 &  129.5 &    ... &  111.7 &    ... &  169.0 &    ... &   52.5 &  118.7 &  122.0 \\
Fe I  &  6301.50 &   3.65 & $-$0.720 &  119.5 &  104.0 &   74.0 &  126.0 &    ... &  141.5 &    ... &   92.0 &   93.7 &  127.5 \\
Fe I  &  6302.49 &   3.69 & $-$1.150 &    ... &   71.0 &    ... &  106.0 &    ... &   90.0 &    ... &    ... &    ... &    ... \\
Fe I  &  6311.51 &   2.83 & $-$3.220 &   69.0 &   36.3 &    ... &    ... &    ... &   60.3 &    ... &   40.0 &    ... &   40.7 \\
Fe I  &  6322.68 &   2.59 & $-$2.469 &  105.7 &  118.7 &   89.0 &   75.3 &   99.3 &  151.3 &    ... &   96.7 &    ... &  101.3 \\
Fe I  &  6335.33 &   2.20 & $-$2.177 &  190.3 &  143.7 &  122.5 &  133.7 &  129.7 &  188.0 &    ... &  132.7 &  117.0 &  143.0 \\
Fe I  &  6336.82 &   3.69 & $-$1.050 &  124.0 &   94.3 &   67.0 &    ... &   80.3 &  131.0 &    ... &    ... &   99.0 &   98.0 \\
Fe I  &  6344.15 &   2.43 & $-$2.877 &  162.3 &   78.7 &   56.0 &   93.0 &   64.0 &  117.3 &    ... &   66.3 &   54.3 &   79.5 \\
Fe I  &  6355.03 &   2.84 & $-$2.291 &  109.3 &   71.3 &   40.0 &   96.3 &   61.0 &  121.3 &    ... &   82.0 &   67.5 &   69.7 \\
Fe I  &  6380.74 &   4.19 & $-$1.375 &   55.5 &    ... &    ... &   59.3 &    ... &   41.5 &    ... &   26.5 &    ... &   27.3 \\
Fe I  &  6392.54 &   2.28 & $-$3.950 &    ... &    ... &    ... &    ... &    ... &   51.5 &    ... &    ... &    ... &    ... \\
Fe I  &  6393.61 &   2.43 & $-$1.576 &    ... &  183.5 &  128.7 &  138.5 &  135.3 &  207.5 &    ... &  167.0 &  148.5 &    ... \\
Fe I  &  6408.03 &   3.69 & $-$1.000 &  113.3 &   80.7 &   44.0 &   96.0 &   68.5 &  118.0 &    ... &   80.0 &   75.3 &   89.7 \\
Fe I  &  6411.65 &   3.65 & $-$0.717 &  126.5 &  114.0 &    ... &  142.5 &   98.3 &  142.7 &    ... &    ... &    ... &  138.0 \\
Fe I  &  6419.96 &   4.73 & $-$0.240 &   73.0 &   46.3 &    ... &   65.0 &    ... &   84.0 &    ... &    ... &    ... &   62.0 \\
Fe I  &  6421.35 &   2.28 & $-$2.014 &  174.5 &  157.0 &  124.7 &  150.0 &  139.0 &  197.3 &    ... &    ... &  120.5 &  148.3 \\
Fe I  &  6430.85 &   2.18 & $-$1.946 &  164.3 &  159.7 &  123.3 &  163.0 &  124.0 &  210.0 &    ... &  156.5 &  147.5 &  160.3 \\
Fe I  &  6481.87 &   2.27 & $-$3.010 &  117.3 &   57.0 &   54.5 &   94.3 &   94.0 &  132.3 &   98.0 &   91.0 &   92.0 &   97.3 \\
Fe I  &  6494.98 &   2.40 & $-$1.239 &    ... &  177.7 &  157.7 &  178.5 &  173.7 &  213.5 &    ... &  189.3 &  151.0 &  189.0 \\
Fe I  &  6498.94 &   0.96 & $-$4.689 &  123.0 &  101.7 &   77.3 &  114.3 &   96.7 &  125.0 &  104.5 &   84.0 &   57.0 &  103.0 \\
Fe I  &  6518.37 &   2.83 & $-$2.297 &  101.0 &   71.0 &    ... &   57.7 &   59.7 &   98.7 &    ... &   73.0 &   32.5 &   60.0 \\
Fe I  &  6533.93 &   4.55 & $-$1.460 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   39.5 &    ... &    ... \\
Fe I  &  6569.22 &   4.73 & $-$0.420 &   44.5 &   44.5 &   26.0 &    ... &   46.0 &   67.0 &   45.0 &   44.5 &   44.5 &   40.5 \\
Fe I  &  6574.23 &   0.99 & $-$5.022 &    ... &   80.0 &   27.0 &    ... &   82.0 &  125.0 &    ... &   51.5 &   79.7 &   82.3 \\
Fe I  &  6581.22 &   1.48 & $-$4.680 &   65.5 &   63.0 &   23.5 &    ... &   32.7 &   84.0 &    ... &    ... &    ... &   41.0 \\
Fe I  &  6592.91 &   2.73 & $-$1.470 &  171.7 &  154.3 &  120.0 &  151.0 &  136.7 &  193.0 &  134.0 &  164.0 &  130.0 &  150.3 \\
Fe I  &  6593.87 &   2.43 & $-$2.366 &  156.0 &  129.3 &   99.0 &    ... &   93.0 &  156.0 &  115.5 &  121.0 &  102.7 &  134.0 \\
Fe I  &  6597.56 &   4.79 & $-$1.070 &    ... &    ... &    ... &    ... &    ... &   32.0 &    ... &    ... &    ... &    ... \\
Fe I  &  6608.03 &   2.28 & $-$3.940 &    ... &   18.0 &    ... &    ... &    ... &   51.7 &    ... &    ... &   33.0 &    ... \\
Fe I  &  6609.11 &   2.56 & $-$2.661 &  123.5 &   92.0 &   50.3 &   99.7 &   76.0 &  135.5 &    ... &   72.0 &   58.7 &   66.0 \\
Fe I  &  6627.54 &   4.54 & $-$1.680 &    ... &    ... &    ... &    ... &    ... &   30.0 &    ... &    ... &   27.3 &    ... \\
Fe I  &  6633.75 &   4.56 & $-$0.799 &    ... &   40.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe I  &  6663.44 &   2.42 & $-$2.479 &  109.5 &  115.3 &   96.0 &    ... &  110.0 &  167.3 &    ... &    ... &  113.5 &  113.0 \\
Fe I  &  6677.99 &   2.69 & $-$1.420 &    ... &  163.5 &  134.5 &  170.0 &  169.0 &  192.3 &    ... &    ... &  122.0 &  173.7 \\
Fe I  &  6750.15 &   2.42 & $-$2.621 &    ... &  110.0 &   70.0 &  116.0 &   92.5 &  140.3 &    ... &   86.0 &    ... &  104.3 \\
Fe II &  5414.08 &   3.22 & $-$3.610 &    ... &   23.0 &    ... &   32.0 &   35.0 &   21.5 &    ... &   16.0 &   26.0 &    ... \\
Fe II &  5425.25 &   3.20 & $-$3.360 &   35.3 &    ... &   48.7 &   66.5 &    ... &   61.5 &    ... &    ... &    ... &    ... \\
Fe II &  5534.85 &   3.24 & $-$2.920 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   75.0 &    ... &   60.0 \\
Fe II &  5991.38 &   3.15 & $-$3.740 &   40.3 &   19.5 &   20.0 &    ... &   27.7 &   39.0 &    ... &    ... &    ... &   23.0 \\
Fe II &  6149.25 &   3.89 & $-$2.720 &   44.3 &   29.7 &    ... &   56.0 &    ... &    ... &    ... &    ... &    ... &    ... \\
Fe II &  6238.38 &   3.89 & $-$2.670 &   29.3 &   23.7 &   33.5 &    ... &   28.0 &   48.0 &    ... &    ... &   54.3 &   44.7 \\
Fe II &  6247.56 &   3.89 & $-$2.360 &   51.7 &   32.7 &   38.3 &   86.3 &   47.3 &   61.0 &    ... &   31.0 &   55.0 &   40.0 \\
Fe II &  6369.46 &   2.89 & $-$4.020 &    ... &   16.5 &    ... &    ... &   23.0 &    ... &    ... &   50.5 &    ... &   18.5 \\
Fe II &  6416.93 &   3.89 & $-$2.790 &   42.0 &   25.7 &   18.0 &    ... &    ... &   37.3 &    ... &   19.0 &   40.0 &    ... \\
Fe II &  6432.68 &   2.89 & $-$3.710 &   61.5 &   37.3 &   37.7 &   44.7 &   40.3 &   47.7 &    ... &   41.3 &   39.5 &   44.7 \\
Fe II &  6456.39 &   3.90 & $-$2.080 &   62.0 &   52.5 &   56.3 &    ... &   63.5 &   78.0 &    ... &   82.0 &   98.3 &   64.0 \\
Fe II &  6516.08 &   2.89 & $-$3.450 &   65.3 &   60.0 &   49.0 &    ... &   56.0 &   63.7 &    ... &   68.0 &   52.0 &   58.5 \\
O  I  &  6300.31 &   0.00 & $-$9.750 &   49.5 &   36.7 &  $<$25.0 &    ... &   15.5 &   42.0 &    ... &   33.0 &    ... &   35.5 \\
Na I  &  5688.21 &   2.10 & $-$0.370 &   27.5 &   44.0 &  $<$25.0 &   40.5 &   18.5 &   78.5 &    ... &   74.7 &   43.0 &   47.5 \\
Mg I  &  5528.41 &   4.34 & $-$0.480 &  191.5 &  172.7 &   90.7 &  182.7 &  153.0 &  195.0 &  195.5 &  138.0 &  167.0 &  182.3 \\
Mg I  &  5711.09 &   4.35 & $-$1.728 &   69.3 &   66.7 &    ... &   41.7 &   47.0 &   92.7 &    ... &   65.7 &    ... &   75.3 \\
Al I  &  6696.03 &   3.14 & $-$1.570 &    ... &  $<$20.0 &  $<$25.0 &  $<$35.0 &  $<$30.0 &  $<$25.0 &  $<$25.0 &    ... &    ... &  $<$20.0 \\
Si I  &  6142.48 &   5.62 & $-$1.510 &   19.0 &    ... &    ... &   28.5 &    ... &    ... &    ... &    ... &   34.5 &    ... \\
Si I  &  6155.14 &   5.62 & $-$0.800 &   42.0 &    ... &    ... &   56.5 &   26.0 &   31.3 &    ... &    ... &   27.5 &   28.0 \\
Si I  &  6237.33 &   5.61 & $-$1.020 &   37.0 &   17.7 &    ... &    ... &    ... &   29.3 &    ... &   19.5 &   19.5 &    ... \\
Si I  &  6244.48 &   5.61 & $-$1.270 &    ... &    ... &    ... &    ... &    ... &   22.5 &    ... &    ... &    ... &    ... \\
Ca I  &  5349.47 &   2.71 & $-$0.310 &  101.5 &    ... &   51.5 &    ... &   53.0 &    ... &    ... &   83.5 &    ... &    ... \\
Ca I  &  5581.97 &   2.52 & $-$0.555 &   93.7 &   82.0 &   34.0 &    ... &   62.0 &  118.7 &    ... &   73.0 &    ... &   96.3 \\
Ca I  &  5588.75 &   2.52 &  0.210 &  157.7 &  123.0 &   73.5 &  131.0 &  119.7 &  166.7 &  117.0 &  116.7 &  119.7 &  143.3 \\
Ca I  &  5590.12 &   2.52 & $-$0.571 &  122.5 &   83.5 &    ... &    ... &   55.3 &  124.0 &    ... &    ... &   86.0 &   68.7 \\
Ca I  &  5594.47 &   2.52 &  0.097 &    ... &    ... &   78.5 &    ... &  104.0 &  177.0 &    ... &    ... &    ... &    ... \\
Ca I  &  5598.49 &   2.52 & $-$0.087 &  171.5 &    ... &    ... &  183.5 &    ... &    ... &    ... &    ... &    ... &    ... \\
Ca I  &  5857.45 &   2.93 &  0.230 &    ... &    ... &   56.3 &  134.0 &   92.0 &  153.0 &    ... &    ... &  136.5 &  119.5 \\
Ca I  &  5601.28 &   2.53 & $-$0.523 &    ... &   88.0 &   40.7 &   53.5 &   64.0 &  117.0 &   75.5 &    ... &   72.7 &   72.7 \\
Ca I  &  6102.73 &   1.88 & $-$0.790 &  138.5 &  136.5 &   60.0 &  112.5 &  110.3 &  159.5 &    ... &  133.0 &  118.3 &   84.5 \\
Ca I  &  6122.23 &   1.89 & $-$0.320 &  181.3 &  160.0 &  103.0 &    ... &  147.3 &  209.0 &  177.5 &  156.0 &  143.7 &  164.0 \\
Ca I  &  6161.30 &   2.52 & $-$1.270 &   81.5 &   38.7 &    ... &    ... &    ... &   82.0 &   91.5 &   39.5 &   35.7 &   47.0 \\
Ca I  &  6162.17 &   1.90 & $-$0.090 &  169.0 &  178.0 &  127.0 &    ... &  168.0 &  220.0 &  198.0 &  189.0 &  155.0 &  181.7 \\
Ca I  &  6166.44 &   2.52 & $-$1.140 &   66.3 &   49.7 &   27.5 &    ... &   29.5 &   67.0 &    ... &   48.5 &   21.7 &   45.0 \\
Ca I  &  6169.04 &   2.52 & $-$0.800 &   96.0 &   81.0 &    ... &    ... &   64.0 &  119.5 &    ... &   92.5 &   75.5 &   75.5 \\
Ca I  &  6169.56 &   2.52 & $-$0.480 &  103.0 &   90.0 &   38.0 &  127.5 &   64.0 &  121.5 &    ... &   89.0 &  105.0 &  100.0 \\
Ca I  &  6439.08 &   2.52 &  0.390 &  208.5 &  147.0 &   92.7 &  129.3 &  145.3 &  184.5 &    ... &  155.0 &  150.7 &  155.0 \\
Ca I  &  6449.81 &   2.52 & $-$0.502 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &  100.5 &    ... \\
Ca I  &  6455.60 &   2.52 & $-$1.290 &   99.5 &   39.0 &    ... &   91.0 &   23.0 &   72.7 &    ... &    ... &    ... &   40.0 \\
Ca I  &  6471.67 &   2.52 & $-$0.760 &  109.0 &   89.0 &   15.0 &   92.3 &   71.5 &  111.7 &    ... &   88.0 &  115.7 &   91.0 \\
Ca I  &  6493.79 &   2.52 & $-$0.320 &  103.7 &  113.7 &   64.3 &  116.7 &   53.7 &  141.0 &  129.5 &  103.5 &   80.0 &  122.5 \\
Ca I  &  6499.65 &   2.52 & $-$0.820 &   77.7 &   71.3 &    ... &   88.7 &   49.5 &  107.0 &    ... &   67.0 &   73.7 &   73.0 \\
Ca I  &  6717.68 &   2.71 & $-$0.610 &  130.5 &   80.7 &   37.7 &   90.3 &   68.0 &  125.3 &    ... &   92.0 &    ... &   93.7 \\
Sc II &  5318.37 &   1.36 & $-$2.010 &   41.0 &   24.0 &    ... &    ... &    ... &   27.0 &    ... &    ... &    ... &   23.0 \\
Sc II &  5526.79 &   1.77 &  0.030 &  114.0 &   88.5 &   68.0 &  102.3 &   79.7 &  125.5 &    ... &   96.5 &  101.5 &  109.7 \\
Sc II &  5641.00 &   1.50 & $-$1.130 &   60.0 &   64.0 &    ... &   55.0 &    ... &   56.0 &    ... &    ... &   41.7 &   62.0 \\
Sc II &  5657.91 &   1.51 & $-$0.600 &    ... &    ... &    ... &   75.5 &   89.0 &    ... &    ... &   88.5 &   71.5 &    ... \\
Sc II &  5667.16 &   1.50 & $-$1.310 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Sc II &  5669.06 &   1.50 & $-$1.200 &    ... &   71.0 &    ... &    ... &   48.5 &   90.0 &    ... &    ... &    ... &   69.3 \\
Sc II &  6245.62 &   1.51 & $-$0.970 &   57.0 &   59.0 &    ... &    ... &   42.5 &   82.5 &    ... &    ... &    ... &    ... \\
Sc II &  6309.90 &   1.50 & $-$1.520 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   61.0 &    ... &   38.5 \\
Sc II &  6604.58 &   1.36 & $-$1.310 &    ... &   47.3 &    ... &    ... &    ... &   72.7 &    ... &   56.7 &    ... &   52.7 \\
Ti I  &  5490.16 &   1.46 & $-$0.933 &    ... &   37.0 &    ... &    ... &    ... &   66.5 &    ... &    ... &   34.0 &   23.0 \\
Ti I  &  5978.54 &   1.87 & $-$0.440 &    ... &   20.7 &    ... &    ... &    ... &    ... &    ... &   21.0 &    ... &    ... \\
Ti I  &  6126.22 &   1.07 & $-$1.425 &   50.0 &   45.0 &    ... &    ... &   31.5 &   91.3 &    ... &   35.0 &    ... &   39.5 \\
Ti I  &  6258.10 &   1.44 & $-$0.355 &   88.0 &    ... &    ... &   70.5 &    ... &    ... &    ... &    ... &   53.5 &    ... \\
Ti I  &  6303.77 &   1.44 & $-$1.570 &   23.0 &    ... &    ... &    ... &    ... &   33.3 &    ... &   26.0 &   24.0 &    ... \\
Ti I  &  6312.24 &   1.46 & $-$1.550 &    ... &    ... &    ... &    ... &    ... &   33.7 &    ... &    ... &    ... &   19.0 \\
Ti I  &  6336.10 &   1.44 & $-$1.740 &    ... &    ... &    ... &   56.5 &    ... &   30.0 &    ... &   24.5 &   19.5 &    ... \\
Ti I  &  6554.24 &   1.44 & $-$1.218 &    ... &   27.3 &    ... &    ... &    ... &   59.0 &    ... &    ... &    ... &   28.5 \\
Ti I  &  6556.08 &   1.46 & $-$1.074 &   38.0 &   30.3 &    ... &    ... &    ... &   58.0 &    ... &    ... &   23.0 &   28.5 \\
Ti I  &  6599.13 &   0.90 & $-$2.090 &    ... &    ... &    ... &    ... &    ... &   42.7 &    ... &    ... &    ... &    ... \\
Ti I  &  6743.13 &   0.90 & $-$1.630 &    ... &   44.0 &    ... &   86.3 &    ... &   78.0 &    ... &    ... &    ... &    ... \\
Ti II &  5336.77 &   1.58 & $-$1.700 &  123.7 &  119.0 &   92.5 &    ... &  116.0 &    ... &    ... &  100.5 &  134.3 &  133.5 \\
Ti II &  5381.01 &   1.57 & $-$1.780 &  106.7 &   94.0 &   68.7 &    ... &   75.7 &  141.0 &    ... &    ... &  108.5 &    ... \\
Ti II &  5418.77 &   1.58 & $-$2.110 &   85.0 &   88.3 &    ... &   94.7 &   90.5 &  111.7 &    ... &   72.0 &    ... &   88.3 \\
Ti II &  6559.59 &   2.05 & $-$2.019 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   58.0 \\
Ti II &  6606.95 &   2.06 & $-$2.790 &    ... &    ... &   29.0 &    ... &    ... &   41.5 &    ... &    ... &    ... &    ... \\
V  I  &  6090.21 &   1.08 & $-$0.060 &    ... &   43.0 &    ... &   39.5 &   23.0 &   82.7 &    ... &    ... &    ... &   53.5 \\
V  I  &  6119.53 &   1.06 & $-$0.320 &    ... &   27.3 &    ... &    ... &    ... &   59.7 &    ... &    ... &   22.0 &   27.5 \\
V  I  &  6135.37 &   1.05 & $-$0.750 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
V  I  &  6150.15 &   0.30 & $-$1.790 &    ... &    ... &    ... &    ... &   22.7 &   42.3 &    ... &    ... &    ... &    ... \\
V  I  &  6199.19 &   0.29 & $-$1.290 &    ... &    ... &    ... &    ... &    ... &   91.7 &    ... &    ... &    ... &    ... \\
V  I  &  6216.36 &   0.28 & $-$0.810 &   45.0 &   41.0 &    ... &    ... &    ... &   97.3 &    ... &   60.0 &    ... &   39.7 \\
V  I  &  6224.51 &   0.29 & $-$2.010 &    ... &    ... &    ... &    ... &    ... &   45.7 &    ... &    ... &    ... &    ... \\
V  I  &  6233.20 &   0.28 & $-$2.070 &   34.7 &    ... &    ... &    ... &    ... &   40.5 &    ... &   24.0 &    ... &    ... \\
V  I  &  6243.11 &   0.30 & $-$0.980 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
V  I  &  6251.82 &   0.29 & $-$1.300 &   56.0 &   33.5 &    ... &   33.0 &    ... &   78.7 &    ... &    ... &    ... &    ... \\
V  I  &  6292.82 &   0.29 & $-$1.520 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
V  I  &  6531.41 &   1.22 & $-$0.840 &    ... &    ... &    ... &    ... &    ... &   25.3 &    ... &    ... &    ... &    ... \\
Cr I  &  5345.80 &   1.00 & $-$0.980 &  133.5 &  142.5 &  106.5 &  135.5 &  127.3 &  207.0 &    ... &  130.0 &   90.0 &  165.0 \\
Cr I  &  5348.33 &   1.00 & $-$1.290 &  145.3 &  127.7 &   83.7 &  134.0 &  119.3 &  166.3 &    ... &  105.7 &   92.7 &  126.0 \\
Cr I  &  5409.80 &   1.03 & $-$0.720 &  169.5 &  163.3 &   97.3 &  188.0 &  147.3 &  212.0 &    ... &  132.7 &  157.5 &  166.3 \\
Cr I  &  6330.09 &   0.94 & $-$2.920 &   69.0 &   29.7 &    ... &    ... &    ... &   62.5 &    ... &   36.7 &   38.0 &   31.7 \\
Mn I  &  5407.42 &   2.14 & $-$1.743 &   31.0 &    ... &    ... &    ... &    ... &  103.0 &    ... &    ... &    ... &    ... \\
Mn I  &  5420.36 &   2.14 & $-$1.460 &    ... &    ... &    ... &    ... &    ... &  117.3 &    ... &    ... &    ... &   47.0 \\
Mn I  &  5432.55 &   0.00 & $-$3.795 &   82.3 &   83.0 &    ... &    ... &   41.0 &  160.5 &    ... &    ... &   63.0 &   94.0 \\
Mn I  &  5516.77 &   2.18 & $-$1.847 &   47.0 &    ... &    ... &    ... &    ... &   72.0 &    ... &   32.5 &   32.0 &   24.0 \\
Mn I  &  6013.51 &   3.07 & $-$0.252 &   63.0 &   27.7 &    ... &    ... &    ... &   90.7 &    ... &    ... &    ... &    ... \\
Mn I  &  6021.82 &   3.08 &  0.035 &  123.3 &   65.0 &    ... &   80.3 &   38.0 &  101.7 &    ... &   51.5 &    ... &   74.5 \\
Co I  &  5647.23 &   2.28 & $-$1.560 &    ... &   24.5 &    ... &   49.5 &    ... &   23.0 &    ... &    ... &    ... &   21.0 \\
Ni I  &  5578.73 &   1.68 & $-$2.670 &   78.5 &   75.5 &    ... &   65.5 &    ... &  119.3 &    ... &   59.5 &   62.5 &   85.0 \\
Ni I  &  5587.87 &   1.93 & $-$2.370 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   53.5 &    ... \\
Ni I  &  6108.12 &   1.68 & $-$2.450 &  116.0 &   97.3 &   29.0 &    ... &   64.0 &  114.0 &  108.5 &   67.0 &   86.5 &   72.3 \\
Ni I  &  6128.97 &   1.68 & $-$3.390 &   25.5 &   48.0 &    ... &   58.0 &    ... &   65.7 &    ... &    ... &    ... &   35.0 \\
Ni I  &  6176.82 &   4.09 & $-$0.430 &   58.0 &    ... &    ... &    ... &   21.5 &   48.5 &    ... &    ... &    ... &   28.7 \\
Ni I  &  6327.60 &   1.68 & $-$3.090 &   71.5 &   44.0 &    ... &    ... &    ... &   95.0 &    ... &    ... &    ... &   66.0 \\
Ni I  &  6384.67 &   4.15 & $-$1.000 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Ni I  &  6482.80 &   1.94 & $-$2.850 &   43.7 &   48.3 &   24.5 &   41.5 &   30.5 &   79.3 &    ... &    ... &   52.3 &   49.7 \\
Ni I  &  6586.32 &   1.95 & $-$2.790 &   65.0 &   48.5 &    ... &    ... &   35.0 &   76.3 &    ... &   35.0 &    ... &   44.7 \\
Ni I  &  6643.64 &   1.68 & $-$2.300 &  120.3 &  119.7 &   59.3 &  130.7 &  101.3 &  170.0 &    ... &  137.5 &   98.3 &  136.5 \\
Ni I  &  6767.78 &   1.83 & $-$2.170 &  109.3 &  109.3 &   65.5 &   77.3 &   96.0 &  126.7 &    ... &    ... &   70.0 &  105.0 \\
Cu I  &  5700.24 &   1.64 & $-$2.330 &   40.0 &   15.0 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Zn I  &  6362.35 &   5.80 &  0.140 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Y  II &  5402.78 &   1.84 & $-$0.510 &    ... &    ... &    ... &    ... &    ... &   14.0 &    ... &    ... &    ... &    ... \\
Ba II &  5853.69 &   0.60 & $-$1.010 &   93.0 &  122.0 &   91.5 &  113.0 &  128.0 &  153.7 &  126.0 &  114.0 &  145.7 &  138.0 \\
Ba II &  6141.73 &   0.70 & $-$0.077 &  168.7 &  186.3 &  138.3 &  154.0 &  184.0 &  214.0 &  194.5 &  214.5 &  187.5 &  189.0 \\
Ba II &  6496.91 &   0.60 & $-$0.380 &  187.3 &  178.0 &  124.7 &  200.5 &  174.0 &  197.5 &    ... &  174.3 &  166.0 &  183.7 \\
La II &  5303.52 &   0.32 & $-$1.350 &   23.0 &   18.0 &    ... &    ... &   16.0 &   26.0 &    ... &    ... &    ... &    ... \\
La II &  6320.43 &   0.17 & $-$1.562 &   31.0 &   30.0 &    ... &    ... &    ... &   23.5 &    ... &    ... &    ... &    ... \\
La II &  6390.46 &   0.32 & $-$1.400 &    ... &    ... &    ... &    ... &    ... &   36.5 &    ... &    ... &   32.0 &    ... \\
La II &  6774.27 &   0.13 & $-$1.708 &    ... &    ... &    ... &    ... &    ... &   30.5 &    ... &   44.5 &    ... &    ... \\
Nd II &  5319.82 &   0.55 & $-$0.140 &   77.5 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... \\
Eu II &  6645.13 &   1.37 &  0.120 &   37.0 &   18.0 &    ... &    ... &    ... &   36.3 &    ... &    ... &    ... &   24.0 \\
\enddata                                                                                                                
\tablenotetext{a}{$S/N$ per $\sim$0.28\,{\AA}~pixel at 5300 -- 5700\,{\AA}.}                                                      
\end{deluxetable}                                                                                                       
\end{center}                                                                                                            


==> table5.tex <==
 % Table 5

\begin{deluxetable}{ccccccc}                                                                                                                  
\tablecolumns{6}                                                                                                                            
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{\label{tab:atpar} Model Atmosphere Parameters for 32 Carina Red Giants}                  
\tablehead{                                                                                                                              
  \colhead{Object}  & {$T_{\rm eff}$} & {$\sigma$T$_{\rm eff}$} & {log~$gf$} & {[M/H]} & {$\xi_t$}     \\  
             {}     & {(K)}   & {(K)}             & {(cgs)} & {(dex)}  & {\rm km~s$^{-1}$}    \\        
           {(1)}    & {(2)}   & {(3)}             & {(4)}   & {(5)}    & {(6)}   
  }                                                                                                                                       

\startdata                                                                                                                               
CC06122 & 4284 &  60 & 0.68 &  $-$1.5 &  2.30  \\
CC06486 & 4524 &  62 & 1.07 &  $-$2.0 &  1.95  \\
CC06975 & 4563 &  84 & 1.18 &  $-$1.8 &  2.30  \\
CC07452 & 4437 &  65 & 0.87 &  $-$1.3 &  2.30  \\
CC07889 & 4675 &  55 & 1.31 &  $-$2.3 &  2.30  \\
CC08447 & 4418 &  72 & 0.93 &  $-$1.5 &  2.15  \\
CC08469 & 4337 &  68 & 0.81 &  $-$1.5 &  2.25  \\
CC08615 & 4651 &  84 & 1.28 &  $-$1.7 &  2.40  \\
CC08695 & 4337 &  89 & 0.84 &  $-$1.3 &  2.10  \\
CC08788 & 4695 &  82 & 1.34 &  $-$1.5 &  2.45  \\
CC09000 & 4230 & 116 & 0.67 &  $-$1.8 &  2.40  \\
CC09179 & 4561 &  87 & 1.15 &  $-$1.8 &  1.85  \\
CC09225 & 4438 &  93 & 0.95 &  $-$1.6 &  2.15  \\
CC09226 & 4619 &  76 & 1.19 &  $-$1.5 &  1.90  \\
CC09430 & 4509 &  74 & 1.10 &  $-$2.1 &  1.95  \\
CC09507 & 4652 &  63 & 1.20 &  $-$1.7 &  2.15  \\
CC09633 & 4487 &  80 & 0.93 &  $-$2.2 &  2.40  \\
CC09869 & 4459 &  74 & 1.01 &  $-$1.3 &  2.10  \\
CC09929 & 4515 &  73 & 1.19 &  $-$1.5 &  2.10  \\
CC10038 & 4486 &  73 & 1.08 &  $-$1.2 &  1.95  \\
CC10194 & 4352 &  98 & 0.80 &  $-$1.7 &  2.05  \\
CC10318 & 4359 &  69 & 0.89 &  $-$1.5 &  2.10  \\
CC10414 & 4442 &  66 & 1.01 &  $-$1.4 &  2.30  \\
CC10686 & 4312 &  73 & 0.76 &  $-$1.6 &  2.05  \\
CC10690 & 4486 &  78 & 1.04 &  $-$1.9 &  2.25  \\
CC10802 & 4587 &  72 & 1.30 &  $-$1.3 &  2.00  \\
CC10944 & 4425 &  69 & 0.85 &  $-$1.9 &  2.40  \\
CC11217 & 4279 &  78 & 0.69 &  $-$1.4 &  2.30  \\
CC11388 & 4454 &  81 & 0.93 &  $-$1.5 &  2.45  \\
CC11560 & 4514 &  68 & 1.06 &  $-$1.5 &  2.20  \\
CC12038 & 4551 &  73 & 1.19 &  $-$1.6 &  1.95  \\
CC12039 & 4412 &  65 & 0.84 &  $-$1.6 &  2.35  \\
\enddata                                                                       
\end{deluxetable}      


==> table6.tex <==
% Table 6

\begin{deluxetable}{lrrrrrr}                                                                                                                  
\tablecolumns{7}                                                                                                                            
\tablewidth{0pt}
\tabletypesize{\tiny}
\tablecaption{\label{tab:abund_gil} Chemical Abundances for 32 Carina Red Giants}                  
\tablehead{                                                                                                                              
  \colhead{Species}  & {log\,$\epsilon$} & {s.e.$_{\log\epsilon}$} & {N}   & {[X/Fe]}  & {$\sigma_{\rm {Sys}}$[X/Fe]}  & {$\sigma_{\rm {Tot}}$[X/Fe]}    \\  
           {(1)}     & {(2)}             & {(3)}                  & {(4)} & {(5)}      & {(6)}                        & {(7)}    
  }                                                                                                                                       
\startdata                                                                                                                               

    CC06122&            &            &            &            &            &            \\ 
   Fe I    &     6.07   &     0.02   &       74   &    $-$1.43\tablenotemark{a}   &     0.14   &     0.14   \\ 
   O I     &     7.58   &     0.17   &        1   &     0.32   &     0.13   &     0.21   \\ 
   Na I    &     4.61   &     0.17   &        1   &    $-$0.20   &     0.08   &     0.19   \\ 
   Mg I    &     6.48   &     0.18   &        2   &     0.31   &     0.03   &     0.18   \\ 
   Al I    &  $<$5.38   &     0.17   &        1   &  $<$0.36   &     0.10   &     0.20   \\ 
   Si I    &     6.29   &     0.17   &        1   &     0.21   &     0.14   &     0.22   \\ 
   Ca I    &     5.09   &     0.04   &       19   &     0.09   &     0.02   &     0.04   \\ 
   Sc II   &     1.89   &     0.14   &        5   &     0.17   &     0.11   &     0.18   \\ 
   Ti I    &     3.67   &     0.04   &        8   &     0.15   &     0.09   &     0.10   \\ 
   Ti II   &     3.86   &     0.08   &        2   &     0.34   &     0.10   &     0.13   \\ 
   V I     &     2.43   &     0.11   &       10   &    $-$0.07   &     0.11   &     0.16   \\ 
   Cr I    &     4.20   &     0.06   &        4   &    $-$0.01   &     0.08   &     0.10   \\ 
   Mn I    &     3.68   &     0.04   &        5   &    $-$0.32   &     0.06   &     0.07   \\ 
   Fe II   &     6.16   &     0.04   &        8   &     0.09   &     0.17   &     0.17   \\ 
   Co I    &     3.53   &     0.17   &        1   &    $-$0.03   &     0.08   &     0.19   \\ 
   Ni I    &     4.71   &     0.07   &       10   &    $-$0.08   &     0.05   &     0.09   \\ 
   Cu I    &     2.13   &     0.17   &        1   &    $-$0.63   &     0.08   &     0.19   \\ 
   Ba II   &     1.19   &     0.08   &        3   &     0.44   &     0.11   &     0.14   \\ 
   La II   &     0.16   &     0.08   &        3   &     0.49   &     0.10   &     0.13   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &     0.13   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC06486 &          &            &            &            &            &            \\ 
   Fe I    &     5.47   &     0.04   &       42   &    $-$2.03\tablenotemark{a}   &     0.16   &     0.16   \\ 
   O I     &  $<$7.46   &     0.26   &        1   &  $<$0.80   &     0.13   &     0.29   \\ 
   Na I    &     4.40   &     0.26   &        1   &     0.19   &     0.10   &     0.28   \\ 
   Mg I    &     5.74   &     0.10   &        2   &     0.17   &     0.07   &     0.12   \\ 
   Al I    &  $<$5.70   &     0.26   &        1   &  $<$1.28   &     0.11   &     0.28   \\ 
   Si I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ca I    &     4.52   &     0.07   &       13   &     0.11   &     0.05   &     0.09   \\ 
   Sc II   &     1.26   &     0.26   &        1   &     0.14   &     0.12   &     0.29   \\ 
   Ti I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ti II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   V I     &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Cr I    &     3.45   &     0.13   &        3   &    $-$0.16   &     0.03   &     0.13   \\ 
   Mn I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Fe II   &     5.89   &     0.26   &        1   &     0.42   &     0.14   &     0.30   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.27   &     0.10   &        5   &     0.08   &     0.05   &     0.11   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &    $-$0.30   &     0.21   &        3   &    $-$0.45   &     0.09   &     0.23   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC06975 &          &            &            &            &            &            \\ 
   Fe I    &     5.66   &     0.03   &       53   &    $-$1.84\tablenotemark{a}   &     0.14   &     0.14   \\ 
   O I     &  $<$7.66   &     0.22   &        1   &  $<$0.81   &     0.11   &     0.25   \\ 
   Na I    &  $<$4.38   &     0.22   &        1   &   $<-$0.02   &     0.09   &     0.24   \\ 
   Mg I    &     6.03   &     0.02   &        2   &     0.27   &     0.05   &     0.05   \\ 
   Al I    &  $<$5.78   &     0.22   &        1   &  $<$1.17   &     0.09   &     0.24   \\ 
   Si I    &      ...   &      ...   &      ...   &      ...   &     0.11   &      ...   \\ 
   Ca I    &     4.73   &     0.05   &       14   &     0.14   &     0.04   &     0.06   \\ 
   Sc II   &     1.70   &     0.38   &        2   &     0.39   &     0.11   &     0.40   \\ 
   Ti I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ti II   &     3.29   &     0.14   &        2   &     0.17   &     0.11   &     0.18   \\ 
   V I     &      ...   &      ...   &      ...   &      ...   &     0.06   &      ...   \\ 
   Cr I    &     3.77   &     0.08   &        2   &    $-$0.03   &     0.04   &     0.09   \\ 
   Mn I    &     3.46   &     0.22   &        1   &    $-$0.13   &     0.08   &     0.23   \\ 
   Fe II   &     6.21   &     0.31   &        2   &     0.55   &     0.14   &     0.34   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.48   &     0.14   &        5   &     0.10   &     0.04   &     0.15   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.73   &     0.05   &        3   &     0.39   &     0.11   &     0.12   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Nd II   &    $-$0.01   &     0.22   &        1   &     0.41   &     0.09   &     0.24   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC07452 &          &            &            &            &            &            \\ 
   Fe I    &     6.21   &     0.02   &       82   &    $-$1.29\tablenotemark{a}   &     0.13   &     0.13   \\ 
   O I     &      ...   &      ...   &      ...   &      ...   &     0.15   &      ...   \\ 
   Na I    &     4.26   &     0.17   &        1   &    $-$0.69   &     0.09   &     0.19   \\ 
   Mg I    &     5.93   &     0.19   &        2   &    $-$0.38   &     0.05   &     0.20   \\ 
   Al I    &  $<$5.22   &     0.17   &        1   &  $<$0.06   &     0.10   &     0.20   \\ 
   Si I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ca I    &     4.82   &     0.04   &       19   &    $-$0.32   &     0.04   &     0.06   \\ 
   Sc II   &     0.96   &     0.17   &        1   &    $-$0.90   &     0.13   &     0.21   \\ 
   Ti I    &     3.34   &     0.12   &        5   &    $-$0.32   &     0.09   &     0.15   \\ 
   Ti II   &     3.51   &     0.12   &        4   &    $-$0.15   &     0.11   &     0.16   \\ 
   V I     &     1.94   &     0.19   &        5   &    $-$0.69   &     0.11   &     0.22   \\ 
   Cr I    &     4.22   &     0.04   &        4   &    $-$0.13   &     0.08   &     0.09   \\ 
   Mn I    &     3.81   &     0.06   &        5   &    $-$0.33   &     0.05   &     0.08   \\ 
   Fe II   &     6.44   &     0.04   &       12   &     0.24   &     0.17   &     0.17   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.50   &     0.06   &        7   &    $-$0.43   &     0.06   &     0.08   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.15   &     0.08   &        3   &    $-$0.74   &     0.08   &     0.11   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &     0.13   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC07889 &          &            &            &            &            &            \\ 
   Fe I    &     5.21   &     0.04   &       27   &    $-$2.29\tablenotemark{a}   &     0.12   &     0.13   \\ 
   O I     &  $<$7.63   &     0.22   &        1   &  $<$1.23   &     0.08   &     0.23   \\ 
   Na I    &  $<$4.72   &     0.22   &        1   &  $<$0.77   &     0.08   &     0.23   \\ 
   Mg I    &     6.13   &     0.22   &        1   &     0.82   &     0.06   &     0.23   \\ 
   Al I    &  $<$5.88   &     0.22   &        1   &  $<$1.72   &     0.08   &     0.23   \\ 
   Si I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ca I    &     4.30   &     0.08   &        8   &     0.16   &     0.05   &     0.09   \\ 
   Sc II   &     0.98   &     0.22   &        1   &     0.12   &     0.10   &     0.24   \\ 
   Ti I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ti II   &     2.99   &     0.22   &        1   &     0.33   &     0.10   &     0.24   \\ 
   V I     &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Cr I    &     2.92   &     0.16   &        2   &    $-$0.42   &     0.03   &     0.16   \\ 
   Mn I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Fe II   &     5.86   &     0.32   &        2   &     0.65   &     0.14   &     0.35   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.36   &     0.22   &        1   &     0.43   &     0.05   &     0.23   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &    $-$0.90   &     0.10   &        2   &    $-$0.79   &     0.07   &     0.12   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC08447 &          &            &            &            &            &            \\ 
   Fe I    &     6.02   &     0.02   &       72   &    $-$1.48\tablenotemark{a}   &     0.13   &     0.13   \\ 
   O I     &      ...   &      ...   &      ...   &      ...   &     0.15   &      ...   \\ 
   Na I    &     4.55   &     0.18   &        1   &    $-$0.21   &     0.08   &     0.20   \\ 
   Mg I    &     6.40   &     0.23   &        2   &     0.28   &     0.04   &     0.23   \\ 
   Al I    &      ...   &      ...   &      ...   &      ...   &     0.10   &      ...   \\ 
   Si I    &     6.13   &     0.18   &        1   &     0.10   &     0.13   &     0.22   \\ 
   Ca I    &     5.03   &     0.03   &       18   &     0.08   &     0.02   &     0.04   \\ 
   Sc II   &     1.68   &     0.09   &        6   &     0.01   &     0.13   &     0.16   \\ 
   Ti I    &     3.59   &     0.04   &        4   &     0.13   &     0.09   &     0.10   \\ 
   Ti II   &     4.01   &     0.06   &        3   &     0.55   &     0.12   &     0.13   \\ 
   V I     &     2.47   &     0.12   &        7   &     0.02   &     0.11   &     0.16   \\ 
   Cr I    &     4.09   &     0.06   &        4   &    $-$0.07   &     0.08   &     0.10   \\ 
   Mn I    &     3.65   &     0.12   &        4   &    $-$0.29   &     0.07   &     0.14   \\ 
   Fe II   &     6.33   &     0.06   &        9   &     0.32   &     0.18   &     0.19   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.47   &     0.07   &        6   &    $-$0.27   &     0.05   &     0.09   \\ 
   Cu I    &     2.23   &     0.18   &        1   &    $-$0.48   &     0.08   &     0.20   \\ 
   Ba II   &     0.81   &     0.09   &        3   &     0.11   &     0.11   &     0.14   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC08469 &          &            &            &            &            &            \\ 
   Fe I    &     6.16   &     0.03   &       68   &    $-$1.34\tablenotemark{a}   &     0.14   &     0.14   \\ 
   O I     &     7.65   &     0.22   &        1   &     0.30   &     0.14   &     0.26   \\ 
   Na I    &     4.46   &     0.22   &        1   &    $-$0.44   &     0.09   &     0.24   \\ 
   Mg I    &     6.24   &     0.06   &        2   &    $-$0.02   &     0.03   &     0.07   \\ 
   Al I    &  $<$5.42   &     0.22   &        1   &  $<$0.31   &     0.10   &     0.24   \\ 
   Si I    &     6.60   &     0.09   &        3   &     0.42   &     0.13   &     0.16   \\ 
   Ca I    &     5.10   &     0.04   &       19   &     0.01   &     0.02   &     0.04   \\ 
   Sc II   &     1.78   &     0.04   &        6   &    $-$0.03   &     0.12   &     0.13   \\ 
   Ti I    &     3.74   &     0.03   &        9   &     0.13   &     0.09   &     0.09   \\ 
   Ti II   &     3.60   &     0.23   &        2   &    $-$0.01   &     0.11   &     0.25   \\ 
   V I     &     2.46   &     0.09   &        4   &    $-$0.13   &     0.11   &     0.14   \\ 
   Cr I    &     4.05   &     0.15   &        4   &    $-$0.25   &     0.09   &     0.17   \\ 
   Mn I    &     3.67   &     0.10   &        4   &    $-$0.43   &     0.05   &     0.11   \\ 
   Fe II   &     6.38   &     0.06   &        9   &     0.22   &     0.18   &     0.19   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.78   &     0.04   &        8   &    $-$0.10   &     0.03   &     0.05   \\ 
   Cu I    &     2.29   &     0.22   &        1   &    $-$0.56   &     0.09   &     0.24   \\ 
   Ba II   &     1.00   &     0.05   &        3   &     0.15   &     0.10   &     0.11   \\ 
   La II   &     0.00   &     0.09   &        2   &     0.24   &     0.11   &     0.14   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC08615 &          &            &            &            &            &            \\ 
   Fe I    &     5.77   &     0.03   &       56   &    $-$1.73\tablenotemark{a}   &     0.11   &     0.11   \\ 
   O I     &     7.51   &     0.22   &        1   &     0.55   &     0.10   &     0.24   \\ 
   Na I    &     4.45   &     0.22   &        1   &    $-$0.06   &     0.07   &     0.23   \\ 
   Mg I    &     6.39   &     0.23   &        2   &     0.52   &     0.05   &     0.24   \\ 
   Al I    &  $<$5.64   &     0.22   &        1   &  $<$0.92   &     0.07   &     0.23   \\ 
   Si I    &     6.34   &     0.22   &        1   &     0.56   &     0.10   &     0.24   \\ 
   Ca I    &     4.88   &     0.04   &       18   &     0.18   &     0.03   &     0.05   \\ 
   Sc II   &     1.47   &     0.22   &        2   &     0.05   &     0.09   &     0.24   \\ 
   Ti I    &     3.67   &     0.24   &        2   &     0.45   &     0.05   &     0.25   \\ 
   Ti II   &     3.27   &     0.23   &        3   &     0.05   &     0.10   &     0.25   \\ 
   V I     &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Cr I    &     3.72   &     0.02   &        3   &    $-$0.19   &     0.04   &     0.04   \\ 
   Mn I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Fe II   &     6.15   &     0.10   &        5   &     0.38   &     0.13   &     0.16   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.63   &     0.14   &        6   &     0.14   &     0.04   &     0.15   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.71   &     0.31   &        3   &     0.26   &     0.11   &     0.33   \\ 
   La II   &     0.01   &     0.22   &        1   &     0.64   &     0.09   &     0.24   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC08695 &          &            &            &            &            &            \\ 
   Fe I    &     6.21   &     0.02   &       71   &    $-$1.29\tablenotemark{a}   &     0.14   &     0.14   \\ 
   O I     &     7.61   &     0.18   &        1   &     0.21   &     0.15   &     0.23   \\ 
   Na I    &     4.81   &     0.18   &        1   &    $-$0.14   &     0.08   &     0.20   \\ 
   Mg I    &     6.43   &     0.13   &        2   &     0.12   &     0.04   &     0.14   \\ 
   Al I    &      ...   &      ...   &      ...   &      ...   &     0.11   &      ...   \\ 
   Si I    &     6.36   &     0.18   &        1   &     0.14   &     0.13   &     0.22   \\ 
   Ca I    &     5.19   &     0.06   &       18   &     0.05   &     0.02   &     0.06   \\ 
   Sc II   &     1.78   &     0.09   &        5   &    $-$0.08   &     0.11   &     0.14   \\ 
   Ti I    &     3.74   &     0.05   &        8   &     0.08   &     0.10   &     0.11   \\ 
   Ti II   &     3.99   &     0.19   &        3   &     0.32   &     0.09   &     0.21   \\ 
   V I     &     2.46   &     0.11   &        8   &    $-$0.19   &     0.11   &     0.16   \\ 
   Cr I    &     3.98   &     0.10   &        4   &    $-$0.37   &     0.09   &     0.13   \\ 
   Mn I    &     3.55   &     0.05   &        6   &    $-$0.59   &     0.07   &     0.09   \\ 
   Fe II   &     6.43   &     0.05   &        9   &     0.21   &     0.17   &     0.18   \\ 
   Co I    &     3.43   &     0.18   &        1   &    $-$0.27   &     0.10   &     0.21   \\ 
   Ni I    &     4.69   &     0.08   &        8   &    $-$0.24   &     0.05   &     0.09   \\ 
   Cu I    &     2.12   &     0.18   &        1   &    $-$0.78   &     0.10   &     0.21   \\ 
   Ba II   &     1.11   &     0.03   &        3   &     0.22   &     0.09   &     0.09   \\ 
   La II   &     0.06   &     0.18   &        1   &     0.25   &     0.12   &     0.22   \\ 
   Nd II   &     0.23   &     0.18   &        1   &     0.10   &     0.09   &     0.20   \\ 
   Eu II   &    $-$0.22   &     0.18   &        1   &     0.55   &     0.13   &     0.22   \\ 
 &          &            &            &            &            &            \\ 
    CC08788 &          &            &            &            &            &            \\ 
   Fe I    &     6.02   &     0.03   &       52   &    $-$1.48\tablenotemark{a}   &     0.13   &     0.13   \\ 
   O I     &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Na I    &     4.63   &     0.22   &        1   &    $-$0.13   &     0.09   &     0.24   \\ 
   Mg I    &     6.38   &     0.13   &        2   &     0.26   &     0.06   &     0.14   \\ 
   Al I    &  $<$5.66   &     0.22   &        1   &  $<$0.69   &     0.08   &     0.23   \\ 
   Si I    &     6.09   &     0.22   &        1   &     0.06   &     0.10   &     0.24   \\ 
   Ca I    &     5.08   &     0.06   &       15   &     0.14   &     0.03   &     0.07   \\ 
   Sc II   &     2.02   &     0.18   &        4   &     0.36   &     0.11   &     0.21   \\ 
   Ti I    &     3.85   &     0.33   &        2   &     0.38   &     0.06   &     0.34   \\ 
   Ti II   &     3.51   &     0.00   &        2   &     0.05   &     0.10   &     0.10   \\ 
   V I     &     2.83   &     0.28   &        3   &     0.39   &     0.07   &     0.29   \\ 
   Cr I    &     3.96   &     0.06   &        3   &    $-$0.19   &     0.04   &     0.07   \\ 
   Mn I    &     3.95   &     0.10   &        2   &     0.01   &     0.05   &     0.11   \\ 
   Fe II   &     6.35   &     0.07   &        7   &     0.33   &     0.15   &     0.17   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.74   &     0.12   &        8   &     0.01   &     0.04   &     0.13   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.74   &     0.08   &        2   &     0.04   &     0.10   &     0.13   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &    $-$0.16   &     0.22   &        1   &     0.80   &     0.12   &     0.25   \\ 
 &          &            &            &            &            &            \\ 
    CC09000 &          &            &            &            &            &            \\ 
   Fe I    &     5.68   &     0.02   &       68   &    $-$1.82\tablenotemark{a}   &     0.13   &     0.13   \\ 
   O I     &      ...   &      ...   &      ...   &      ...   &     0.13   &      ...   \\ 
   Na I    &  $<$3.94   &     0.16   &        1   &   $<-$0.48   &     0.08   &     0.18   \\ 
   Mg I    &     5.55   &     0.16   &        2   &    $-$0.23   &     0.04   &     0.16   \\ 
   Al I    &  $<$5.23   &     0.16   &        1   &  $<$0.60   &     0.08   &     0.18   \\ 
   Si I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ca I    &     4.39   &     0.03   &       16   &    $-$0.22   &     0.03   &     0.04   \\ 
   Sc II   &     1.09   &     0.12   &        3   &    $-$0.25   &     0.11   &     0.16   \\ 
   Ti I    &     3.05   &     0.03   &        3   &    $-$0.08   &     0.08   &     0.09   \\ 
   Ti II   &     3.60   &     0.19   &        2   &     0.46   &     0.10   &     0.21   \\ 
   V I     &     1.93   &     0.31   &        2   &    $-$0.18   &     0.10   &     0.33   \\ 
   Cr I    &     3.64   &     0.05   &        4   &    $-$0.19   &     0.08   &     0.09   \\ 
   Mn I    &     3.18   &     0.03   &        3   &    $-$0.44   &     0.05   &     0.06   \\ 
   Fe II   &     6.10   &     0.05   &        9   &     0.42   &     0.14   &     0.15   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.16   &     0.04   &        9   &    $-$0.25   &     0.04   &     0.06   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.64   &     0.02   &        3   &     0.28   &     0.10   &     0.10   \\ 
   La II   &    $-$0.24   &     0.16   &        1   &     0.48   &     0.10   &     0.19   \\ 
   Nd II   &     0.13   &     0.16   &        1   &     0.53   &     0.07   &     0.17   \\ 
   Eu II   &    $-$0.46   &     0.16   &        1   &     0.84   &     0.12   &     0.20   \\ 
 &          &            &            &            &            &            \\ 
    CC09179 &          &            &            &            &            &            \\ 
   Fe I    &     5.72   &     0.03   &       59   &    $-$1.78\tablenotemark{a}   &     0.15   &     0.15   \\ 
   O I     &  $<$7.48   &     0.21   &        1   &  $<$0.57   &     0.13   &     0.25   \\ 
   Na I    &  $<$4.20   &     0.21   &        1   &   $<-$0.26   &     0.09   &     0.23   \\ 
   Mg I    &     5.86   &     0.38   &        2   &     0.03   &     0.05   &     0.38   \\ 
   Al I    &  $<$5.48   &     0.21   &        1   &  $<$0.81   &     0.10   &     0.23   \\ 
   Si I    &     6.57   &     0.21   &        1   &     0.84   &     0.11   &     0.24   \\ 
   Ca I    &     4.51   &     0.07   &       14   &    $-$0.14   &     0.04   &     0.08   \\ 
   Sc II   &     1.15   &     0.12   &        2   &    $-$0.22   &     0.12   &     0.17   \\ 
   Ti I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ti II   &     3.10   &     0.05   &        2   &    $-$0.08   &     0.11   &     0.12   \\ 
   V I     &     2.44   &     0.21   &        1   &     0.29   &     0.08   &     0.22   \\ 
   Cr I    &     3.73   &     0.11   &        3   &    $-$0.13   &     0.05   &     0.12   \\ 
   Mn I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Fe II   &     6.03   &     0.07   &        7   &     0.31   &     0.14   &     0.16   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.16   &     0.07   &        3   &    $-$0.28   &     0.07   &     0.10   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.81   &     0.09   &        3   &     0.41   &     0.13   &     0.16   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &    $-$0.31   &     0.21   &        1   &     0.95   &     0.13   &     0.25   \\ 
 &          &            &            &            &            &            \\ 
    CC09225 &          &            &            &            &            &            \\ 
   Fe I    &     5.93   &     0.02   &       69   &    $-$1.57\tablenotemark{a}   &     0.13   &     0.13   \\ 
   O I     &     7.60   &     0.17   &        1   &     0.48   &     0.13   &     0.21   \\ 
   Na I    &     4.33   &     0.17   &        1   &    $-$0.34   &     0.09   &     0.19   \\ 
   Mg I    &     6.39   &     0.05   &        2   &     0.36   &     0.05   &     0.07   \\ 
   Al I    &  $<$5.39   &     0.17   &        1   &  $<$0.51   &     0.09   &     0.19   \\ 
   Si I    &     6.02   &     0.17   &        1   &     0.08   &     0.12   &     0.21   \\ 
   Ca I    &     4.95   &     0.06   &       20   &     0.08   &     0.03   &     0.07   \\ 
   Sc II   &     1.64   &     0.06   &        6   &     0.05   &     0.12   &     0.13   \\ 
   Ti I    &     3.61   &     0.12   &        2   &     0.23   &     0.08   &     0.14   \\ 
   Ti II   &     3.89   &     0.14   &        3   &     0.51   &     0.12   &     0.18   \\ 
   V I     &     2.32   &     0.17   &        6   &    $-$0.05   &     0.10   &     0.20   \\ 
   Cr I    &     3.81   &     0.08   &        4   &    $-$0.26   &     0.06   &     0.10   \\ 
   Mn I    &     3.54   &     0.07   &        3   &    $-$0.32   &     0.06   &     0.09   \\ 
   Fe II   &     6.09   &     0.03   &        8   &     0.16   &     0.17   &     0.17   \\ 
   Co I    &     3.50   &     0.17   &        1   &     0.08   &     0.08   &     0.19   \\ 
   Ni I    &     4.65   &     0.06   &        8   &     0.00   &     0.04   &     0.07   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.92   &     0.04   &        3   &     0.30   &     0.12   &     0.13   \\ 
   La II   &     0.26   &     0.17   &        1   &     0.73   &     0.11   &     0.20   \\ 
   Nd II   &     0.06   &     0.17   &        1   &     0.21   &     0.10   &     0.20   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &     0.14   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC09226 &          &            &            &            &            &            \\ 
   Fe I    &     5.94   &     0.03   &       65   &    $-$1.56\tablenotemark{a}   &     0.13   &     0.13   \\ 
   O I     &     7.58   &     0.24   &        1   &     0.45   &     0.13   &     0.27   \\ 
   Na I    &     4.46   &     0.24   &        1   &    $-$0.22   &     0.09   &     0.26   \\ 
   Mg I    &     6.22   &     0.14   &        2   &     0.18   &     0.05   &     0.15   \\ 
   Al I    &  $<$5.51   &     0.24   &        1   &  $<$0.62   &     0.09   &     0.26   \\ 
   Si I    &     6.28   &     0.27   &        2   &     0.34   &     0.11   &     0.29   \\ 
   Ca I    &     4.97   &     0.05   &       15   &     0.11   &     0.03   &     0.06   \\ 
   Sc II   &     1.69   &     0.10   &        4   &     0.10   &     0.12   &     0.16   \\ 
   Ti I    &      ...   &      ...   &      ...   &      ...   &     0.08   &      ...   \\ 
   Ti II   &     3.63   &     0.14   &        3   &     0.24   &     0.11   &     0.18   \\ 
   V I     &     2.94   &     0.17   &        2   &     0.58   &     0.08   &     0.19   \\ 
   Cr I    &     4.01   &     0.12   &        4   &    $-$0.06   &     0.04   &     0.13   \\ 
   Mn I    &     3.70   &     0.24   &        1   &    $-$0.17   &     0.05   &     0.25   \\ 
   Fe II   &     6.09   &     0.09   &        6   &     0.15   &     0.15   &     0.17   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.57   &     0.04   &        7   &    $-$0.09   &     0.06   &     0.07   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     1.07   &     0.16   &        3   &     0.45   &     0.13   &     0.21   \\ 
   La II   &     0.69   &     0.24   &        1   &     1.15   &     0.11   &     0.26   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC09430 &          &            &            &            &            &            \\ 
   Fe I    &     5.37   &     0.03   &       46   &    $-$2.13\tablenotemark{a}   &     0.15   &     0.15   \\ 
   O I     &  $<$7.35   &     0.18   &        1   &  $<$0.79   &     0.12   &     0.22   \\ 
   Na I    &  $<$4.18   &     0.18   &        1   &  $<$0.07   &     0.10   &     0.21   \\ 
   Mg I    &     6.23   &     0.21   &        2   &     0.75   &     0.06   &     0.22   \\ 
   Al I    &  $<$5.58   &     0.18   &        1   &  $<$1.26   &     0.10   &     0.21   \\ 
   Si I    &      ...   &      ...   &      ...   &      ...   &     0.12   &      ...   \\ 
   Ca I    &     4.44   &     0.08   &       13   &     0.14   &     0.05   &     0.09   \\ 
   Sc II   &     1.41   &     0.04   &        4   &     0.38   &     0.11   &     0.12   \\ 
   Ti I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ti II   &     3.19   &     0.19   &        3   &     0.37   &     0.10   &     0.21   \\ 
   V I     &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Cr I    &     3.23   &     0.07   &        3   &    $-$0.28   &     0.01   &     0.07   \\ 
   Mn I    &     3.74   &     0.05   &        2   &     0.44   &     0.07   &     0.09   \\ 
   Fe II   &     5.75   &     0.19   &        3   &     0.37   &     0.14   &     0.24   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.06   &     0.04   &        4   &    $-$0.03   &     0.06   &     0.07   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &    $-$0.08   &     0.05   &        2   &    $-$0.13   &     0.11   &     0.12   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC09507 &          &            &            &            &            &            \\ 
   Fe I    &     5.78   &     0.03   &       58   &    $-$1.72\tablenotemark{a}   &     0.12   &     0.12   \\ 
   O I     &  $<$7.55   &     0.22   &        1   &  $<$0.58   &     0.11   &     0.25   \\ 
   Na I    &  $<$4.25   &     0.22   &        1   &   $<-$0.27   &     0.08   &     0.23   \\ 
   Mg I    &     5.76   &     0.03   &        2   &    $-$0.12   &     0.06   &     0.07   \\ 
   Al I    &  $<$5.65   &     0.22   &        1   &  $<$0.92   &     0.09   &     0.24   \\ 
   Si I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ca I    &     4.60   &     0.04   &       15   &    $-$0.11   &     0.04   &     0.06   \\ 
   Sc II   &     1.35   &     0.16   &        5   &    $-$0.08   &     0.11   &     0.19   \\ 
   Ti I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ti II   &     3.09   &     0.22   &        1   &    $-$0.14   &     0.10   &     0.24   \\ 
   V I     &     2.72   &     0.22   &        1   &     0.51   &     0.07   &     0.23   \\ 
   Cr I    &     4.09   &     0.11   &        3   &     0.17   &     0.07   &     0.13   \\ 
   Mn I    &     3.95   &     0.22   &        1   &     0.24   &     0.06   &     0.23   \\ 
   Fe II   &     5.98   &     0.08   &        4   &     0.20   &     0.14   &     0.16   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.23   &     0.08   &        6   &    $-$0.27   &     0.06   &     0.10   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.97   &     0.06   &        2   &     0.51   &     0.12   &     0.13   \\ 
   La II   &     0.10   &     0.22   &        1   &     0.72   &     0.10   &     0.24   \\ 
   Nd II   &     0.01   &     0.22   &        1   &     0.31   &     0.09   &     0.24   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC09633 &          &            &            &            &            &            \\ 
   Fe I    &     5.00   &     0.04   &       34   &    $-$2.50\tablenotemark{a}   &     0.14   &     0.15   \\ 
   O I     &  $<$7.33   &     0.23   &        1   &  $<$1.14   &     0.10   &     0.25   \\ 
   Na I    &  $<$4.27   &     0.23   &        1   &  $<$0.53   &     0.07   &     0.24   \\ 
   Mg I    &     5.25   &     0.23   &        1   &     0.15   &     0.06   &     0.24   \\ 
   Al I    &  $<$5.67   &     0.23   &        1   &  $<$1.72   &     0.09   &     0.25   \\ 
   Si I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ca I    &     4.04   &     0.07   &       10   &     0.11   &     0.06   &     0.09   \\ 
   Sc II   &     1.10   &     0.13   &        2   &     0.45   &     0.10   &     0.16   \\ 
   Ti I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ti II   &     2.55   &     0.12   &        2   &     0.09   &     0.11   &     0.16   \\ 
   V I     &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Cr I    &     2.88   &     0.03   &        3   &    $-$0.26   &     0.02   &     0.04   \\ 
   Mn I    &     3.14   &     0.23   &        1   &     0.21   &     0.07   &     0.24   \\ 
   Fe II   &     5.48   &     0.06   &        2   &     0.48   &     0.13   &     0.14   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     3.64   &     0.23   &        1   &    $-$0.08   &     0.04   &     0.23   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &    $-$1.32   &     0.23   &        1   &    $-$1.00   &     0.08   &     0.24   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &     0.10   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC09869 &          &            &            &            &            &            \\ 
   Fe I    &     6.24   &     0.03   &       66   &    $-$1.26\tablenotemark{a}   &     0.15   &     0.15   \\ 
   O I     &      ...   &      ...   &      ...   &      ...   &     0.15   &      ...   \\ 
   Na I    &     4.79   &     0.20   &        1   &    $-$0.19   &     0.09   &     0.22   \\ 
   Mg I    &     6.53   &     0.00   &        2   &     0.19   &     0.04   &     0.04   \\ 
   Al I    &  $<$5.49   &     0.20   &        1   &  $<$0.30   &     0.11   &     0.23   \\ 
   Si I    &     6.38   &     0.06   &        2   &     0.13   &     0.13   &     0.14   \\ 
   Ca I    &     5.23   &     0.06   &       18   &     0.06   &     0.02   &     0.06   \\ 
   Sc II   &     2.03   &     0.08   &        5   &     0.14   &     0.11   &     0.14   \\ 
   Ti I    &     3.75   &     0.06   &        3   &     0.05   &     0.08   &     0.10   \\ 
   Ti II   &     3.98   &     0.21   &        4   &     0.29   &     0.09   &     0.23   \\ 
   V I     &     2.39   &     0.12   &        5   &    $-$0.28   &     0.10   &     0.16   \\ 
   Cr I    &     4.42   &     0.11   &        4   &     0.04   &     0.06   &     0.13   \\ 
   Mn I    &     3.83   &     0.06   &        4   &    $-$0.34   &     0.04   &     0.07   \\ 
   Fe II   &     6.34   &     0.10   &        6   &     0.09   &     0.15   &     0.18   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.84   &     0.06   &        9   &    $-$0.12   &     0.05   &     0.08   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     1.06   &     0.14   &        3   &     0.13   &     0.10   &     0.17   \\ 
   La II   &     0.25   &     0.05   &        2   &     0.41   &     0.12   &     0.13   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &     0.14   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC09929 &          &            &            &            &            &            \\ 
   Fe I    &     6.00   &     0.03   &       40   &    $-$1.50\tablenotemark{a}   &     0.15   &     0.15   \\ 
   O I     &     7.95   &     0.22   &        1   &     0.76   &     0.13   &     0.26   \\ 
   Na I    &     4.35   &     0.22   &        1   &    $-$0.39   &     0.10   &     0.24   \\ 
   Mg I    &     6.26   &     0.06   &        2   &     0.16   &     0.05   &     0.08   \\ 
   Al I    &  $<$5.64   &     0.22   &        1   &  $<$0.69   &     0.10   &     0.24   \\ 
   Si I    &     6.22   &     0.22   &        1   &     0.21   &     0.13   &     0.26   \\ 
   Ca I    &     5.17   &     0.07   &       16   &     0.24   &     0.03   &     0.08   \\ 
   Sc II   &     1.86   &     0.18   &        4   &     0.20   &     0.12   &     0.22   \\ 
   Ti I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ti II   &     3.66   &     0.13   &        3   &     0.21   &     0.11   &     0.17   \\ 
   V I     &     2.60   &     0.07   &        2   &     0.16   &     0.08   &     0.11   \\ 
   Cr I    &     4.14   &     0.09   &        4   &     0.00   &     0.05   &     0.10   \\ 
   Mn I    &     3.61   &     0.14   &        4   &    $-$0.32   &     0.07   &     0.16   \\ 
   Fe II   &     6.29   &     0.11   &        3   &     0.29   &     0.15   &     0.19   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.75   &     0.09   &        7   &     0.03   &     0.04   &     0.10   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &     0.08   &      ...   \\ 
   Ba II   &     1.09   &     0.09   &        2   &     0.40   &     0.11   &     0.14   \\ 
   La II   &     0.33   &     0.01   &        3   &     0.73   &     0.12   &     0.12   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &    $-$0.13   &     0.22   &        1   &     0.85   &     0.14   &     0.26   \\ 
 &          &            &            &            &            &            \\ 
    CC10038 &          &            &            &            &            &            \\ 
   Fe I    &     6.20   &     0.02   &       63   &    $-$1.30\tablenotemark{a}   &     0.15   &     0.15   \\ 
   O I     &     7.93   &     0.19   &        1   &     0.54   &     0.13   &     0.23   \\ 
   Na I    &     4.65   &     0.19   &        1   &    $-$0.29   &     0.09   &     0.21   \\ 
   Mg I    &     6.53   &     0.25   &        2   &     0.24   &     0.05   &     0.25   \\ 
   Al I    &  $<$5.61   &     0.19   &        1   &  $<$0.46   &     0.10   &     0.21   \\ 
   Si I    &     6.54   &     0.13   &        3   &     0.33   &     0.13   &     0.18   \\ 
   Ca I    &     5.10   &     0.07   &       17   &    $-$0.02   &     0.03   &     0.08   \\ 
   Sc II   &     1.88   &     0.03   &        6   &     0.03   &     0.10   &     0.10   \\ 
   Ti I    &     3.62   &     0.18   &        3   &    $-$0.03   &     0.09   &     0.20   \\ 
   Ti II   &     3.99   &     0.15   &        3   &     0.35   &     0.08   &     0.17   \\ 
   V I     &     2.47   &     0.08   &        2   &    $-$0.15   &     0.09   &     0.12   \\ 
   Cr I    &     4.32   &     0.07   &        4   &    $-$0.02   &     0.06   &     0.09   \\ 
   Mn I    &     3.70   &     0.12   &        5   &    $-$0.42   &     0.06   &     0.13   \\ 
   Fe II   &     6.26   &     0.08   &        9   &     0.06   &     0.14   &     0.16   \\ 
   Co I    &     3.65   &     0.19   &        1   &    $-$0.04   &     0.10   &     0.21   \\ 
   Ni I    &     4.72   &     0.06   &        8   &    $-$0.20   &     0.06   &     0.08   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &     0.11   &      ...   \\ 
   Ba II   &     0.98   &     0.14   &        3   &     0.10   &     0.10   &     0.17   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &     0.12   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC10194 &          &            &            &            &            &            \\ 
   Fe I    &     6.08   &     0.03   &       53   &    $-$1.42\tablenotemark{a}   &     0.15   &     0.15   \\ 
   O I     &     7.44   &     0.22   &        1   &     0.17   &     0.15   &     0.27   \\ 
   Na I    &     4.51   &     0.22   &        1   &    $-$0.31   &     0.10   &     0.24   \\ 
   Mg I    &     6.33   &     0.13   &        2   &     0.15   &     0.06   &     0.14   \\ 
   Al I    &  $<$5.45   &     0.22   &        1   &  $<$0.42   &     0.12   &     0.25   \\ 
   Si I    &     6.27   &     0.22   &        1   &     0.18   &     0.15   &     0.27   \\ 
   Ca I    &     5.03   &     0.07   &       16   &     0.01   &     0.03   &     0.08   \\ 
   Sc II   &     1.46   &     0.08   &        4   &    $-$0.27   &     0.13   &     0.15   \\ 
   Ti I    &     3.74   &     0.16   &        5   &     0.21   &     0.10   &     0.19   \\ 
   Ti II   &     3.76   &     0.11   &        2   &     0.23   &     0.11   &     0.16   \\ 
   V I     &     2.27   &     0.16   &        5   &    $-$0.25   &     0.11   &     0.19   \\ 
   Cr I    &     4.23   &     0.22   &        4   &     0.00   &     0.08   &     0.23   \\ 
   Mn I    &     3.11   &     0.15   &        3   &    $-$0.90   &     0.09   &     0.17   \\ 
   Fe II   &     6.08   &     0.10   &        5   &    $-$0.01   &     0.18   &     0.21   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &     0.10   &      ...   \\ 
   Ni I    &     4.56   &     0.10   &        7   &    $-$0.25   &     0.06   &     0.12   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.89   &     0.19   &        3   &     0.13   &     0.11   &     0.22   \\ 
   La II   &    $-$0.08   &     0.22   &        1   &     0.24   &     0.13   &     0.26   \\ 
   Nd II   &    $-$0.31   &     0.22   &        1   &    $-$0.31   &     0.12   &     0.25   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC10318 &          &            &            &            &            &            \\ 
   Fe I    &     5.91   &     0.02   &       59   &    $-$1.59\tablenotemark{a}   &     0.14   &     0.14   \\ 
   O I     &     7.75   &     0.19   &        1   &     0.65   &     0.13   &     0.23   \\ 
   Na I    &  $<$4.23   &     0.19   &        1   &   $<-$0.42   &     0.09   &     0.21   \\ 
   Mg I    &     6.11   &     0.20   &        2   &     0.10   &     0.05   &     0.21   \\ 
   Al I    &  $<$5.44   &     0.19   &        1   &  $<$0.58   &     0.10   &     0.21   \\ 
   Si I    &     6.23   &     0.10   &        2   &     0.31   &     0.13   &     0.16   \\ 
   Ca I    &     4.86   &     0.05   &       15   &     0.02   &     0.03   &     0.06   \\ 
   Sc II   &     2.04   &     0.08   &        5   &     0.48   &     0.11   &     0.14   \\ 
   Ti I    &     3.55   &     0.07   &        4   &     0.19   &     0.09   &     0.11   \\ 
   Ti II   &     3.93   &     0.24   &        2   &     0.57   &     0.11   &     0.26   \\ 
   V I     &     2.03   &     0.19   &        3   &    $-$0.31   &     0.10   &     0.21   \\ 
   Cr I    &     3.87   &     0.07   &        4   &    $-$0.18   &     0.08   &     0.11   \\ 
   Mn I    &     3.47   &     0.06   &        4   &    $-$0.36   &     0.07   &     0.09   \\ 
   Fe II   &     6.18   &     0.07   &        7   &     0.27   &     0.18   &     0.19   \\ 
   Co I    &     3.55   &     0.19   &        1   &     0.15   &     0.08   &     0.21   \\ 
   Ni I    &     4.62   &     0.07   &        8   &    $-$0.01   &     0.04   &     0.08   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.87   &     0.33   &        3   &     0.28   &     0.11   &     0.35   \\ 
   La II   &     0.00   &     0.19   &        1   &     0.49   &     0.12   &     0.22   \\ 
   Nd II   &     0.16   &     0.19   &        1   &     0.33   &     0.09   &     0.21   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC10414 &          &            &            &            &            &            \\ 
   Fe I    &     6.15   &     0.03   &       57   &    $-$1.35\tablenotemark{a}   &     0.14   &     0.14   \\ 
   O I     &     7.91   &     0.22   &        1   &     0.57   &     0.13   &     0.26   \\ 
   Na I    &     4.13   &     0.22   &        1   &    $-$0.76   &     0.10   &     0.24   \\ 
   Mg I    &     6.35   &     0.25   &        2   &     0.10   &     0.05   &     0.25   \\ 
   Al I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Si I    &     6.45   &     0.06   &        2   &     0.29   &     0.13   &     0.14   \\ 
   Ca I    &     5.20   &     0.07   &       18   &     0.12   &     0.02   &     0.07   \\ 
   Sc II   &     1.80   &     0.14   &        4   &     0.00   &     0.11   &     0.18   \\ 
   Ti I    &     3.67   &     0.03   &        3   &     0.08   &     0.08   &     0.09   \\ 
   Ti II   &     3.64   &     0.07   &        3   &     0.04   &     0.10   &     0.12   \\ 
   V I     &     2.53   &     0.33   &        3   &    $-$0.04   &     0.09   &     0.34   \\ 
   Cr I    &     4.07   &     0.17   &        4   &    $-$0.22   &     0.06   &     0.18   \\ 
   Mn I    &     3.76   &     0.14   &        5   &    $-$0.32   &     0.06   &     0.15   \\ 
   Fe II   &     6.26   &     0.06   &        8   &     0.11   &     0.16   &     0.17   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.73   &     0.07   &        8   &    $-$0.13   &     0.05   &     0.09   \\ 
   Cu I    &     2.52   &     0.22   &        1   &    $-$0.32   &     0.08   &     0.23   \\ 
   Ba II   &     0.56   &     0.19   &        3   &    $-$0.26   &     0.08   &     0.21   \\ 
   La II   &     0.09   &     0.22   &        1   &     0.34   &     0.11   &     0.25   \\ 
   Nd II   &     0.43   &     0.22   &        1   &     0.36   &     0.09   &     0.24   \\ 
   Eu II   &    $-$0.21   &     0.22   &        1   &     0.62   &     0.12   &     0.25   \\ 
 &          &            &            &            &            &            \\ 
    CC10686 &          &            &            &            &            &            \\ 
   Fe I    &     5.82   &     0.02   &       75   &    $-$1.68\tablenotemark{a}   &     0.13   &     0.13   \\ 
   O I     &     7.57   &     0.17   &        1   &     0.56   &     0.13   &     0.21   \\ 
   Na I    &     4.35   &     0.17   &        1   &    $-$0.21   &     0.08   &     0.19   \\ 
   Mg I    &     6.22   &     0.19   &        2   &     0.30   &     0.04   &     0.19   \\ 
   Al I    &  $<$5.29   &     0.17   &        1   &  $<$0.52   &     0.09   &     0.19   \\ 
   Si I    &     6.07   &     0.17   &        1   &     0.24   &     0.13   &     0.21   \\ 
   Ca I    &     4.82   &     0.02   &       17   &     0.07   &     0.02   &     0.03   \\ 
   Sc II   &     1.60   &     0.09   &        6   &     0.13   &     0.11   &     0.14   \\ 
   Ti I    &     3.37   &     0.05   &        6   &     0.10   &     0.08   &     0.09   \\ 
   Ti II   &     3.58   &     0.12   &        3   &     0.32   &     0.11   &     0.16   \\ 
   V I     &     1.95   &     0.11   &        4   &    $-$0.29   &     0.10   &     0.15   \\ 
   Cr I    &     3.76   &     0.02   &        4   &    $-$0.19   &     0.08   &     0.08   \\ 
   Mn I    &     3.19   &     0.09   &        3   &    $-$0.56   &     0.06   &     0.11   \\ 
   Fe II   &     5.98   &     0.04   &        8   &     0.17   &     0.16   &     0.16   \\ 
   Co I    &     3.38   &     0.17   &        1   &     0.07   &     0.08   &     0.19   \\ 
   Ni I    &     4.47   &     0.04   &        8   &    $-$0.06   &     0.04   &     0.06   \\ 
   Cu I    &     1.87   &     0.17   &        1   &    $-$0.64   &     0.09   &     0.19   \\ 
   Ba II   &     0.77   &     0.06   &        3   &     0.27   &     0.10   &     0.12   \\ 
   La II   &    $-$0.20   &     0.10   &        2   &     0.38   &     0.11   &     0.15   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &    $-$0.72   &     0.17   &        1   &     0.44   &     0.13   &     0.21   \\ 
 &          &            &            &            &            &            \\ 
    CC10690 &          &            &            &            &            &            \\ 
   Fe I    &     5.54   &     0.02   &       55   &    $-$1.96\tablenotemark{a}   &     0.14   &     0.14   \\ 
   O I     &  $<$7.37   &     0.18   &        1   &  $<$0.64   &     0.11   &     0.21   \\ 
   Na I    &  $<$4.15   &     0.18   &        1   &   <$-$0.13   &     0.09   &     0.20   \\ 
   Mg I    &     5.22   &     0.18   &        1   &    $-$0.42   &     0.06   &     0.19   \\ 
   Al I    &  $<$5.54   &     0.18   &        1   &  $<$1.05   &     0.08   &     0.20   \\ 
   Si I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ca I    &     4.22   &     0.05   &       14   &    $-$0.24   &     0.05   &     0.07   \\ 
   Sc II   &     0.92   &     0.18   &        1   &    $-$0.27   &     0.10   &     0.21   \\ 
   Ti I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ti II   &     3.28   &     0.28   &        3   &     0.30   &     0.10   &     0.30   \\ 
   V I     &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Cr I    &     3.29   &     0.12   &        3   &    $-$0.39   &     0.03   &     0.12   \\ 
   Mn I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Fe II   &     5.87   &     0.06   &        6   &     0.34   &     0.14   &     0.15   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     3.89   &     0.12   &        3   &    $-$0.37   &     0.05   &     0.13   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.00   &     0.06   &        3   &    $-$0.22   &     0.09   &     0.11   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC10802 &          &            &            &            &            &            \\ 
   Fe I    &     6.23   &     0.03   &       48   &    $-$1.27\tablenotemark{a}   &     0.14   &     0.14   \\ 
   O I     &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Na I    &     4.47   &     0.22   &        1   &    $-$0.50   &     0.10   &     0.24   \\ 
   Mg I    &     6.28   &     0.43   &        2   &    $-$0.05   &     0.06   &     0.43   \\ 
   Al I    &  $<$5.78   &     0.22   &        1   &  $<$0.60   &     0.10   &     0.24   \\ 
   Si I    &     6.69   &     0.22   &        1   &     0.45   &     0.12   &     0.25   \\ 
   Ca I    &     5.29   &     0.13   &       12   &     0.13   &     0.03   &     0.13   \\ 
   Sc II   &     1.79   &     0.06   &        3   &    $-$0.09   &     0.12   &     0.13   \\ 
   Ti I    &     4.31   &     0.35   &        3   &     0.63   &     0.07   &     0.36   \\ 
   Ti II   &     3.99   &     0.22   &        1   &     0.31   &     0.11   &     0.25   \\ 
   V I     &     2.51   &     0.04   &        2   &    $-$0.16   &     0.10   &     0.11   \\ 
   Cr I    &     4.46   &     0.19   &        3   &     0.09   &     0.07   &     0.20   \\ 
   Mn I    &     3.86   &     0.22   &        1   &    $-$0.30   &     0.04   &     0.22   \\ 
   Fe II   &     6.65   &     0.13   &        4   &     0.42   &     0.15   &     0.20   \\ 
   Co I    &     4.14   &     0.22   &        1   &     0.42   &     0.08   &     0.23   \\ 
   Ni I    &     4.84   &     0.16   &        5   &    $-$0.11   &     0.05   &     0.17   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     1.10   &     0.23   &        3   &     0.19   &     0.10   &     0.25   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC10944 &          &            &            &            &            &            \\ 
   Fe I    &     5.61   &     0.03   &       62   &    $-$1.89\tablenotemark{a}   &     0.12   &     0.12   \\ 
   O I     &      ...   &      ...   &      ...   &      ...   &     0.12   &      ...   \\ 
   Na I    &      ...   &      ...   &      ...   &      ...   &     0.07   &      ...   \\ 
   Mg I    &     5.97   &     0.12   &        2   &     0.26   &     0.05   &     0.13   \\ 
   Al I    &  $<$5.62   &     0.21   &        1   &  $<$1.06   &     0.08   &     0.22   \\ 
   Si I    &     6.06   &     0.21   &        1   &     0.44   &     0.11   &     0.24   \\ 
   Ca I    &     4.59   &     0.04   &       19   &     0.06   &     0.04   &     0.06   \\ 
   Sc II   &     1.25   &     0.11   &        4   &    $-$0.01   &     0.12   &     0.16   \\ 
   Ti I    &     3.49   &     0.21   &        1   &     0.43   &     0.06   &     0.22   \\ 
   Ti II   &     3.27   &     0.18   &        3   &     0.21   &     0.12   &     0.22   \\ 
   V I     &     2.31   &     0.33   &        2   &     0.27   &     0.07   &     0.34   \\ 
   Cr I    &     3.68   &     0.05   &        3   &    $-$0.06   &     0.07   &     0.09   \\ 
   Mn I    &     3.07   &     0.07   &        2   &    $-$0.47   &     0.06   &     0.09   \\ 
   Fe II   &     5.91   &     0.04   &        8   &     0.30   &     0.16   &     0.16   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.32   &     0.05   &        6   &    $-$0.01   &     0.04   &     0.06   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.49   &     0.03   &        3   &     0.20   &     0.12   &     0.12   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &     0.11   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC11217 &          &            &            &            &            &            \\ 
   Fe I    &     6.22   &     0.02   &       72   &    $-$1.28\tablenotemark{a}   &     0.14   &     0.14   \\ 
   O I     &     7.69   &     0.16   &        1   &     0.28   &     0.13   &     0.21   \\ 
   Na I    &     4.73   &     0.16   &        1   &    $-$0.23   &     0.07   &     0.17   \\ 
   Mg I    &     6.41   &     0.12   &        2   &     0.09   &     0.03   &     0.12   \\ 
   Al I    &  $<$5.37   &     0.16   &        1   &  $<$0.20   &     0.09   &     0.18   \\ 
   Si I    &     6.34   &     0.08   &        3   &     0.11   &     0.13   &     0.15   \\ 
   Ca I    &     5.19   &     0.03   &       19   &     0.04   &     0.02   &     0.04   \\ 
   Sc II   &     1.83   &     0.08   &        6   &    $-$0.04   &     0.11   &     0.14   \\ 
   Ti I    &     3.79   &     0.03   &        9   &     0.12   &     0.10   &     0.10   \\ 
   Ti II   &     4.03   &     0.06   &        3   &     0.36   &     0.09   &     0.11   \\ 
   V I     &     2.52   &     0.07   &        9   &    $-$0.13   &     0.11   &     0.13   \\ 
   Cr I    &     4.24   &     0.09   &        4   &    $-$0.12   &     0.08   &     0.12   \\ 
   Mn I    &     3.84   &     0.05   &        6   &    $-$0.31   &     0.04   &     0.06   \\ 
   Fe II   &     6.36   &     0.04   &        8   &     0.14   &     0.16   &     0.16   \\ 
   Co I    &     3.30   &     0.16   &        1   &    $-$0.41   &     0.08   &     0.18   \\ 
   Ni I    &     4.82   &     0.06   &        9   &    $-$0.11   &     0.04   &     0.07   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.97   &     0.06   &        3   &     0.07   &     0.09   &     0.11   \\ 
   La II   &    $-$0.06   &     0.06   &        4   &     0.12   &     0.11   &     0.13   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &    $-$0.32   &     0.16   &        1   &     0.44   &     0.12   &     0.20   \\ 
 &          &            &            &            &            &            \\ 
    CC11388 &          &            &            &            &            &            \\ 
   Fe I    &     5.98   &     0.05   &       23   &    $-$1.52\tablenotemark{a}   &     0.13   &     0.14   \\ 
   O I     &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Na I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Mg I    &     6.60   &     0.25   &        1   &     0.52   &     0.05   &     0.25   \\ 
   Al I    &  $<$5.50   &     0.25   &        1   &  $<$0.57   &     0.09   &     0.27   \\ 
   Si I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ca I    &     4.99   &     0.15   &        6   &     0.08   &     0.02   &     0.15   \\ 
   Sc II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ti I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ti II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   V I     &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Cr I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Mn I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Fe II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.66   &     0.25   &        1   &    $-$0.04   &     0.02   &     0.25   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.68   &     0.08   &        2   &     0.02   &     0.11   &     0.14   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC11560 &          &            &            &            &            &            \\ 
   Fe I    &     5.90   &     0.03   &       60   &    $-$1.60\tablenotemark{a}   &     0.14   &     0.14   \\ 
   O I     &     7.67   &     0.20   &        1   &     0.58   &     0.13   &     0.24   \\ 
   Na I    &     4.89   &     0.20   &        1   &     0.25   &     0.06   &     0.21   \\ 
   Mg I    &     6.03   &     0.10   &        2   &     0.03   &     0.04   &     0.11   \\ 
   Al I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Si I    &      ...   &      ...   &      ...   &      ...   &     0.12   &      ...   \\ 
   Ca I    &     4.97   &     0.04   &       15   &     0.15   &     0.02   &     0.04   \\ 
   Sc II   &     1.70   &     0.13   &        4   &     0.16   &     0.12   &     0.18   \\ 
   Ti I    &     3.99   &     0.18   &        3   &     0.65   &     0.07   &     0.19   \\ 
   Ti II   &     3.40   &     0.02   &        2   &     0.05   &     0.10   &     0.10   \\ 
   V I     &     2.66   &     0.38   &        2   &     0.33   &     0.07   &     0.39   \\ 
   Cr I    &     3.84   &     0.13   &        4   &    $-$0.20   &     0.04   &     0.14   \\ 
   Mn I    &     3.63   &     0.23   &        2   &    $-$0.19   &     0.07   &     0.24   \\ 
   Fe II   &     6.26   &     0.07   &        5   &     0.37   &     0.15   &     0.17   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.55   &     0.17   &        4   &    $-$0.06   &     0.03   &     0.17   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.91   &     0.21   &        3   &     0.33   &     0.11   &     0.24   \\ 
   La II   &     0.39   &     0.20   &        1   &     0.89   &     0.11   &     0.23   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC12038 &          &            &            &            &            &            \\ 
   Fe I    &     6.01   &     0.03   &       51   &    $-$1.49\tablenotemark{a}   &     0.15   &     0.15   \\ 
   O I     &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Na I    &     4.50   &     0.22   &        1   &    $-$0.25   &     0.10   &     0.24   \\ 
   Mg I    &     6.53   &     0.22   &        1   &     0.42   &     0.06   &     0.23   \\ 
   Al I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Si I    &     6.57   &     0.42   &        2   &     0.55   &     0.13   &     0.44   \\ 
   Ca I    &     5.09   &     0.07   &       15   &     0.15   &     0.03   &     0.08   \\ 
   Sc II   &     1.56   &     0.07   &        3   &    $-$0.10   &     0.11   &     0.13   \\ 
   Ti I    &     3.75   &     0.20   &        3   &     0.29   &     0.09   &     0.22   \\ 
   Ti II   &     4.03   &     0.23   &        2   &     0.57   &     0.11   &     0.25   \\ 
   V I     &      ...   &      ...   &      ...   &      ...   &     0.09   &      ...   \\ 
   Cr I    &     3.91   &     0.25   &        4   &    $-$0.24   &     0.04   &     0.25   \\ 
   Mn I    &     3.69   &     0.22   &        2   &    $-$0.25   &     0.09   &     0.24   \\ 
   Fe II   &     6.21   &     0.08   &        6   &     0.20   &     0.16   &     0.18   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ni I    &     4.57   &     0.08   &        6   &    $-$0.16   &     0.05   &     0.09   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     1.20   &     0.14   &        3   &     0.51   &     0.11   &     0.18   \\ 
   La II   &     0.20   &     0.22   &        1   &     0.59   &     0.12   &     0.25   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
 &          &            &            &            &            &            \\ 
    CC12039 &          &            &            &            &            &            \\ 
   Fe I    &     5.89   &     0.02   &       73   &    $-$1.61\tablenotemark{a}   &     0.12   &     0.12   \\ 
   O I     &     7.58   &     0.16   &        1   &     0.50   &     0.13   &     0.21   \\ 
   Na I    &     4.46   &     0.16   &        1   &    $-$0.17   &     0.08   &     0.18   \\ 
   Mg I    &     6.32   &     0.14   &        2   &     0.34   &     0.04   &     0.15   \\ 
   Al I    &  $<$5.37   &     0.16   &        1   &  $<$0.53   &     0.09   &     0.18   \\ 
   Si I    &     6.11   &     0.16   &        1   &     0.21   &     0.12   &     0.20   \\ 
   Ca I    &     4.86   &     0.05   &       18   &     0.04   &     0.02   &     0.05   \\ 
   Sc II   &     1.66   &     0.05   &        6   &     0.12   &     0.12   &     0.13   \\ 
   Ti I    &     3.50   &     0.06   &        4   &     0.16   &     0.08   &     0.10   \\ 
   Ti II   &     3.63   &     0.11   &        3   &     0.29   &     0.12   &     0.16   \\ 
   V I     &     2.16   &     0.17   &        3   &    $-$0.16   &     0.08   &     0.19   \\ 
   Cr I    &     3.93   &     0.06   &        4   &    $-$0.10   &     0.08   &     0.10   \\ 
   Mn I    &     3.52   &     0.04   &        4   &    $-$0.30   &     0.07   &     0.08   \\ 
   Fe II   &     6.01   &     0.05   &        7   &     0.12   &     0.16   &     0.17   \\ 
   Co I    &      ...   &      ...   &      ...   &      ...   &     0.07   &      ...   \\ 
   Ni I    &     4.55   &     0.06   &        9   &    $-$0.05   &     0.04   &     0.07   \\ 
   Cu I    &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Ba II   &     0.72   &     0.03   &        3   &     0.15   &     0.11   &     0.11   \\ 
   La II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Nd II   &      ...   &      ...   &      ...   &      ...   &      ...   &      ...   \\ 
   Eu II   &    $-$0.57   &     0.16   &        1   &     0.52   &     0.12   &     0.20   \\ 
 &          &            &            &            &            &            \\ 
\enddata 
\tablenotetext{a}{[Fe/H]}                                                                                                     
\end{deluxetable}      


==> table7.tex <==
% Table 7

\begin{deluxetable}{lrrrrr}                                                                                                                  
\tablecolumns{6}                                                                                                                            
\tablewidth{0pt}                                                                                                                  
\tablecaption{\label{tab:errors}Average Abundance Uncertainties in [Fe/H] and [X/Fe]}                   
\tablehead{                                                                                                                              
  \colhead{Species} & {$\sigma_{T_{\rm eff}}$} & {$\sigma_{{\rm log}g}$} & {$\sigma_{\rm [M/H]}$} & {$\sigma_{\xi{_t}}$} & {$\sigma_{\rm [X/Fe]}$} \\   
             {}     & {(80~K)}             & {(0.07~dex)}           & {(0.15~dex)}            & {(0.2~{\rm km~s$^{-1}$})}     &                         \\
           {(1)}    & {(2)}                & {(3)}                  &{(4)}                   &{(5)}               & {(6)}        
}                                                                                                                                       
\startdata                                                                                                          
   Fe I\tablenotemark{a}   &    0.109  &   $-$0.001  &   $-$0.015  &   $-$0.082  &    0.136 \\
   O I    &   $-$0.099  &      0.029  &    0.097  &    0.078  &    0.128 \\
   Na I   &   $-$0.043  &   $-$0.004  &    0.000  &    0.070  &    0.084 \\
   Mg I   &   $-$0.035  &   $-$0.008  &    0.002  &    0.018  &    0.047 \\
   Al I   &   $-$0.048  &   $-$0.002  &    0.004  &    0.077  &    0.092 \\
   Si I   &   $-$0.099  &      0.007  &    0.030  &    0.078  &    0.123 \\
   Ca I   &   $-$0.015  &   $-$0.005  & $-$0.010  &    0.016  &    0.027 \\
   Sc II  &   $-$0.115  &      0.028  &    0.074  &    0.042  &    0.111 \\
   Ti I   &      0.034  &   $-$0.004  & $-$0.011  &    0.073  &    0.079 \\
   Ti II  &   $-$0.116  &      0.026  &    0.069  &    0.007  &    0.104 \\
   V I    &      0.051  &   $-$0.004  & $-$0.011  &    0.071  &    0.086 \\
   Cr I   &      0.050  &   $-$0.002  & $-$0.021  & $-$0.019  &    0.054 \\
   Mn I   &      0.025  &   $-$0.002  & $-$0.006  &    0.052  &    0.057 \\
   Fe II  &   $-$0.163  &      0.032  &    0.079  &    0.053  &    0.153 \\
   Co I   &      0.000  &      0.002  &    0.015  &    0.083  &    0.084 \\
   Ni I   &   $-$0.001  &      0.005  &    0.016  &    0.044  &    0.046 \\
   Cu I   &      0.004  &      0.004  &    0.016  &    0.086  &    0.087 \\
   Ba II  &   $-$0.080  &      0.027  &    0.074  & $-$0.064  &    0.100 \\
   La II  &   $-$0.084  &      0.028  &    0.079  &    0.075  &    0.111 \\
   Nd II  &   $-$0.082  &      0.028  &    0.073  &    0.051  &    0.092 \\
   Eu II  &   $-$0.110  &      0.025  &    0.077  &    0.073  &    0.126 \\
\enddata                                                                                                      
\tablenotetext{a}{Errors pertain to uncertainties in [Fe/H]}
\end{deluxetable}      


==> table8.tex <==
% Table 8
\begin{deluxetable}{lrrrrrrrrrrrrrrrrrrrrr}                                                                                    
\tabletypesize{\tiny}                                                                                                   
\tablecolumns{22}                                                                                                       
\tablewidth{0pt}                                                                                                        
\rotate                                                                                                                 
\tablecaption{\label{tab:relabs_gil} Summary\tablenotemark{a} of [Fe/H], [X/Fe], and Total Errors $\sigma_{\rm {Tot}}$ for 32 Carina Red Giants}                          

\tablehead{                                                                                                                              
  \colhead{Object} & {[Fe/H]} & {O}  & {Na} & {Mg} & {Al} & {Si} & {Ca} & {Sc} & {Ti~I} & {Ti~II} & {V} & {Cr} & {Mn} & {Fe~II} & {Co} & {Ni} & {Cu} & {Ba} & {La} & {Nd} & {Eu}\\  
  }
\startdata    

    CC06122   &  $-$1.43  &   0.32 &  $-$0.20 &   0.31 & $<$ 0.36 &   0.21 &   0.09 &   0.17 &   0.15 &   0.34 &  $-$0.07 &  $-$0.01 &  $-$0.32 &   0.09 &  $-$0.03 &  $-$0.08 &  $-$0.63 &   0.44 &   0.49 &    ... &    ... \\
               &   0.14   &   0.21 &   0.19 &   0.18 &   0.20 &   0.22 &   0.04 &   0.18 &   0.10 &   0.13 &   0.16 &   0.10 &   0.07 &   0.17 &   0.19 &   0.09 &   0.19 &   0.14 &   0.13 &    ... &    ... \\
               &     74   &      1 &      1 &      2 &      1 &      1 &     19 &      5 &      8 &      2 &     10 &      4 &      5 &      8 &      1 &     10 &      1 &      3 &      3 &    ... &    ... \\
               &          &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC06486    &  $-$2.03 & $<$ 0.80 &   0.19 &   0.17 & $<$ 1.28 &    ... &   0.11 &   0.14 &    ... &    ... &    ... &  $-$0.16 &    ... &   0.42 &    ... &   0.08 &    ... &  $-$0.45 &    ... &    ... &    ... \\
               &   0.16   &   0.29 &   0.28 &   0.12 &   0.28 &    ... &   0.09 &   0.29 &    ... &    ... &    ... &   0.13 &    ... &   0.30 &    ... &   0.11 &    ... &   0.23 &    ... &    ... &    ... \\
               &     42   &      1 &      1 &      2 &      1 &    ... &     13 &      1 &    ... &    ... &    ... &      3 &    ... &      1 &    ... &      5 &    ... &      3 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC06975   &  $-$1.84 & $<$ 0.81 & $<$$-$0.02 &   0.27 & $<$ 1.17 &    ... &   0.14 &   0.39 &    ... &   0.17 &    ... &  $-$0.03 &  $-$0.13 &   0.55 &    ... &   0.10 &    ... &   0.39 &    ... &   0.41 &    ... \\
               &   0.14 &   0.25 &   0.24 &   0.05 &   0.24 &    ... &   0.06 &   0.40 &    ... &   0.18 &    ... &   0.09 &   0.23 &   0.34 &    ... &   0.15 &    ... &   0.12 &    ... &   0.24 &    ... \\
               &     53 &      1 &      1 &      2 &      1 &    ... &     14 &      2 &    ... &      2 &    ... &      2 &      1 &      2 &    ... &      5 &    ... &      3 &    ... &      1 &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC07452   &  $-$1.29 &    ... &  $-$0.69 &  $-$0.38 & $<$ 0.06 &    ... &  $-$0.32 &  $-$0.90 &  $-$0.32 &  $-$0.15 &  $-$0.69 &  $-$0.13 &  $-$0.33 &   0.24 &    ... &  $-$0.43 &    ... &  $-$0.74 &    ... &    ... &    ... \\
               &   0.13 &    ... &   0.19 &   0.20 &   0.20 &    ... &   0.06 &   0.21 &   0.15 &   0.16 &   0.22 &   0.09 &   0.08 &   0.17 &    ... &   0.08 &    ... &   0.11 &    ... &    ... &    ... \\
               &     82 &    ... &      1 &      2 &      1 &    ... &     19 &      1 &      5 &      4 &      5 &      4 &      5 &     12 &    ... &      7 &    ... &      3 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC07889   &  $-$2.29 & $<$ 1.23 & $<$ 0.77 &   0.82 & $<$ 1.72 &    ... &   0.16 &   0.12 &    ... &   0.33 &    ... &  $-$0.42 &    ... &   0.65 &    ... &   0.43 &    ... &  $-$0.79 &    ... &    ... &    ... \\
               &   0.13 &   0.23 &   0.23 &   0.23 &   0.23 &    ... &   0.09 &   0.24 &    ... &   0.24 &    ... &   0.16 &    ... &   0.35 &    ... &   0.23 &    ... &   0.12 &    ... &    ... &    ... \\
               &     27 &      1 &      1 &      1 &      1 &    ... &      8 &      1 &    ... &      1 &    ... &      2 &    ... &      2 &    ... &      1 &    ... &      2 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC08447   &  $-$1.48 &    ... &  $-$0.21 &   0.28 &    ... &   0.10 &   0.08 &   0.01 &   0.13 &   0.55 &   0.02 &  $-$0.07 &  $-$0.29 &   0.32 &    ... &  $-$0.27 &  $-$0.48 &   0.11 &    ... &    ... &    ... \\
               &   0.13 &    ... &   0.20 &   0.23 &    ... &   0.22 &   0.04 &   0.16 &   0.10 &   0.13 &   0.16 &   0.10 &   0.14 &   0.19 &    ... &   0.09 &   0.20 &   0.14 &    ... &    ... &    ... \\
               &     72 &    ... &      1 &      2 &    ... &      1 &     18 &      6 &      4 &      3 &      7 &      4 &      4 &      9 &    ... &      6 &      1 &      3 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC08469   &  $-$1.34 &   0.30 &  $-$0.44 &  $-$0.02 & $<$ 0.31 &   0.42 &   0.01 &  $-$0.03 &   0.13 &  $-$0.01 &  $-$0.13 &  $-$0.25 &  $-$0.43 &   0.22 &    ... &  $-$0.10 &  $-$0.56 &   0.15 &   0.24 &    ... &    ... \\
               &   0.14 &   0.26 &   0.24 &   0.07 &   0.24 &   0.16 &   0.04 &   0.13 &   0.09 &   0.25 &   0.14 &   0.17 &   0.11 &   0.19 &    ... &   0.05 &   0.24 &   0.11 &   0.14 &    ... &    ... \\
               &     68 &      1 &      1 &      2 &      1 &      3 &     19 &      6 &      9 &      2 &      4 &      4 &      4 &      9 &    ... &      8 &      1 &      3 &      2 &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC08615   &  $-$1.73 &   0.55 &  $-$0.06 &   0.52 & $<$ 0.92 &   0.56 &   0.18 &   0.05 &   0.45 &   0.05 &    ... &  $-$0.19 &    ... &   0.38 &    ... &   0.14 &    ... &   0.26 &   0.64 &    ... &    ... \\
               &   0.11 &   0.24 &   0.23 &   0.24 &   0.23 &   0.24 &   0.05 &   0.24 &   0.25 &   0.25 &    ... &   0.04 &    ... &   0.16 &    ... &   0.15 &    ... &   0.33 &   0.24 &    ... &    ... \\
               &     56 &      1 &      1 &      2 &      1 &      1 &     18 &      2 &      2 &      3 &    ... &      3 &    ... &      5 &    ... &      6 &    ... &      3 &      1 &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC08695   &  $-$1.29 &   0.21 &  $-$0.14 &   0.12 &    ... &   0.14 &   0.05 &  $-$0.08 &   0.08 &   0.32 &  $-$0.19 &  $-$0.37 &  $-$0.59 &   0.21 &  $-$0.27 &  $-$0.24 &  $-$0.78 &   0.22 &   0.25 &   0.10 &   0.55 \\
               &   0.14 &   0.23 &   0.20 &   0.14 &    ... &   0.22 &   0.06 &   0.14 &   0.11 &   0.21 &   0.16 &   0.13 &   0.09 &   0.18 &   0.21 &   0.09 &   0.21 &   0.09 &   0.22 &   0.20 &   0.22 \\
               &     71 &      1 &      1 &      2 &    ... &      1 &     18 &      5 &      8 &      3 &      8 &      4 &      6 &      9 &      1 &      8 &      1 &      3 &      1 &      1 &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC08788   &  $-$1.48 &    ... &  $-$0.13 &   0.26 & $<$ 0.69 &   0.06 &   0.14 &   0.36 &   0.38 &   0.05 &   0.39 &  $-$0.19 &   0.01 &   0.33 &    ... &   0.01 &    ... &   0.04 &    ... &    ... &   0.80 \\
               &   0.13 &    ... &   0.24 &   0.14 &   0.23 &   0.24 &   0.07 &   0.21 &   0.34 &   0.10 &   0.29 &   0.07 &   0.11 &   0.17 &    ... &   0.13 &    ... &   0.13 &    ... &    ... &   0.25 \\
               &     52 &    ... &      1 &      2 &      1 &      1 &     15 &      4 &      2 &      2 &      3 &      3 &      2 &      7 &    ... &      8 &    ... &      2 &    ... &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC09000   &  $-$1.82 &    ... & $<$$-$0.48 &  $-$0.23 & $<$ 0.60 &    ... &  $-$0.22 &  $-$0.25 &  $-$0.08 &   0.46 &  $-$0.18 &  $-$0.19 &  $-$0.44 &   0.42 &    ... &  $-$0.25 &    ... &   0.28 &   0.48 &   0.53 &   0.84 \\
               &   0.13 &    ... &   0.18 &   0.16 &   0.18 &    ... &   0.04 &   0.16 &   0.09 &   0.21 &   0.33 &   0.09 &   0.06 &   0.15 &    ... &   0.06 &    ... &   0.10 &   0.19 &   0.17 &   0.20 \\
               &     68 &    ... &      1 &      2 &      1 &    ... &     16 &      3 &      3 &      2 &      2 &      4 &      3 &      9 &    ... &      9 &    ... &      3 &      1 &      1 &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC09179   &  $-$1.78 & $<$ 0.57 & $<$$-$0.26 &   0.03 & $<$ 0.81 &   0.84 &  $-$0.14 &  $-$0.22 &    ... &  $-$0.08 &   0.29 &  $-$0.13 &    ... &   0.31 &    ... &  $-$0.28 &    ... &   0.41 &    ... &    ... &   0.95 \\
               &   0.15 &   0.25 &   0.23 &   0.38 &   0.23 &   0.24 &   0.08 &   0.17 &    ... &   0.12 &   0.22 &   0.12 &    ... &   0.16 &    ... &   0.10 &    ... &   0.16 &    ... &    ... &   0.25 \\
               &     59 &      1 &      1 &      2 &      1 &      1 &     14 &      2 &    ... &      2 &      1 &      3 &    ... &      7 &    ... &      3 &    ... &      3 &    ... &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC09225   &  $-$1.57 &   0.48 &  $-$0.34 &   0.36 & $<$ 0.51 &   0.08 &   0.08 &   0.05 &   0.23 &   0.51 &  $-$0.05 &  $-$0.26 &  $-$0.32 &   0.16 &   0.08 &   0.00 &    ... &   0.30 &   0.73 &   0.21 &    ... \\
               &   0.13 &   0.21 &   0.19 &   0.07 &   0.19 &   0.21 &   0.07 &   0.13 &   0.14 &   0.18 &   0.20 &   0.10 &   0.09 &   0.17 &   0.19 &   0.07 &    ... &   0.13 &   0.20 &   0.20 &    ... \\
               &     69 &      1 &      1 &      2 &      1 &      1 &     20 &      6 &      2 &      3 &      6 &      4 &      3 &      8 &      1 &      8 &    ... &      3 &      1 &      1 &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC09226   &  $-$1.56 &   0.45 &  $-$0.22 &   0.18 & $<$ 0.62 &   0.34 &   0.11 &   0.10 &    ... &   0.24 &   0.58 &  $-$0.06 &  $-$0.17 &   0.15 &    ... &  $-$0.09 &    ... &   0.45 &   1.15 &    ... &    ... \\
               &   0.13 &   0.27 &   0.26 &   0.15 &   0.26 &   0.29 &   0.06 &   0.16 &    ... &   0.18 &   0.19 &   0.13 &   0.25 &   0.17 &    ... &   0.07 &    ... &   0.21 &   0.26 &    ... &    ... \\
               &     65 &      1 &      1 &      2 &      1 &      2 &     15 &      4 &    ... &      3 &      2 &      4 &      1 &      6 &    ... &      7 &    ... &      3 &      1 &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC09430   &  $-$2.13 & $<$ 0.79 & $<$ 0.07 &   0.75 & $<$ 1.26 &    ... &   0.14 &   0.38 &    ... &   0.37 &    ... &  $-$0.28 &   0.44 &   0.37 &    ... &  $-$0.03 &    ... &  $-$0.13 &    ... &    ... &    ... \\
               &   0.15 &   0.22 &   0.21 &   0.22 &   0.21 &    ... &   0.09 &   0.12 &    ... &   0.21 &    ... &   0.07 &   0.09 &   0.24 &    ... &   0.07 &    ... &   0.12 &    ... &    ... &    ... \\
               &     46 &      1 &      1 &      2 &      1 &    ... &     13 &      4 &    ... &      3 &    ... &      3 &      2 &      3 &    ... &      4 &    ... &      2 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC09507   &  $-$1.72 & $<$ 0.58 & $<$$-$0.27 &  $-$0.12 & $<$ 0.92 &    ... &  $-$0.11 &  $-$0.08 &    ... &  $-$0.14 &   0.51 &   0.17 &   0.24 &   0.20 &    ... &  $-$0.27 &    ... &   0.51 &   0.72 &   0.31 &    ... \\
               &   0.12 &   0.25 &   0.23 &   0.07 &   0.24 &    ... &   0.06 &   0.19 &    ... &   0.24 &   0.23 &   0.13 &   0.23 &   0.16 &    ... &   0.10 &    ... &   0.13 &   0.24 &   0.24 &    ... \\
               &     58 &      1 &      1 &      2 &      1 &    ... &     15 &      5 &    ... &      1 &      1 &      3 &      1 &      4 &    ... &      6 &    ... &      2 &      1 &      1 &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC09633   &  $-$2.50 & $<$ 1.14 & $<$ 0.53 &   0.15 & $<$ 1.72 &    ... &   0.11 &   0.45 &    ... &   0.09 &    ... &  $-$0.26 &   0.21 &   0.48 &    ... &  $-$0.08 &    ... &  $-$1.00 &    ... &    ... &    ... \\
               &   0.15 &   0.25 &   0.24 &   0.24 &   0.25 &    ... &   0.09 &   0.16 &    ... &   0.16 &    ... &   0.04 &   0.24 &   0.14 &    ... &   0.23 &    ... &   0.24 &    ... &    ... &    ... \\
               &     34 &      1 &      1 &      1 &      1 &    ... &     10 &      2 &    ... &      2 &    ... &      3 &      1 &      2 &    ... &      1 &    ... &      1 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC09869   &  $-$1.26 &    ... &  $-$0.19 &   0.19 & $<$ 0.30 &   0.13 &   0.06 &   0.14 &   0.05 &   0.29 &  $-$0.28 &   0.04 &  $-$0.34 &   0.09 &    ... &  $-$0.12 &    ... &   0.13 &   0.41 &    ... &    ... \\
               &   0.15 &    ... &   0.22 &   0.04 &   0.23 &   0.14 &   0.06 &   0.14 &   0.10 &   0.23 &   0.16 &   0.13 &   0.07 &   0.18 &    ... &   0.08 &    ... &   0.17 &   0.13 &    ... &    ... \\
               &     66 &    ... &      1 &      2 &      1 &      2 &     18 &      5 &      3 &      4 &      5 &      4 &      4 &      6 &    ... &      9 &    ... &      3 &      2 &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC09929   &  $-$1.50 &   0.76 &  $-$0.39 &   0.16 & $<$ 0.69 &   0.21 &   0.24 &   0.20 &    ... &   0.21 &   0.16 &   0.00 &  $-$0.32 &   0.29 &    ... &   0.03 &    ... &   0.40 &   0.73 &    ... &   0.85 \\
               &   0.15 &   0.26 &   0.24 &   0.08 &   0.24 &   0.26 &   0.08 &   0.22 &    ... &   0.17 &   0.11 &   0.10 &   0.16 &   0.19 &    ... &   0.10 &    ... &   0.14 &   0.12 &    ... &   0.26 \\
               &     40 &      1 &      1 &      2 &      1 &      1 &     16 &      4 &    ... &      3 &      2 &      4 &      4 &      3 &    ... &      7 &    ... &      2 &      3 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC10038   &  $-$1.30 &   0.54 &  $-$0.29 &   0.24 & $<$ 0.46 &   0.33 &  $-$0.02 &   0.03 &  $-$0.03 &   0.35 &  $-$0.15 &  $-$0.02 &  $-$0.42 &   0.06 &  $-$0.04 &  $-$0.20 &    ... &   0.10 &    ... &    ... &    ... \\
               &   0.15 &   0.23 &   0.21 &   0.25 &   0.21 &   0.18 &   0.08 &   0.10 &   0.20 &   0.17 &   0.12 &   0.09 &   0.13 &   0.16 &   0.21 &   0.08 &    ... &   0.17 &    ... &    ... &    ... \\
               &     63 &      1 &      1 &      2 &      1 &      3 &     17 &      6 &      3 &      3 &      2 &      4 &      5 &      9 &      1 &      8 &    ... &      3 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC10194   &  $-$1.42 &   0.17 &  $-$0.31 &   0.15 & $<$ 0.42 &   0.18 &   0.01 &  $-$0.27 &   0.21 &   0.23 &  $-$0.25 &   0.00 &  $-$0.90 &  $-$0.01 &    ... &  $-$0.25 &    ... &   0.13 &   0.24 &  $-$0.31 &    ... \\
               &   0.15 &   0.27 &   0.24 &   0.14 &   0.25 &   0.27 &   0.08 &   0.15 &   0.19 &   0.16 &   0.19 &   0.23 &   0.17 &   0.21 &    ... &   0.12 &    ... &   0.22 &   0.26 &   0.25 &    ... \\
               &     53 &      1 &      1 &      2 &      1 &      1 &     16 &      4 &      5 &      2 &      5 &      4 &      3 &      5 &    ... &      7 &    ... &      3 &      1 &      1 &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC10318   &  $-$1.59 &   0.65 & $<$$-$0.42 &   0.10 & $<$ 0.58 &   0.31 &   0.02 &   0.48 &   0.19 &   0.57 &  $-$0.31 &  $-$0.18 &  $-$0.36 &   0.27 &   0.15 &  $-$0.01 &    ... &   0.28 &   0.49 &   0.33 &    ... \\
               &   0.14 &   0.23 &   0.21 &   0.21 &   0.21 &   0.16 &   0.06 &   0.14 &   0.11 &   0.26 &   0.21 &   0.11 &   0.09 &   0.19 &   0.21 &   0.08 &    ... &   0.35 &   0.22 &   0.21 &    ... \\
               &     59 &      1 &      1 &      2 &      1 &      2 &     15 &      5 &      4 &      2 &      3 &      4 &      4 &      7 &      1 &      8 &    ... &      3 &      1 &      1 &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC10414   &  $-$1.35 &   0.57 &  $-$0.76 &   0.10 &    ... &   0.29 &   0.12 &   0.00 &   0.08 &   0.04 &  $-$0.04 &  $-$0.22 &  $-$0.32 &   0.11 &    ... &  $-$0.13 &  $-$0.32 &  $-$0.26 &   0.34 &   0.36 &   0.62 \\
               &   0.14 &   0.26 &   0.24 &   0.25 &    ... &   0.14 &   0.07 &   0.18 &   0.09 &   0.12 &   0.34 &   0.18 &   0.15 &   0.17 &    ... &   0.09 &   0.23 &   0.21 &   0.25 &   0.24 &   0.25 \\
               &     57 &      1 &      1 &      2 &    ... &      2 &     18 &      4 &      3 &      3 &      3 &      4 &      5 &      8 &    ... &      8 &      1 &      3 &      1 &      1 &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC10686   &  $-$1.68 &   0.56 &  $-$0.21 &   0.30 & $<$ 0.52 &   0.24 &   0.07 &   0.13 &   0.10 &   0.32 &  $-$0.29 &  $-$0.19 &  $-$0.56 &   0.17 &   0.07 &  $-$0.06 &  $-$0.64 &   0.27 &   0.38 &    ... &   0.44 \\
               &   0.13 &   0.21 &   0.19 &   0.19 &   0.19 &   0.21 &   0.03 &   0.14 &   0.09 &   0.16 &   0.15 &   0.08 &   0.11 &   0.16 &   0.19 &   0.06 &   0.19 &   0.12 &   0.15 &    ... &   0.21 \\
               &     75 &      1 &      1 &      2 &      1 &      1 &     17 &      6 &      6 &      3 &      4 &      4 &      3 &      8 &      1 &      8 &      1 &      3 &      2 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC10690   &  $-$1.96 & $<$ 0.64 & $<$$-$0.13 &  $-$0.42 & $<$ 1.05 &    ... &  $-$0.24 &  $-$0.27 &    ... &   0.30 &    ... &  $-$0.39 &    ... &   0.34 &    ... &  $-$0.37 &    ... &  $-$0.22 &    ... &    ... &    ... \\
               &   0.14 &   0.21 &   0.20 &   0.19 &   0.20 &    ... &   0.07 &   0.21 &    ... &   0.30 &    ... &   0.12 &    ... &   0.15 &    ... &   0.13 &    ... &   0.11 &    ... &    ... &    ... \\
               &     55 &      1 &      1 &      1 &      1 &    ... &     14 &      1 &    ... &      3 &    ... &      3 &    ... &      6 &    ... &      3 &    ... &      3 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC10802   &  $-$1.27 &    ... &  $-$0.50 &  $-$0.05 & $<$ 0.60 &   0.45 &   0.13 &  $-$0.09 &   0.63 &   0.31 &  $-$0.16 &   0.09 &  $-$0.30 &   0.42 &   0.42 &  $-$0.11 &    ... &   0.19 &    ... &    ... &    ... \\
               &   0.14 &    ... &   0.24 &   0.43 &   0.24 &   0.25 &   0.13 &   0.13 &   0.36 &   0.25 &   0.11 &   0.20 &   0.22 &   0.20 &   0.23 &   0.17 &    ... &   0.25 &    ... &    ... &    ... \\
               &     48 &    ... &      1 &      2 &      1 &      1 &     12 &      3 &      3 &      1 &      2 &      3 &      1 &      4 &      1 &      5 &    ... &      3 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC10944   &  $-$1.89 &    ... &    ... &   0.26 & $<$ 1.06 &   0.44 &   0.06 &  $-$0.01 &   0.43 &   0.21 &   0.27 &  $-$0.06 &  $-$0.47 &   0.30 &    ... &  $-$0.01 &    ... &   0.20 &    ... &    ... &    ... \\
               &   0.12 &    ... &    ... &   0.13 &   0.22 &   0.24 &   0.06 &   0.16 &   0.22 &   0.22 &   0.34 &   0.09 &   0.09 &   0.16 &    ... &   0.06 &    ... &   0.12 &    ... &    ... &    ... \\
               &     62 &    ... &    ... &      2 &      1 &      1 &     19 &      4 &      1 &      3 &      2 &      3 &      2 &      8 &    ... &      6 &    ... &      3 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC11217   &  $-$1.28 &   0.28 &  $-$0.23 &   0.09 & $<$ 0.20 &   0.11 &   0.04 &  $-$0.04 &   0.12 &   0.36 &  $-$0.13 &  $-$0.12 &  $-$0.31 &   0.14 &  $-$0.41 &  $-$0.11 &    ... &   0.07 &   0.12 &    ... &   0.44 \\
               &   0.14 &   0.21 &   0.17 &   0.12 &   0.18 &   0.15 &   0.04 &   0.14 &   0.10 &   0.11 &   0.13 &   0.12 &   0.06 &   0.16 &   0.18 &   0.07 &    ... &   0.11 &   0.13 &    ... &   0.20 \\
               &     72 &      1 &      1 &      2 &      1 &      3 &     19 &      6 &      9 &      3 &      9 &      4 &      6 &      8 &      1 &      9 &    ... &      3 &      4 &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC11388   &  $-$1.52 &    ... &    ... &   0.52 & $<$ 0.57 &    ... &   0.08 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &  $-$0.04 &    ... &   0.02 &    ... &    ... &    ... \\
               &   0.14 &    ... &    ... &   0.25 &   0.27 &    ... &   0.15 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &   0.25 &    ... &   0.14 &    ... &    ... &    ... \\
               &     23 &    ... &    ... &      1 &      1 &    ... &      6 &    ... &    ... &    ... &    ... &    ... &    ... &    ... &    ... &      1 &    ... &      2 &    ... &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC11560   &  $-$1.60 &   0.58 &   0.25 &   0.03 &    ... &    ... &   0.15 &   0.16 &   0.65 &   0.05 &   0.33 &  $-$0.20 &  $-$0.19 &   0.37 &    ... &  $-$0.06 &    ... &   0.33 &   0.89 &    ... &    ... \\
               &   0.14 &   0.24 &   0.21 &   0.11 &    ... &    ... &   0.04 &   0.18 &   0.19 &   0.10 &   0.39 &   0.14 &   0.24 &   0.17 &    ... &   0.17 &    ... &   0.24 &   0.23 &    ... &    ... \\
               &     60 &      1 &      1 &      2 &    ... &    ... &     15 &      4 &      3 &      2 &      2 &      4 &      2 &      5 &    ... &      4 &    ... &      3 &      1 &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC12038   &  $-$1.49 &    ... &  $-$0.25 &   0.42 &    ... &   0.55 &   0.15 &  $-$0.10 &   0.29 &   0.57 &    ... &  $-$0.24 &  $-$0.25 &   0.20 &    ... &  $-$0.16 &    ... &   0.51 &   0.59 &    ... &    ... \\
               &   0.15 &    ... &   0.24 &   0.23 &    ... &   0.44 &   0.08 &   0.13 &   0.22 &   0.25 &    ... &   0.25 &   0.24 &   0.18 &    ... &   0.09 &    ... &   0.18 &   0.25 &    ... &    ... \\
               &     51 &    ... &      1 &      1 &    ... &      2 &     15 &      3 &      3 &      2 &    ... &      4 &      2 &      6 &    ... &      6 &    ... &      3 &      1 &    ... &    ... \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
    CC12039   &  $-$1.61 &   0.50 &  $-$0.17 &   0.34 & $<$ 0.53 &   0.21 &   0.04 &   0.12 &   0.16 &   0.29 &  $-$0.16 &  $-$0.10 &  $-$0.30 &   0.12 &    ... &  $-$0.05 &    ... &   0.15 &    ... &    ... &   0.52 \\
               &   0.12 &   0.21 &   0.18 &   0.15 &   0.18 &   0.20 &   0.05 &   0.13 &   0.10 &   0.16 &   0.19 &   0.10 &   0.08 &   0.17 &    ... &   0.07 &    ... &   0.11 &    ... &    ... &   0.20 \\
               &     73 &      1 &      1 &      2 &      1 &      1 &     18 &      6 &      4 &      3 &      3 &      4 &      4 &      7 &    ... &      9 &    ... &      3 &    ... &    ... &      1 \\
               &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        \\
\enddata                                                                        
\tablenotetext{a}{For each object the three rows contain [Fe/H] and [X/Fe]; $\sigma_{\rm {Tot}}$; and the number of lines, respectively.}
\end{deluxetable}      


==> table9.tex <==
% Table 9

\begin{deluxetable}{lcrrrrrrrrrrrr}                                                                                                                   
\tablecolumns{14}                                                                                                                            
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\rotate
\tablecaption{\label{tab:litdat} Coordinates, Photometry, and Atmospheric Parameters for 49 Carina Red Giants from the Literature}                  
\tablehead{                                                                                                                              
  \colhead{Object} & {Source\tablenotemark{a}} & {RA   (2000)  Dec } & {$V$}       & {$B$-$V$}        &    {$I$} 

&    {$J$}  &     {$H$} &     {$K$} &  {$T_{\rm eff}$} &  {$\sigma$$T_{\rm eff}$}& {log~$gf$} &  {[Fe/H]}& {$\xi_t$}  \\  
            {(1)}  & {(2)}    &         {(3)}       & {(4)}       &    {(5)}       &    {(6)} &    {(7)}  &     {(8)} &     {(9)} &  {(10)} &        {(11)}    &  {(12)}  &   {(13)} & {(14)}   
  }                                                                                      
\startdata                                                                                                                               
Car-484    & 1 &   06 41 39.64 $-$50 49 58.8 &   17.60 &    1.43 &   16.18 &   15.23 &   14.48 &   14.34    & 4284 &  60 &  0.68 & $-$1.53   & 2.25 \\
Car-524    & 1 &   06 41 14.71 $-$50 51 10.1 &   17.62 &    1.31 &   16.29 &   15.37 &   14.75 &   14.59    & 4436 &  71 &  0.79 & $-$1.72   & 2.50 \\
Car-612    & 1 &   06 40 58.46 $-$50 53 35.5 &   17.80 &    1.29 &   16.41 &   15.52 &   14.88 &   14.74    & 4437 &  65 &  0.87 & $-$1.34   & 2.35 \\
Car-705    & 1 &   06 42 17.43 $-$50 55 55.3 &   17.81 &    1.29 &   16.43 &   15.47 &   14.80 &   14.64    & 4337 &  68 &  0.81 & $-$1.47   & 2.25 \\
Car-769    & 1 &   06 41 19.70 $-$50 57 25.6 &   18.01 &    1.21 &   16.71 &   15.74 &   15.14 &   15.02    & 4438 &  93 &  0.95 & $-$1.64   & 2.30 \\
Car-1013    & 1 &   06 41 21.98 $-$51 03 43.3 &   17.78 &    1.27 &   16.42 &   15.50 &   14.83 &   14.71    & 4412 &  65 &  0.84 & $-$1.62   & 2.35 \\
Car-1087    & 1 &   06 41 15.47 $-$51 01 16.0 &   18.03 &    1.14 &   16.74 &   15.84 &   15.28 &   15.14    & 4542 &  78 &  1.02 & $-$2.79   & 2.05 \\
Car-5070    & 1 &   06 41 53.85 $-$50 58 11.2 &   17.88 &    1.21 &   16.53 &   15.62 &   15.04 &   14.90    & 4487 &  80 &  0.93 & $-$2.24   & 1.80 \\
Car-7002    & 1 &   06 40 49.17 $-$51 00 33.4 &   18.33 &    0.97 &   17.15 &   16.31 &   15.79 &   15.66    & 4708 &  75 &  1.23 & $-$2.67   & 2.65 \\
M2       & 2 &   06 41 57.63 $-$50 59 32.8 &   17.97 &    1.25 &   16.61 &   15.65 &   14.99 &   14.84    & 4359 &  69 &  0.89 & $-$1.53   & 2.10 \\
M3       & 2 &   06 41 54.60 $-$50 57 00.9 &   17.67 &    1.49 &   16.10 &   15.06 &   14.44 &   14.27    & 4230 & 116 &  0.67 & $-$1.79   & 2.35 \\
M4       & 2 &   06 41 48.23 $-$50 55 01.8 &   17.61 &    1.39 &   16.19 &   15.20 &   14.52 &   14.37    & 4291 &  78 &  0.69 & $-$1.48   & 2.05 \\
M10      & 2 &   06 41 46.37 $-$51 01 22.8 &   17.89 &    1.27 &   16.50 &   15.54 &   14.95 &   14.81    & 4411 &  94 &  0.89 & $-$2.01   & 2.10 \\
M12      & 2 &   06 41 36.49 $-$50 56 23.3 &   17.88 &    1.29 &   16.53 &   15.53 &   14.90 &   14.74    & 4337 &  89 &  0.84 & $-$1.32   & 1.90 \\
MKV0397    & 3 &   06 41 58.27 $-$50 46 41.4 &   18.51 &    1.09 &   17.24 &   16.35 &   15.79 &   15.67    & 4567 &  83 &  1.24 & $-$2.01   & 2.35 \\
MKV0458    & 3 &   06 41 58.20 $-$50 48 58.0 &   18.48 &    1.09 &   17.25 &   16.41 &   15.79 &   15.66    & 4586 &  57 &  1.24 & $-$1.45   & 2.05 \\
MKV0514    & 3 &   06 41 46.00 $-$50 51 00.6 &   18.17 &    1.24 &   16.89 &   16.01 &   15.41 &   15.27    & 4524 &  62 &  1.07 & $-$2.05   & 2.20 \\
MKV0556    & 3 &   06 42 22.27 $-$50 52 09.6 &   19.21 &    0.94 &   18.09 &   17.32 &   16.77 &   16.66    & 4814 &  59 &  1.65 & $-$1.61   & 1.90 \\
MKV0577    & 3 &   06 41 45.03 $-$50 52 49.1 &   18.92 &    1.01 &   17.78 &   16.98 &   16.43 &   16.33    & 4766 &  63 &  1.52 & $-$1.06   & 1.90 \\
MKV0596    & 3 &   06 41 17.69 $-$50 53 07.8 &   18.51 &    1.09 &   17.30 &   16.47 &   15.89 &   15.78    & 4655 &  62 &  1.29 & $-$1.57   & 2.05 \\
MKV0614    & 3 &   06 42 37.98 $-$50 53 38.0 &   18.75 &    1.01 &   17.55 &   16.70 &   16.16 &   16.02    & 4656 &  73 &  1.39 & $-$1.55   & 2.30 \\
MKV0628    & 3 &   06 40 35.38 $-$50 54 07.7 &   18.25 &    1.18 &   16.94 &   16.01 &   15.40 &   15.22    & 4429 &  77 &  1.05 & $-$1.69   & 2.35 \\
MKV0640    & 3 &   06 40 40.84 $-$50 54 29.3 &   18.32 &    1.20 &   17.06 &   16.12 &   15.55 &   15.38    & 4473 &  87 &  1.10 & $-$1.85   & 2.50 \\
MKV0652    & 3 &   06 41 40.83 $-$50 54 45.8 &   18.55 &    1.06 &   17.34 &   16.53 &   15.97 &   15.83    & 4675 &  55 &  1.31 & $-$2.27   & 2.30 \\
MKV0677    & 3 &   06 40 31.14 $-$50 55 24.7 &   17.76 &    1.29 &   16.38 &   15.40 &   14.79 &   14.64    & 4372 &  94 &  0.81 & $-$1.66   & 2.15 \\
MKV0698    & 3 &   06 41 26.12 $-$50 55 44.0 &   17.60 &    1.38 &   16.18 &   15.18 &   14.50 &   14.34    & 4273 &  80 &  0.68 & $-$1.29   & 2.25 \\
MKV0708    & 3 &   06 42 38.52 $-$50 56 00.8 &   18.45 &    1.18 &   17.31 &   16.45 &   15.92 &   15.76    & 4659 &  78 &  1.27 & $-$1.50   & 2.00 \\
MKV0729    & 3 &   06 42 17.46 $-$50 56 26.2 &   18.69 &    1.06 &   17.47 &   16.59 &   16.03 &   15.90    & 4600 &  76 &  1.33 & $-$1.17   & 1.85 \\
MKV0733    & 3 &   06 42 30.38 $-$50 56 33.2 &   18.78 &    1.04 &   17.55 &   16.67 &   16.15 &   15.99    & 4610 &  93 &  1.37 & $-$1.19   & 1.95 \\
MKV0740    & 3 &   06 41 29.07 $-$50 56 46.3 &   18.97 &    1.03 &   17.79 &   16.94 &   16.38 &   16.26    & 4664 &  65 &  1.48 & $-$0.97   & 2.35 \\
MKV0743    & 3 &   06 41 45.92 $-$50 56 54.3 &   19.22 &    0.97 &   18.11 &   17.30 &   16.80 &   16.67    & 4803 &  69 &  1.65 & $-$0.76   & 1.90 \\
MKV0770    & 3 &   06 41 12.30 $-$50 57 26.1 &   18.33 &    1.04 &   17.13 &   16.25 &   15.69 &   15.57    & 4619 &  76 &  1.19 & $-$1.49   & 1.80 \\
MKV0780    & 3 &   06 40 57.09 $-$50 57 44.5 &   18.60 &    1.05 &   17.42 &   16.56 &   16.01 &   15.90    & 4665 &  76 &  1.33 & $-$1.41   & 2.00 \\
MKV0812    & 3 &   06 40 51.62 $-$50 58 21.9 &   19.15 &    0.95 &   18.05 &   17.25 &   16.73 &   16.61    & 4810 &  60 &  1.63 & $-$1.34   & 1.90 \\
MKV0825    & 3 &   06 40 56.96 $-$50 58 38.4 &   18.11 &    1.20 &   16.81 &   15.89 &   15.28 &   15.13    & 4459 &  74 &  1.01 & $-$1.30   & 2.25 \\
MKV0840    & 3 &   06 42 02.81 $-$50 58 59.5 &   18.25 &    1.16 &   16.98 &   16.06 &   15.45 &   15.32    & 4486 &  73 &  1.08 & $-$1.25   & 1.90 \\
MKV0842    & 3 &   06 40 22.52 $-$50 59 02.0 &   19.08 &    0.94 &   17.96 &   17.14 &   16.61 &   16.44    & 4726 &  76 &  1.56 & $-$1.38   & 2.40 \\
MKV0880    & 3 &   06 41 15.67 $-$50 59 48.1 &   17.83 &    1.32 &   16.43 &   15.44 &   14.77 &   14.62    & 4306 &  78 &  0.79 & $-$1.52   & 2.20 \\
MKV0900    & 3 &   06 41 27.18 $-$51 00 18.4 &   17.75 &    1.30 &   16.36 &   15.37 &   14.69 &   14.55    & 4312 &  73 &  0.76 & $-$1.63   & 1.90 \\
MKV0902    & 3 &   06 41 16.31 $-$51 00 18.7 &   18.14 &    1.16 &   16.84 &   15.92 &   15.33 &   15.19    & 4486 &  78 &  1.04 & $-$1.91   & 2.25 \\
MKV0914    & 3 &   06 40 42.49 $-$51 00 42.7 &   18.26 &    1.10 &   16.98 &   16.07 &   15.55 &   15.39    & 4551 &  99 &  1.12 & $-$2.07   & 1.95 \\
MKV0916    & 3 &   06 42 08.97 $-$51 00 48.0 &   18.59 &    1.04 &   17.41 &   16.54 &   15.93 &   15.81    & 4596 &  56 &  1.29 & $-$1.36   & 2.50 \\
MKV0925    & 3 &   06 40 43.17 $-$51 01 06.7 &   18.69 &    1.01 &   17.51 &   16.62 &   16.14 &   16.04    & 4702 & 114 &  1.39 & $-$1.34   & 1.70 \\
MKV0948    & 3 &   06 41 37.66 $-$51 01 43.8 &   18.00 &    1.23 &   16.64 &   15.71 &   15.14 &   14.97    & 4449 &  91 &  0.96 & $-$1.94   & 2.20 \\
MKV0976    & 3 &   06 40 57.68 $-$51 02 40.7 &   18.99 &    0.93 &   17.88 &   17.09 &   16.56 &   16.47    & 4832 &  69 &  1.57 & $-$1.54   & 2.35 \\
MKV1007    & 3 &   06 41 44.65 $-$51 03 31.4 &   18.30 &    1.21 &   16.99 &   16.03 &   15.38 &   15.27    & 4408 &  78 &  1.05 & $-$1.42   & 1.90 \\
MKV1009    & 3 &   06 40 59.29 $-$51 02 26.7 &   18.14 &    1.15 &   16.87 &   15.98 &   15.38 &   15.23    & 4514 &  68 &  1.06 & $-$1.52   & 1.75 \\
MKV1012    & 3 &   06 41 00.31 $-$51 03 43.1 &   18.42 &    1.10 &   17.19 &   16.29 &   15.70 &   15.58    & 4551 &  73 &  1.19 & $-$1.56   & 2.20 \\
MKV1061    & 3 &   06 41 29.16 $-$51 05 22.2 &   18.60 &    1.12 &   17.38 &   16.54 &   15.93 &   15.83    & 4618 &  66 &  1.30 & $-$1.37   & 2.15 \\
\enddata                                                                                                      
\tablenotetext{a} {Sources: 1 = \citet{venn12}; 2 = \citet{shetrone03}; and 3 = \citet{lemasle12}}
\end{deluxetable}      

